Invalidation-Based Protocols for Replicated Datastores

Distributed in-memory datastores underpin cloud applications that run within a datacenter and demand high performance, strong consistency, and availability. A key feature of datastores is data replication. The data are replicated across servers because a single server often cannot handle the request load. Replication is also necessary to guarantee that a server or link failure does not render a portion of the dataset inaccessible. A replication protocol is responsible for ensuring strong consistency between the replicas of a datastore, even when faults occur, by determining the actions necessary to access and manipulate the data. Consequently, a replication protocol also drives the datastore's performance. Existing strongly consistent replication protocols deliver fault tolerance but fall short in terms of performance. Meanwhile, the opposite occurs in the world of multiprocessors, where data are replicated across the private caches of different cores. The multiprocessor regime uses invalidations to afford strongly consistent replication with high performance but neglects fault tolerance. Although handling failures in the datacenter is critical for data availability, we observe that the common operation is fault-free and far exceeds the operation during faults. In other words, the common operating environment inside a datacenter closely resembles that of a multiprocessor. Based on this insight, we draw inspiration from the multiprocessor for high-performance, strongly consistent replication in the datacenter. The primary contribution of this thesis is in adapting invalidating protocols to the nuances of replicated datastores, which include skewed data accesses, fault tolerance, and distributed transactions.

==> Makefile <==
#
## Makefile for acmart package
#

PACKAGE=infthesis

MAIN_TEX=main


TEXSRCS := $(wildcard *.tex) \
	   $(wildcard ./Visuals/*/.tex) \
	   $(wildcard ./Tweaks/*.tex) \
	   $(wildcard ./Text/*.tex) \
	   $(wildcard ./Text/*/*.tex) \
	   $(wildcard ./Text/*/*/*.tex) \


all:  $(MAIN_TEX).pdf

%.cls:   %.ins %.dtx  
		pdflatex $<

#$(MAIN_TEX).pdf:  $(PACKAGE).cls ACM-Reference-Format.bst $(TEXSRCS)
$(MAIN_TEX).pdf:  $(PACKAGE).cls $(TEXSRCS)
		pdflatex $(MAIN_TEX)
		- bibtex $(MAIN_TEX)
		pdflatex $(MAIN_TEX)
		pdflatex $(MAIN_TEX)

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	./Text/Appendixes/*.aux \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

pdf-clean: clean
	$(RM) $(MAIN_TEX).pdf


==> Makefile-old <==
# Makefile for installing the infthesis LaTeX class, eushield
# package, and associated logos.
#
# To install infthesis.cls type:
# $ make install
#
# To install the required eushield.sty type:
# $ make install-eushield
#
# To install logos type:
# $ make install-logo-inf
# $ make install-logo-cdtppar
# $ make install-logo-epsrc
#
# Each install command has an associated uninstall command, e.g. to
# uninstall the infthesis class and eushield.sty type:
# $ make uninstall
# $ make uninstall-eushield

TEXMF=$(HOME)/.texmf/tex/latex
INSTDIR?=$(TEXMF)
TEXINFTHESIS=$(INSTDIR)/uoe/informatics/infthesis

TEXEUSHIELD=$(INSTDIR)/uoe/informatics/eushield
EUSHIELDURL=http://dream.inf.ed.ac.uk/projects/polyml/application/cover-letter/tex/logos
EUSHIELD= \
	eushield.sty eushield.eps \
	eushield-normal.pdf eushield-normal.ps \
	eushield-noback.pdf eushield-noback.ps \
	eushield-reversed.pdf eushield-reversed.ps \
	eushield-twocolour.pdf eushield-twocolour.ps \
	eushield-fullcolour.pdf eushield-fullcolour.ps

INFLOGODIR=$(INSTDIR)/logos/informatics
INFURL=http://media.inf.ed.ac.uk/infweb/logos
INFLOGO=InformaticsUni_spot.eps InformaticsUni_CMYK.eps

CDTPPARLOGODIR=$(INSTDIR)/logos/cdtppar
CDTPPARURL=http://media.inf.ed.ac.uk/infweb/ppar-logos
CDTPPARLOGO=cmyk.eps black.eps white.eps

EPSRCLOGODIR=$(INSTDIR)/logos/epsrc
EPSRCURL=https://www.epsrc.ac.uk/files/aboutus/logos-and-indentity
EPSRCLOGO=white-out-sponsorship-logo:sponsor-wofullres.eps \
					black-and-white-sponsorship-logo-full-resolution:sponsor-bwfullres.eps \
					colour-sponsorship-logo-full-resolution:sponsorfullres.eps


install: infthesis.cls
	@mkdir -v -p $(TEXINFTHESIS) && \
	cp -v infthesis.cls $(TEXINFTHESIS)/infthesis.cls && \
	texhash --verbose $(INSTDIR) && \
	echo "Installation complete." || echo "Installation failed."

uninstall: $(TEXINFTHESIS)/infthesis.cls
	@rm -v $(TEXINFTHESIS)/infthesis.cls && \
	texhash --verbose $(INSTDIR) && \
	echo "Uninstallation complete." || echo "Uninstallation failed."
	@echo "Attempting to removing directory structure."
	@rmdir -v -p $(TEXINFTHESIS) && true || true

install-eushield:
	@mkdir -v -p $(TEXEUSHIELD)
	$(foreach dep, $(EUSHIELD), \
		echo "Installing $(dep)..." && \
		curl -o $(TEXEUSHIELD)/$(dep) -O $(EUSHIELDURL)/$(dep) && \
		echo "Installation of $(dep) complete." || echo "Installation of $(dep) failed." ; \
	)
	texhash $(INSTDIR)

uninstall-eushield:
	$(foreach dep, $(EUSHIELD), \
		echo "Uninstalling $(dep)..." && \
		rm -v $(TEXEUSHIELD)/$(dep) && \
		echo "Uninstallation of $(dep) complete." || echo "Uninstallation of $(dep) failed." ; \
	)
	texhash $(INSTDIR) && \
	@rmdir -p -v $(TEXEUSHIELD) && true || true

install-logo-inf:
	@mkdir -v -p $(INFLOGODIR)
	$(foreach dep, $(INFLOGO), \
		echo "Installing $(dep)..." && \
		curl -o $(INFLOGODIR)/$(dep) -O $(INFURL)/$(dep) && \
		echo "Installation of $(dep) complete." || echo "Installation of $(dep) failed." ; \
	)

uninstall-logo-inf:
	$(foreach dep, $(INFLOGO), \
		echo "Uninstalling $(dep)..." && \
		rm -v $(INFLOGODIR)/$(dep) && \
		echo "Uninstallation of $(dep) complete." || echo "Uninstallation of $(dep) failed." ; \
	)
	@rmdir -v -p $(INFLOGODIR) && true || true


install-logo-cdtppar:
	@mkdir -v -p $(CDTPPARLOGODIR)
	$(foreach dep, $(CDTPPARLOGO), \
		echo "Installing $(dep)..." && \
		curl -o $(CDTPPARLOGODIR)/$(dep) -O $(CDTPPARURL)/$(dep) && \
		echo "Installation of $(dep) complete." || echo "Installation of $(dep) failed." ; \
	)

uninstall-logo-cdtppar:
	$(foreach dep, $(CDTPPARLOGO), \
		echo "Uninstalling $(dep)..." && \
		curl -o $(CDTPPARLOGODIR)/$(dep) -O $(CDTPPARURL)/$(dep) && \
		echo "Uninstallation of $(dep) complete." || echo "Uninstallation of $(dep) failed." ; \
	)
	@rmdir -v -p $(CDTPPARLOGODIR) && true || true

install-logo-epsrc:
	@mkdir -v -p $(EPSRCLOGODIR)
	$(foreach dep, $(EPSRCLOGO), \
		$(eval dep1 = $(word 1,$(subst :, ,$(dep)))) \
		$(eval dep2 = $(word 2,$(subst :, ,$(dep)))) \
		echo "Installing $(dep2)..." && \
		curl -o $(EPSRCLOGODIR)/$(dep2) -O $(EPSRCURL)/$(dep1) && \
		echo "Installation of $(dep2) complete." || echo "Installation of $(dep2) failed." ; \
	)

uninstall-logo-epsrc:
	$(foreach dep, $(EPSRCLOGO), \
		$(eval dep1 = $(word 1,$(subst :, ,$(dep)))) \
		$(eval dep2 = $(word 2,$(subst :, ,$(dep)))) \
		echo "Uninstalling $(dep2)..." && \
		curl -o $(EPSRCLOGODIR)/$(dep2) -O $(EPSRCURL)/$(dep1) && \
		echo "Uninstallation of $(dep2) complete." || echo "Uninstallation of $(dep2) failed." ; \
	)
	@rmdir -v -p $(EPSRCLOGODIR) && true || true


==> Text/0-Preface/acknowledgements.tex <==
\begin{acknowledgements}

\equote{-5}{0}{Here I stand at what is called the Cross of Edinburgh,\linebreak %\\
and can in a few minutes take fifty men of genius by the hand.}{John Amyatt}
% TODO
% \begin{comment}
% \antonis{System research is full of collaboration}
% \antonis{Impact vs. Papers}
% \todo{My warmest thanks to Arpit Joshi, for without his help in the early stages of my PhD it would have taken me much longer to get acclimated to the PhD life.}

To properly thank everyone who contributed in one way or another to this thesis would be impossible, for I would need as many pages 
as the remainder of this work.
% as remain in this work.
While, I will keep this section brief, I am incredibly thankful to all of you!

% Of course, t
This thesis would not have been possible without the guidance of my principal advisor Prof. Boris Grot. I immensely appreciate his patience, invested time, and detailed feedback on scientific matters as well as  on communication skills. I will also never forget the countless all-nighters he undertook to assist with paper deadlines. His cultivation of ideas and clarity of thought is astounding.

Throughout my studies and my life in general, I have been blessed with many advisors and mentors who have granted me valuable research and life advice. First, I would like to thank Prof. Vijay Nagarajan, who has an excellent character and is a role model of an academic. He taught me to think based on first principles and always encouraged me to go one level deeper, leading to valuable insights. I cannot thank enough Aleksandar Dragojevic and Bozidar Radunovic of Microsoft Research for their mentorship, long conversations, and for trusting me with exciting projects throughout almost the entire span of my postgraduate studies. 
% 
My Ph.D. journey would not have begun without my undergraduate advisor, Prof. Angelos Bilas, who made me fall in love with research. I am forever obliged to him.
I also owe special thanks to Panagiotis Garefalakis and Vasileios Trigonakis for guiding me through important life and career decisions.
Finally, I am particularly indebted to my swimming coach, Michalis Iliopoulos who taught 
me a great deal about 
\scalebox{1}{\textit{consistency}, \textit{fault tolerance}, and \textit{high performance}.}


I am grateful for the opportunity to learn and receive feedback from the best across several fields of computer science, spanning architecture, databases, and systems.
% , some specializing in hardware, others on software. 
% Moreover,
I am very thankful to Anuj Kalia, Dushant Nagarajan, Haggai Eran, Miguel Castro, Nikos Nikoleris, Paolo Costa, Pramod Bhatotia, Robbert van Renesse, Virendra Marathe, and Vitor Enes for their research advice and comments on manuscripts. 
% In addition, 
I especially want to thank the numerous anonymous reviewers, as well as Rodrigo Rodrigues, Kimberly Keeton, and Liuba Shrira, all of whom shepherded papers containing results that appear on this thesis. Finally, I want to express my most profound appreciation to Michio Honda, Murray Cole, and Rodrigo Rodrigues, who served on my dissertation committee and provided feedback that substantially improved the shaping of this thesis.

This work would have been impossible without the support of others, as well. First and foremost, I was fortunate enough to collaborate closely with Vasilis Gavrielatos, a researcher with an incredible mind but, more importantly, a friend who always listened to my worries.
I also offer my warmest thanks to Arpit Joshi; without his help 
in the early stages of my Ph.D., 
it would have taken me much longer to get acclimated. I also extend great thanks to Yijun Ma, whose internship performance was astonishingly good, despite working remotely.
% during a pandemic.
% , and all other co-authors and researchers who directly or indirectly influenced my work. 
I am fortunate to have  had brilliant colleagues~---~Adarsh, Amna, Artemiy, Cillian, Dmitrii, Fazel, Giorgos P., Harsa, Jose, Mahesh, Mingcan, Nicolai, Priyank, Rodrigo, and Siavash~---~with whom I regularly exchanged ideas and good laughs. Furthermore, I am very appreciative to the Mosque Kitchen personnel, who spiced up my day-to-day life with their delicious food, and Rita the cleaner, who kept my desk free of clutter, allowing me to focus on my research without distractions. Finally, I am thankful for the generous funding, equipment, and other support provided by Microsoft Research, the University of Edinburgh, EPSRC, and Cloudlab that I received during my studies.

This endeavor would have been much more difficult without friends and family.
I would like to offer individual thanks to Aleksis, Andreas, Dimitra, Dimitris, Eleana, Giannis, Giorgos K., Giorgos N., Giorgos Z., Giota, Hara, Ilias, Manos, Maria, Nantia, Natasa, Nicole, Nikos K., Nikos X., Polis, Stelios, Spyros, and Vivi for keeping me sane and providing me with a beautiful life outside science. I cannot thank my brother Aleksandros and my parents, Apostolia and Emmanouel, enough for their unconditional love, relentless encouragement, and for being a positive influence in my life.
Last but not least, I want to express my deepest gratitude to my dear Despina for following me to Edinburgh without hesitation while always offering her love and patience throughout these years.

\vspace{10pt}
\textit{Isolated during a pandemic, October 2021 \hfill Antonios Katsarakis}


\begin{comment}

Since I was a kid, I was taught to be grateful for everyone and everything, no matter how insignificant or adverse they might seem at first glance.
I sincerely believe that there is not even a single person I have interacted with who has not influenced me positively through my lifespan in this world. 
Consequently, to properly thank everyone who contributed in one way or another to this thesis is impossible, for I would need at least as many pages as the reminder of this work.
To properly thank everyone who contributed in one way or another to this thesis is impossible, for I would need at least as many pages as the reminder of this work.
Instead, I will try to keep this section brief to aid the reader, yet I am incredibly thankful to all of you!

This thesis would have been impossible without the guidance of my principal advisor Prof. Boris Grot. I immensely appreciate his patience, invested time, and detailed feedback on scientific matters and communication skills. I will also never forget the countless all-nighters he undertook to help with paper deadlines. His cultivation of ideas and clarity of thought is unbelievable.

% There is no doubt that I was fortunate to have other advisors and mentors 
I have been blessed throughout my Ph.D. and life in general with many advisors and mentors who have granted me valuable research and life advice.
Namely, Prof. Vijay Nagarajan, who has a beautiful character and is a role model of an academic, taught me to think based on first principles and always encouraged me to go one level deeper, leading to valuable insights.
I would like to especially thank Aleksandar Dragojevic and Bozidar Radunovic from Microsoft Research for their mentorship, long-lasting conversations, and for trusting me with exciting projects during almost the entire span of my Ph.D. Special thanks are also deserved to Vasileios Trigonakis and Panagiotis Garefalakis for guiding me through important life and career decisions.
I am particularly indebted to my swimming coach Michalis Iliopoulos who taught me a lot, including the art of \textit{fault tolerance}, \textit{consistency} and \textit{high performance} (in real life).
Finally, my Ph.D. endeavor would not have started without my undergraduate advisor Angelos Bilas, who made me fall in love with research. I am forever obliged to him.
% including that discipline and consistency are necessary for performance in life (unlike in systems). 
% I am also grateful to hundreds of book authors for sharing their thoughts and ideas, which have shaped my character.


I am grateful for the opportunity to interact, learn and get feedback from the best across several fields of computer science spanning computer architecture, databases, and systems, some specializing in hardware others on software. 
Moreover, I am very thankful to Anuj Kalia, Dushant Nagarajan, Haggai Eran, Miguel Castro, Nikos Nikoleris, Virendra Marathe, Vitor Enes, Paolo Costa, Pramod Bhatotia, and Robbert van Renesse for their research advice and comments on manuscripts. I want to express my deepest appreciation to numerous anonymous reviewers, Rodrigo Rodrigues, Kimberly Keeton and Liuba Shrira who shephered our work. Finally, I want to especially thank Michio Honda and Rodrigo Rodrigues who served on my dissertation committee and provided feedback that dramatically improved the shaping of this thesis.
% both in theory and practice, 
% I want to especially thank Panagiota Fatourou for helping me to demystify systems theory and write with more rigor. 

% Unlike my other students my PhD was far from a struggle. This was mainly due to fruitful collaborations which always kept the spark on. 
This work would have been impossible without the support of other people.
First and foremost, I was fortunate to collaborate closely with Vasilis Gavrielatos, a researcher with a beautiful mind but, more importantly, a friend who always listened to my worries.
My warmest thanks to Arpit Joshi, for without his help in the early stages of my Ph.D. it would have taken me much longer to get acclimated to the Ph.D. life.
Big thanks to Yijun, an astonishingly good intern, and all other co-authors and researchers who directly or indirectly influenced my work. I was also extremely lucky to have brilliant colleagues; Adarsh, Amna, Dmitrii, Mahesh, Mingcan, Nicolai, Priyank, Rodrigo and Siavash with whom I ate and exchanged ideas regularly. I am very appreciative to the Mosque Kitchen personnel that spiced up my Ph.D. life through their delicious food and Rita the cleaner, who kept my desk clutter-free, allowing me to focus solely on my research without distractions.
Finally, I am thankful for the generous funding, equipment any other support I received during my studies provided by Microsoft Research, University of Edinburgh, EPSRC, and Cloudlab.
% If my PhD had much less struggle than usual I own it to him and our fruitful collaborations. % I was extremely lucky to have numerous fruitful collaborations with him.




This endeavor would have been very difficult without friends and family.
Individual thanks to Aleksis, Andreas, Dimitra, Dimitris, Giannis, Giorgos, Giorgos, Giota, Hara, Manos, Maria, Nikos, Nikos, Polis, and Vivi for keeping me sane and happy and for providing me with a beautiful life outside of science. 
I could not thank my brother Aleksandros enough and my parents, Apostolia and Emmanouel, for their unconditional love, encouragement and for being such a positive influence in my life.
Last but not least, I want to express my deepest gratitude to my dear Despina for following me in Edinburgh without hesitation while always filling me with her selfless love, support, understanding and the much-needed patience throughout all these years.
% \vspace{10pt}
\textit{Isolated during a pandemic, August 2021 \hfill Antonios Katsarakis}
\end{comment}

% \noindent\textit{The University of Edinburgh,}
% 
% \hfill \textit{Antonios Katsarakis}
% \end{comment}

\begin{comment}
Since I was a kid, I was taught to be grateful for everyone and everything, no matter how insignificant or adverse they might seem at first glance.
I sincerely believe that there is not even a single person I have interacted with who has not influenced me positively through my lifespan in this world. 
Consequently, to properly thank everyone who contributed in one way or another to this thesis is impossible, for I would need at least as many pages as the reminder of this work.
Rather I will keep this section brief to aid the reader, yet I am incredibly thankful to all of you!

This thesis would not have been possible without the relentless guidance of my principal advisor Prof. Boris Grot. I immensely appreciated his patience, invested time and the countless all-nighters he undertook to help with paper deadlines. I will never forget his elaborate feedback on scientific matters and communication skills. His cultivation of ideas and clarity of thought is unbelievable.

There is no doubt that I was extremely lucky to have other advisors and mentors who offered me valuable advise throughout my PhD. Namely, Vijay Nagarajan who has a beautiful character and is a role model as an academic taught me to think based on first principles and always try to go one level deeper.
I would like to especially thank Aleksandar Dragojevic and Bozidar Radunovic from Microsoft Research for their mentorship, relentless conversations, and for trusting me to participate in exciting projects  during almost the entire span of my PhD.
Finally, this endeavour would have not started without my undergraduate advisor Angelos Bilas, who introduced me to and made me fall in love with research. I am forever grateful to him.


I am grateful for the opportunity I had to interact, learn and get feedback from the best across several fields of computer science spanning architecture, databases and systems, both in theory and practise, some specializing on hardware others on software. I want to especially thank Panagiota Fatourou for helping me to demystify systems theory and write with more rigor. Moreover, I am very thankful to Dushant Nagarajan, Miguel Castro, Virendra Marathe, Vitor Enes, Paolo Costa, and Robbert van Renesse for their research advice and comments on manuscripts. Finally, I want to express my deep appreciation to numerous anonymous reviewers, shepherds and to the dissertation committee who invested their time and provided feedback that dramatically improved the shaping of the works on this thesis.

This work would have been impossible without the support of other people.
First and foremost, Vasilis Gavrielatos who has a beautiful mind, is a fantastic collaborator and friend who always listened to me. I was extremely lucky to have numerous fruitful collaborations with him.
Big thanks to Yijun who was an astonishingly good intern and all other co-authors and researchers that directly or in-directly influenced my work. I was also extremely lucky to have brilliant colleagues I ate and exchanged ideas with, including Adarsh, Amna, Arpit, Dmitrii, Mahesh, Mingcan, Nicolai, Priyank, Rodrigo and Siavash.
% 
The Mosque Kitchen personel that spiced up my PhD life through their delicious food and Rita the cleaner that kept my desk clutter-free allowing me to focus solely on my research without distractions.
Finally, I am thankful for the generous funding, equipment any other support I received during my studies provided by Microsoft Research, University of Edinburgh, EPSRC and Cloudlab.

I have been blessed throughout my life with many great mentors. I am particularly
indebted to my swimming coach Michalis Iliopoulos who taught me a lot including that in life (and unlike in systems) discipline and consistency is necessary for performance. 
Special thanks to Vasilios Trigonakis and Panagiotis Garefalakis for guiding me through important decisions in my life and career.
I am also grateful to hundreds of book authors for sharing their thoughts and ideas which have shaped my character.

This endeavour would have been very difficult without friends and family.
Individual thanks to Andreas, Aleksis, Dimitris, Dimitra, Giannis, Giota, Giorgos, Giorgos, Hara, Nikos, Nikos, Maria, Manos, Polis and Vivi for keeping me happy and sane, and for providing me with a tremendous life outside of science. 
I could not thank enough my brother Aleksandros and parents, Apostolia and Emmanouel, for their unconditional love and encouragement, and for being such a positive influence in my life.
Last but definitely not least, I want to express my deepest gratitude to Despina for following and staying with me in Edinburgh unconditionally whilst filling me always with her love, support and much needed patience throughout this endeavor.
           
\end{comment}
% his valuable advise throughout my PhD
% I would also like to
% His life 


% There is no doubt that I was extremely lucky to interact and learn from the best across several fields of computer science, from architecture to databases and distributed systems and from theory to practise work at the intersection of hardware and software.

% If you were to say to me 60 months ago that I would 
% I could have not 

% with
% From 

\begin{comment}

experiments , and relentless confidence throughout these

% First and foremost I would like to expresse
% Thank 
\begin{enumerate}
  \item First and foremost.
  \item Last but not least
  \item  wish to thank
  \item wish to express my gratitude 
  \item grateful to
  \item his valuable advise throughout my PhD
  \item his extensive comments and feedback
  \item enjoyable fruitful
  \item I am indebted to for the technical discussions during my internship
  \item I am immensely grateful to my family
  \item without the support and encourangment of several people
  \item several other people played an important role in my doctorate
  \item last but definatelly not least, I am extremely thankful to my brother and parents for their unconditonal love and for being such a positive influcence in my life.
  \item who served on my defense committee. I very much appreciate the time and effort they took to
supervise my dissertation work.
\end{enumerate}

\begin{enumerate}
Since I was a kid I was ta
    I am extremely grateful to have met and be positively influenced by many great people.
    some of which have undertaken this endeavour.
    to several people who one way or the other contributed to this work.
    wish to express my gratidute to ... for  the valuable scientific discussions we had, and for motivating and encouraging my work.
    
    This thesis would not have been possible without the contributions of many people, including the people I may not know or remember.
    First and foremost I would like to thank Boris Grot for his support, guidance and commitment all those years.
    
    \item his patience, guidance, and relentless confidence throughout these
  
    \item Vijay Nagarajan a good human being and always trying think based on first principles.
    \item I  would  also  like  to  thank my co-advisors Vijay Nagarajan and Aleksandar Dragojevic for their time and mentorship
    \item Bozidar Radunovic mentor
    \item Dissertation committee
    \item Panagiota Fatourou: for helping me to demystify systems theory and write rigorously.
    \item Vasilis Trigonakis, Miguel Castro, Virendra Marathe, Paolo Costa, Dushant Nagarajan and Robbert van Renesse for their comments and advice
    
    \item All Co-authors and researchers the directly or in-directly influenced this work.
    \item Vasilis Gavrielatos: was a fantastic collaborator and friend I was extremely lucky to have.
    \item Use only names for the rest no surnames Adarsh, Amna, Arpit, Dmitrii, Mahesh, Mingcan, Nicolai, Priyank and Siavash.
    \item Vitor Enes for his thoughtful 
    \item Alex Miller, Murat Demirbas, Dimos Raptis, Ivan Prisyazhnyy
    
    
    \item Not have been possible without my undergraduate advisor Angelos Bilas, who introduced me and made me fall in love with research.
    \item EPSRC, MSR grants and any other source of funding I have received for their generous support during my studies. 
          The University of Edinburgh, Microsoft Research and Cloudlab for the equipment which they provided that was necessary for our experiments.
    \item I am thankful for numerous anonymous reviewers who invested their time and provided feedback that dramatically improved the shaping of the works of this thesis.
    
    
    \item I am grateful All the teachers since my early years and especially my swimming coach who taught me that (unlike system research beliefs) discipline and consistency is necessary for high-performance. 
    \item I am grateful to hundreds of book authors for sharing their thoughts and ideas which have shaped my character.
    \item Brian Johnson for distilling ideas and ancient wisdom and made them practical in the modern context 
    \item The creativeness of ancient myths that provide inspiration to this work.
    
    \item Mosque Kitchen that empowered me through their delicious food and Rita the cleaner that kept my desk clutter-free allowing me to focus on my research without distractions.
    
    
    
    
   
    % without all the support from my parents, Štefanija and Milenko, and my sister Tanja.
    
    % Antonios Katsarakis 
    % Isolated during a pandemic, 15th May 2021,   
\end{enumerate}
\end{comment}

\end{acknowledgements}

% Sparked my curiosity!
% Loving of all people
% Competitive yet

==> Text/0-Preface/biosketch.tex <==
\begin{biosketch}
Get inspiration from the hilarious one included in "RELIABLE COMMUNICATION FOR DATACENTERS (Mahesh Balakrishnan)" 
\end{biosketch}


==> Text/0-Preface/dedication.tex <==

\dedication{
% \equote{-50}{150}{'Εν οἶδα, ὅτι οὐδέν οἶδα.\\I know that I know nothing.}{Socrates}
\equote{-50}{150}{I know that I know nothing.}{Socrates}
% \vspace{200pt}

% \vspace{100pt}
% Στη Δέσποινα και τους γονείς μου,
% \\ Αποστολία και Εμμανουήλ
% \vspace{40pt}
% \\To Despina and my parents,
% \\ Apostolia and Emmanuel
\vspace{20pt}
To Despina and my parents,
\\ Apostolia and Emmanuel
\vspace{20pt}


% \equote{150}{0}{Good artists copy, great artists \sout{steal}\\ \textit{consistently replicate} with a spark of originality.} {\sout{Pablo Picasso}\\ The author}

% \equote{150}{0}{\sout{Good artists copy, great artists steal.}} {\sout{Pablo Picasso}}
% \equote{0}{0}{Good researchers reproduce,\\ great researchers \textit{consistently replicate}\\ with a spark of originality.} {The author}

\equote{150}{0}{Good researchers reproduce,\\ great researchers \textit{consistently replicate}\\ with a spark of originality.\\\vspace{5pt}
\sout{Good artists copy, great artists steal.}} {\sout{Pablo Picasso}}
% \equote{0}{0}{} {The author}

}

% \dedication{\textit{To Despina and my parents, Apostolia and Emmanuel}}
% \dedication{\textit{To Despina and my parents,\\ Apostolia and Emmanuel}}
% \dedication{\textit{To Despina and my parents}}

==> Text/0-Preface/lay.tex <==
\begin{lay} % lay summary
Today's most popular applications, including social networks, telecommunications, and financial services, rely on datastores to store their ever-growing data. Datastores split and store application data across a cluster of machines. As modern applications have numerous concurrent users who generate data requests, datastores must deliver high performance. For performance, datastores replicate application data across multiple machines. Replication also ensures that data remain accessible in the face of machine crashes and other faults.

Datastores deploy replication protocols to keep the replicas synchronized and provide the illusion of a single copy (i.e., strong consistency), even when faults occur. To achieve this, replication protocols define the exact actions required to access and update the data. Thus, in addition to guaranteeing strong consistency and the ability to endure faults, replication protocols also determine the performance of a datastore.

However, the existing replication protocols deployed by datastores fall short in terms of performance. Meanwhile, protocols for strong consistency are also well established when data are replicated across different memories inside a multiprocessor. Protocols in the multiprocessor context synchronize replicas using invalidations to deliver high performance but cannot tolerate failures.

In this thesis, we observe that the common operation of replication protocols in datastores does not involve faults closely resembling the multiprocessor setting. Based on this insight, we propose multiprocessor-inspired invalidating protocols for replicated datastores that achieve high performance. The invalidating protocols of this thesis are adapted to the challenges of replicated datastores, which (among others) include guaranteeing data availability and fault tolerance.

% However, existing replication protocols deployed by datastores fall short in performance. Meanwhile, protocols for strong consistency are not a unique feature of datastores, they are also well-established in the context of data replication within the multiprocessor. Protocols in the multiprocessor context use invalidations to efficiently synchronize replicas and deliver high performance, albeit they do not tolerate faults.
\end{lay}

\begin{comment}
Today's cloud applications, including social networks, telecommunication and financial services, rely on datastores to store their important and ever-growing data. Datastores split and store the application data across a cluster of machines. As modern applications have numerous concurrent users generating data requests, datastores must deliver high performance.
Datastores replicate the application data across different machines to increase performance and ensure that data remain accessible despite machine crashes and other faults.

Datastores deploy replication protocols to facilitate correctness when updating replicated data. A replication protocol keeps the replicas synchronized -- even when faults occur -- providing the illusion of a single copy (i.e., strong consistency). To attain that, replication protocols define the exact actions to access and update the data. Thus, besides guaranteeing strong consistency and sustaining faults, replication protocols also determine the datastore's performance.

However, existing replication protocols deployed by datastores fall short in performance. Meanwhile, protocols for strong consistency are also long-practiced in another context, when the hardware replicates data across different memories in the multiprocessor. Strongly-consistent protocols deployed by the multiprocessor use invalidations to deliver high performance but unlike replication protocols in datastores they cannot tolerate failures and provide data availability.

In this thesis, we observe that the common operation of replication protocols in datastores does not involve failures. Based on this insight we apply multiprocessor-inspired invalidating protocols in the datastore setting to increase the performance of replicated datastores while also adequately adapting those protocols to the different context and challenges of datastores
which among others includes guaranteeing data availability when faults occur.
\end{comment}

% fault tolerance and data availability.
% adequately adapted to the different context and challenges of datastores.

% To facilitate correctness when updates occur on replicated data, datastores rely on replication protocols which keep the replicas synchronized -- even if faults happen -- providing the illusion of a single data copy (i.e., strong consistency). Replication protocols achieve that by defining the exact actions to access and update the data. Thus, besides guaranteeing strong consistency and sustaining faults, replication protocols also determine the datastore's performance.

% Existing replication protocols deployed by datastores fall short in performance. Meanwhile, protocols for strong consistency are also long-practiced when data are replicated within a single machine.
% In contrast, to replication protocols in datastores, 
% Protocols deployed to keep the replicas synchronized within a single machine use invalidations to deliver high performance but they cannot tolerate failures.


% Existing replication protocols deployed by datastores provide strong consistency between data replicas and remain operational despite failures, albeit they fall short in performance. 
% Meanwhile, protocols for strong consistency are also long-practiced when data are replicated within a single machine.

\begin{comment}
\begin{lay}
\todo{General todos}
\squishlist
    \item Make sure all figures have the same "theme" look-alike
    \item use the same font as the text in the figures
    % 
    \item ensure consistency across chapters on capitalization, ttt (pick font) etc. eval numbers in math or not
    \item Minimize forward references 
    \item Minimize different emphasis
    \item avoid hyphenated words (e.g., via linebreak)
    \item remove mathmode from all numbers inside the text
    \item avoid duplicate references or in text (?)
    \item Go again over reviewer comments
    \item fully-distributed vs decentralized
    % \item Add logical timestamps in intro/background
    \item Fault-tolerance (not durability)
    \item Define partial synchrony/asynchrony
    \item remove a "pool of nodes" from ccKVS description
\squishend

Content 
\squishlist
    \item add Hermes RMW graph
    \item listing for the protocols
    \item supplementing images, analogies and examples. Minimize JARGON!
    % \item SMR great abstraction to waste performance in a modern world, it is not a good fit for multi-threading. A lot are trying to retrofit parallelism via speculation or reactive re-ordering of non-conflicting commands (e.g., parallelism ) but still no go!
    \item Merged related work?
    \item minimize parenthesis, this that 
    \item Less boring section titles (e.g., get ideas from books)
    \item Research questions asked? and answered
    \item  \beginbsec{Research Question} \beginbsec{Challenge} \beginbsec{Opportunity}
\squishend

\end{lay}
\end{comment}


% Modern applications and services including social networks, e-commerce, health, as well as telecommunication and the financial sector are housed in .

% in datacenters where clusters of computers collaborativelly store and serve their data.
% In today's a data-driven world most modern applications including social networks, e-commerce, 
% as well as telecommunication and financial services 
% , as well as telecommunication and the financial sector 
% are housed in inside datacenters where large clusters of computers exists.
% To store their data across the machines 
% A similar strongly-consistent replication is already solved for data replicated within a single multiprocessor machine which are in an efficient way. However, since multiprocessors tend to fail individually these protocols fail to consider fault-tolerance.
% These applications rely on datastores services that split and partition their data provided
% inside datacenters where large clusters of computers exists (also known as "the cloud").

% Datastores: High performance and availability.
% Data availability and performance
% Replication 
% Strong consistency (remain synchronize in the presence of updates as if there is no replication)
% Performance
% Existing replication protocols fail to offer performance
% Multiprocessor strongly consistent replication with high performance over invalidation protocols. However, these protocols are tailored for the single machine setting and are thus are not fault-tolerant. 
% In this thesis we take inspiration from the multi-processor and design invalidation-based replication protocols
% primitives like atomic durability, which allow programmers to write crash consistent programs for systems with persistent memory.
% Datastores split the application

% Data are replicated across nodes because a single node often cannot keep up with the request load. Replication is  also  necessary  to  guarantee  that  a  node  or  link  failure  does  not  render a  portion  of  the  dataset  inaccessible. 

% Today's cloud applications, including social networks, telecommunication and financial services, rely on datastores to store their important and ever-growing data.
% Datastores split and store the application data across a cluster of several machines.
% Since modern applications have numerous concurrent users requests, datastores must deliver high performance.
% Datastores must also replicate the application data across different machines to guarantee that the data remain accessible in the presence of failures such as machine crashes.

% To facilitate correctness when updates occur on replicated data, datastores rely on replication protocols which keep the replicas synchronized providing the illusion of a single data copy (i.e., strongly-consistent). Replication protocols achieve that by determining the exact actions to access and update the data even when faults occur. Thus, besides guaranteeing strongly-consistent replicas and sustaining faults, replication protocols also determine the datastore's performance.

% Existing replication protocols deployed by datastores fall short in performance. Meanwhile, protocols for strong consistency are also long-practiced when data are replicated within a single machine.
% In contrast, to replication protocols in datastores, 
% Protocols deployed to keep the replicas synchronized within a single machine use invalidations to deliver high performance but they cannot tolerate failures.

% Existing replication protocols deployed by datastores provide strong consistency between data replicas and remain operational despite failures, albeit they fall short in performance. 
% Meanwhile, strongly-consistent protocols is a well-established practice when data are replicated within a single machine.
% Protocols deployed to keep the replicas synchronized within a single machine use invalidations to deliver high performance but they cannot tolerate failures.

% In this thesis we observe that the common operation of replication protocols in datastores does not involve failures. Based on this insight we apply single-machine-inspired invalidating protocols in the datastore setting to increase the performance of replicated datastores while also adapting those protocols to ensure that data remain available when faults occur.

% provide high performance but they cannot guarantee operation under faults. 

% are also used in a similar setting where

% This thesis take inspiration from the multiprocessor and presents efficient invalidation-based replication protocols tailored to advance the performance of replicated datastores without compromising data availability. 



==> Text/0-Preface/preface.tex <==
\begin{preface}
The work presented in this thesis was conducted in the EASE lab at
The University of Edinburgh under the supervision of Prof. Boris Grot and Prof. Vijay Nagarajan.

\vspace{10pt}
\noindent The results of this thesis are based on the following papers:
\begin{enumerate}
    \item so-ccNuma
    
    \item Lara (and faults). Under submission
    \item Hermes (+ async)
    \item Zeus
    % \item rVNF
    % \item New internship work (?)
\end{enumerate}

\vspace{10pt}
\noindent Besides work presented in the thesis, during my PhD I carried out research resulting in several other publications including:
\begin{enumerate}
    \item rVNF
    \item Kite
    \item Odyssey
    \item Extending Classic Paxos for High-performance Read-Modify-Write Registers
    \item Mingcan's paper
\end{enumerate}

\end{preface}


==> Text/0-Preliminaries/Misc/Fig_ops.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Text/0-Preliminaries/Figures/ops.pdf}
  \caption{Primitives offered by datastores. 
%   A partial order to relate various isolation levels.
  Arrows point to more general primitives.}
%   \todo{May add single-shard transactions.}} 
  \label{figB:ops}
\end{figure}

==> Text/0-Preliminaries/Misc/Fig_ops_example.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/0-Preliminaries/Figures/ops-example.pdf}
  \caption{Examples of different update operations offered by datastores.} 
  \label{figB:ops_example}
\end{figure}

==> Text/0-Preliminaries/Misc/Tab_motivation2.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.8 \textwidth}
\begin{tabular}{l|lll}
                  & \textbf{\hyperref[chap:cckvs]{Scale-out ccNUMA}} 
                  & \textbf{\hyperref[chap:hermes]{Hermes}} 
                  & \textbf{\hyperref[chap:Zeus]{Zeus}} \\ \cline{2-4} 
                %   & \textbf{{Scale-out ccNUMA}} 
                %   & \textbf{{Hermes}} 
                %   & \textbf{{Zeus}} \\ \cline{2-4} 
\textbf{\begin{tabular}[c]{@{}l@{}}Key drive \\ for replication\end{tabular}} &
  performance &
  \begin{tabular}[c]{@{}l@{}}availability\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}availability\end{tabular} \\
\textbf{\begin{tabular}[c]{@{}l@{}}Access\\primitives\end{tabular}} &
  reads/writes &
  reads/writes &
%   single-object &
%   single-object &
%   \begin{tabular}[c]{@{}l@{}}multi-object\\ transactions\end{tabular} \\
  transactions\\
%   \begin{tabular}[c]{@{}l@{}}transactions\end{tabular} \\
\textbf{Data sharding} & static                    & static          & dynamic 
% \\ \textbf{Evaluated networking} & RDMA & RDMA & DPDK 
\end{tabular}
\end{adjustbox}

% \caption{Different replication contexts in datastores improved by this thesis.
\mcaption{Different contexts of replicated datastores improved by this thesis.}
{Context differences in replicated datastores improved by this thesis.
% which benefited by invalidation-based protocols to improve performance and guarantee the strongest consistent.
}
\label{tabM:contexes}
\end{table}

==> Text/0-Preliminaries/Misc/Tab_read2.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.8 \textwidth}





\begin{tabular}{l|ccc}
 &
  \begin{tabular}[c]{@{}c@{}}\textbf{Coordination}
%   \\ (round-trips to other\\ replicas in critical path)
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Strong consistency} \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Fault tolerance} \end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Reads\\ Writes\end{tabular} & \begin{tabular}[c]{@{}c@{}} \hspace{9pt}0\\ \hspace{9pt}0\end{tabular}                                 & \xmark & \xmark \\ \hline
\begin{tabular}[c]{@{}l@{}}Reads\\ Writes\end{tabular} & \begin{tabular}[c]{@{}c@{}}\hspace{9pt}1\\\hspace{9pt}0\end{tabular}                                 & \cmark & \xmark \\ \hline
% \begin{tabular}[c]{@{}l@{}}Reads\\ Writes\end{tabular} & \begin{tabular}[c]{@{}c@{}}0\\ 1\end{tabular}                                 & v & v \\ \hline
\begin{tabular}[c]{@{}l@{}}Reads\\ Writes\end{tabular} & \begin{tabular}[c]{@{}c@{}} \raisebox{2pt}{\scalebox{0.7}{$\geq$}} 0\\ 
\raisebox{2pt}{\scalebox{0.7}{$\geq$}} 1\end{tabular} & \cmark & \cmark
\end{tabular}








\end{adjustbox}



\mcaption
{Coordination of reads and writes for fault tolerance and consistency.}
{Fault tolerance and consistency of reads and writes from all replicas 
based on coordination (i.e., round-trips to other replicas in the critical path).}
\label{tabM:read-write}
\end{table}

==> Text/1-ccKVS/5.5-Protocol.tex <==
\vspace{0.02in}
\noindent\textbf{\textit{Read}}: 
Any cache can service a read request of a cached object by returning the local value of the requested key if it is in the Valid state. If the key is in any other state, the request is temporarily stalled.

\noindent\textbf{\textit{Write}}\footnote{\CAP{RMW}s to a key are handled in the same way.}:
Any node with a cache may invoke a write to a cached key. That node is called the write's \textit{coordinator}, the rest of the nodes caching (i.e., holding a replica of) the key are called \textit{followers} for that write.\\
% \underline{Coordinator}: 
\centerline{\underline{Coordinator}}
The coordinator issues a write only if its local (cached) replica of the key is in the Valid state; otherwise the write is temporarily stalled. To issue and complete a write, the coordinator node: 
% \underline{Coordinator}: The coordinator node issues a write to a key only if it is in the Valid state; otherwise the write is stalled. To issue and complete a write, the coordinator node: 
\begin{itemize}[leftmargin=*]
\item\textbf{C\textsubscript{\CAP{TS}}}: Updates the key's local timestamp by incrementing its \VAR{version} and appending its node id as the 
\cid, and assigns this new timestamp to the write.

\item\textbf{C\textsubscript{\CAP{INV}}}: Promptly broadcasts an \CAP{INV} message consisting of the \VAR{key} and the new timestamp (\VAR{\CAP{TS}}) to all other caches and transitions the key to the Write state. 

% \item\textbf{C\textsubscript{\CAP{ACK}}}: Once the coordinator receives \CAP{ACK}s from all other caches, it checks if its local timestamp for the key is the same as that of the write (i.e., it has not being increased by another concurrent remote write). If the timestamp has remained the same, it applies the write in its local cache by updating the key's value and transitioning the key's state back to Valid.

\item\textbf{C\textsubscript{\CAP{ACK}}}: If the coordinator receives \CAP{ACK}s from all other caches, it has gotten exclusive access to the key and it can safely complete its write in its local cache by updating the key's value and transitioning the key's state back to Valid.
% At this point, the write is completed.
% , even if the new value was not actually applied locally 
% because another concurrent write with higher timestamp took precedence.
% because it got covered by another concurrent update.
% At this point, the write is completed --- regardless if it was actually applied (or not).
% The coordinator check
% , the write is completed.
% 
% , it can proceed by performing the write locally. is completed by transitioning the key to the Valid state (Invalid state if the key was in Trans state\footnote{The Trans state indicates a coordinator with a pending write that got invalidated. While not required, the Trans state is useful for tracking when the coordinator's original write completes, hence allowing the coordinator to notify the client of the write's completion.}).

\item\textbf{C\textsubscript{\CAP{VAL}}}: After completing the write locally, the coordinator broadcasts a \CAP{VAL} message consisting of the key, the same timestamp and the new value to all the followers. 

% If it did not apply it locally, then another concurrent write with higher timestamp took precedence and the coordinator does not need to broadcast its write's value.
% \item\textbf{C\textsubscript{\CAP{VAL}}}: Finally, if the coordinator applied the write locally it broadcasts a \CAP{VAL} message consisting of the key and the same timestamp to all the followers. If it did not apply it locally, then another concurrent write with higher timestamp took precedence and the coordinator does not need to broadcast its write's value.
\end{itemize}

\vspace{10pt}
\centerline{\underline{Follower}}
\vspace{-20pt}
\begin{itemize}[leftmargin=*]
\item\textbf{F\textsubscript{\CAP{INV}}}: Upon receiving an \CAP{INV} message, a follower compares the timestamp from the incoming message to its local timestamp of the key.
If the received timestamp is lower than the local timestamp, the follower simply ignores the message. Otherwise,
% If the received timestamp is higher than the local timestamp, 
the follower \textit{applies} the \CAP{INV} to its local cache by transitioning the key to the Invalid state and updating the key's local timestamp (both its \VAR{version} and \cid).

If prior applying the \CAP{INV} the key was in Write state locally, 
% If the local state of the key before applying the INV was Write state,
the follower retries its write (with a new timestamp) once its local cache gets back into Valid state.

\item \textbf{F\textsubscript{\CAP{ACK}}}: After applying an \CAP{INV}
% was applied 
% Irrespective of the result of the timestamp comparison, 
a follower responds to the coordinator with an \CAP{ACK} containing the same timestamp as that in the \CAP{INV} message of the write. 
% \todo{Not if an RMW.}
% \item \textbf{F\textsubscript{\CAP{ACK}}}: Irrespective of the result of the timestamp comparison, a follower always responds with an \CAP{ACK} containing the same timestamp as that in the \CAP{INV} message of the write. \todo{Not if an RMW.}

\item \textbf{F\textsubscript{\CAP{VAL}}}: When a follower receives a \CAP{VAL} message, it transitions the key to the Valid state and updates the key's local value with that from the message if and only if the received timestamp is equal to the key's local timestamp. Otherwise, the \CAP{VAL} message is simply ignored. 
\end{itemize}

% \noindent \underline{Verification.} 
\beginfsec{Formal verification} 
% \todo{Update the TLA spec}
%\hl{
% The Lin protocol has one stable state and two transient states, making it more complex than the SC protocol, which has only one stable state and no transient states and has been formally shown to be correct by Burckhardt~\cite{Burckhardt:2014}. Therefore, we wanted to formally verify the Lin protocol. To this end, 
We have expressed Galene in \tla\cite{Lamport:1994} and verified it for safety and the absence of deadlocks. For safety, we verified two invariants. First, the \emph{single-writer-multiple-reader} invariant (\CAP{SWMR})~\cite{Vijay:20}: at any given time there can be at most one writer that can update an object (multiple readers can safely read an object). Second, the \emph{data value invariant}: if an object is in a valid state (that can be read), then it must hold the most recent value that was written to that object. Our \tla model allows for the number of caches, and the number of total writes to be configured. We have verified with up to 5 processors and 3 writes. A detailed state transition table as well as the \tla specification are available online.\footnote{ 
\label{footC:link}\href{http://s.a-phd.com}{http://s.a-phd.com}} 

% \beginbsec{Optimizations} \todo{In Hermes this is a subsection}
\tsubsection{Optimizations}
% \begin{description}

\noindent\textbf{[O\textsubscript{1}] \textit{Request coalescing}} \hspace{2pt} Concurrent \CAP{RMW}s and writes to the same key () by a thread can be coalesced and executed once the block has been acquired into exclusive mode
\todo{finish}
% \item[O\textsubscript{1}]\textbf{\hspace{-5pt}]} \textbf{Virtual node ids}


\noindent\textbf{[O\textsubscript{2}] \textit{Enhancing fairness}} \hspace{2pt} 
% Similarly to Galane, Hermes can utilize virtual node ids to facilitate fairness in the order of concurrent writes to the same key from different replicas. 
Galene linearizes writes based on their unique timestamps, consisting of a version and a node id.
% (\textbf{C\textsubscript{\CAP{TS}}}). 
In case of same versions (i.e., concurrent writes), the linearization is resolved based on the node ids, which might raise concerns about fairness. 
% Although we do not expect this be a major issue, it 
This is easily mitigated by assigning several \textit{virtual node ids} to each physical node. With this scheme, before issuing a write, a node randomly picks one of its assigned virtual node ids to be used for the write's logical timestamp. Of course, to maintain correctness, the same virtual node id cannot be assigned to more than one physical node. 
%Last but not least, we note that the number and selection of virtual node ids can increase the fairness accordingly. 
For example, given three nodes (\textit{A, B, and C}), the following sets of virtual ids \textit{A}: $\{$1, 4, 7, 10$\}$, \textit{B}: $\{$2, 5, 8, 11$\}$, and \textit{C}: $\{$3, 6, 9, 12$\}$ are safe and would increase fairness. 

% \end{description}

\begin{comment}
\vspace{10pt}
\centerline{\underline{RMWs}}
\vspace{-10pt}
Unlike writes, a coordinator may not be able to complete a read-modify-write (\CAP{RMW}) if it was concurrent with other updates (writes or RMWs). Intuitively, this is because the final value of an RMW depends on the previous value of the key, and these values can be determined by other concurrent write operations (with smaller timestamps). 
% The easiest way to support RMWs in our scheme is by simply detecting that
% 
Below we demonstrate the smallest changes to our scheme to safely support RMWs:
% \footnote{
% Note that with a more complex protocol we could allow for all concurrent RMWs to complete without retries. Simply if an INV refering to an RMW is applied by a node who was previously in Write state then that follower piggybacks its update (RMW or write) to be executed by that coordinator

% All must keep their pending write and its ts even if overwritten. Because they might have to communicate it even if they they have transitioned into Invalid state from another node.
% If an RMW comes they piggybacks their ts and write to the coordinator

% This would need every node to communicate its indented update (write or RMW) to any coordinator of an INV with 
% (i.e., by having each communicating all dependent RMWs to all caches). We deliberately chose not to do so to avoid having those but this would mandate communicating all RMW
% }.
\begin{itemize}[leftmargin=*]
\item \textbf{C\textsubscript{\CAP{INV}}}: An extra bit is included with the \CAP{INV} indicating that it refers to an \CAP{RMW}.

\item\textbf{F\textsubscript{\CAP{INV}}}: 
A follower that applies an \CAP{INV} (that has a higher timestamp) locally and is coordinating an \CAP{RMW}, it retries its \CAP{RMW} with a new timestamp once its local cache gets back into Valid state.

\item \textbf{F\textsubscript{\CAP{ACK}}}: Unlike an \CAP{INV} for a write which is always acknowledged, an \CAP{INV} referring to an \CAP{RMW} 

is only acknowledged if and only if it got applied by the follower (i.e., the timestamp in the message was higher than the local timestamp of the follower).

\end{itemize}

\end{comment}

==> Text/1-ccKVS/Miscellaneous/Fig_consistency_example_1.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/Lin-violation.pdf}
  \caption{Session B seeing the old value is a violation of Lin, but not SC.}
  \label{figC:consistency-example-1}
\end{figure}


==> Text/1-ccKVS/Miscellaneous/Fig_consistency_example_2.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/SC-violation.pdf}
  \caption{Sessions B and C do not agree on the order of writes and hence this is a SC violation (also a Lin violation).} 
  \label{figC:consistency-example-2}
\end{figure}


==> Text/1-ccKVS/Opportunity.tex <==
\subsection{Opportunity Analysis}
\label{secC:opportunity}

\boris{Should this be here or in Motivation?}
\vasilis{It was very challenging to analyze the opportunity, if we do not explain how symmetric caching works, i.e. black box, caches,life of a request}


To analyze the opportunity of Symmetric Caching, we investigate what is the maximum theoretical speed-up that can be achieved with this technique. Firstly we assume a black box architecture similar to RackOut, where the maximum throughput can be achieved under a uniform distribution.
%: the clients request data item from any server of the KVS independently of whether that server is the home owner of the requested data items.
%If a server is not the owner of the requested data, it in turn issues a request to the server which owns the data over RDMA network. Therefore each server in the KVS both issues and responds to requests. 
In this setup we will compare the performance of a baseline black box system when the access pattern is uniform and the same system with Symmetric Caching when the access pattern is Zipfian. 
\arpit{Should we briefly explain somewhere why is uniform distribution (the baseline) the best case scenario for the current state of the art.}\vasilis{The background section on RackOut explains this now}

In the baseline system caching would have no effect, since all data items are equally popular; the system is totally load-balanced and thus each server can service a fixed number of requests every second, that is ultimately limited by the hardware of the system (i.e. it can be CPU bound or Network Bandwidth bound).

%The first hypothesis of our analysis is that the  baseline system with no caching but with a uniform pattern access is botllenecked by the available network bandwidth. Under this assumption the maximum throughput in that system is achieved, without fully utilizing the CPU capabilities of the servers. Either not all cores are used or the cores are spending most of the time busy looping waiting for the requests.% 

In the caching system, if we assume a zipfian distribution with exponent $a=0.99$ and a software cache that stores the 0.1\% hottest data items of the workload, then 65\% of the total requests will be cache hits, according to Figure \ref{figC:caching}. The rest 35\% of the accesses are requests to cold objects, each of which needs to be propagated to the appropriate remote server within the KVS. The throughput at which the cold requests can be serviced is capped by the throughput of one server in the baseline system. Therefore, in our example the upper bound of the throughput that the caching server can achieve is 2.85 \footnote{$100/35 =2.85$} times the throughput of the baseline server. 

To achieve this upper-bound, two hypotheses must hold true: 
\begin{enumerate}
    \item The baseline system must be bottlenecked by the \antonis{internal} network. More precisely the baseline must under-utilize the CPU enough, such that accessing the hot items in the cache will be essentially free
    \item The accesses to the cold items that miss in the cache must follow a distribution that is close to the uniform
\end{enumerate}

Our evaluation proves both hypotheses. More precisely, we build ccKVS: a black box, RDMA-based KVS with Symmetric Caching that achieves 2.85x in throughput in comparison to a black box baseline under uniform distribution.
% 

==> Text/1-ccKVS/break-even-write-ratio.tex <==
\subsubsection{When does Symmetric Caching break even?}  

%When applying Symmetric Caching, each write to a hot item generates consistency traffic. inside the black box. 
%Therefore, an increase in the write ratio results in an increase in consistency traffic, which leads to a decrease in the rate at which cache misses are handled. As discussed, the performance of ccKVS is determined by the rate at which it can serve the cache misses and therefore, a decrease in that rate can be directly correlated to the maximum performance that the system can achieve. 


Our primary goal is to answer this question: for a deployment of X servers what is the write ratio at which the ccKVS yields the same throughput as Uniform.
We call this write ratio the \textit{break-even write ratio}. Figure~\ref{figC:break-even} illustrates the break-even write ratio for a ccKVS-SC and ccKVS-Lin deployment of up to 40 servers. For example, a ccKVS-SC deployment with 20 servers will yield the same performance as Uniform at a write ratio of $8\%$. As expected the break-even write ratios of ccKVS-LIN are consistently lower than ccKVS-SC. The reason behind this is that a write in ccKVS-Lin translates into more consistency messages, because LIN requires a two-phase protocol that contains a round of invalidations and acknowledgements before the update.

Additionally we note that, as the number of servers increases the break-even write ratio decreases in both consistency models. The reason this happens is because the consistency traffic increases linearly with the number of servers, since a write to a hot object must be propagated to all servers. With 40 servers the break-even write ratio is almost $4\%$ for ccKVS-SC and $1.7\%$ for ccKVS-Lin. This indicates that in a moderately sized deployment ccKVS outperforms the baseline for moderate write ratios, while maintaining strong consistency guarantees.\vasilis{it may be good to add that this study is independent of the skew}


\begin{comment}

As discussed in Section~\ref{secC:write-perf}, the throughput of ccKVS is proportional to the proportion of data traffic in the network. 
Using this correlation, we build an analytical model that computes the throughput as the proportion of data traffic to the
%decrease in the rate at which cache misses can be serviced, 
consistency traffic changes, for both ccKVS-SC and ccKVS-Lin. 
Our primary goal is to answer this question: for a deployment of X servers what is the write ratio at which the ccKVS yields the same throughput as Uniform.
We call this write ratio the \textit{break-even write ratio}. Figure~\ref{figC:break-even} illustrates the break-even write ratio for a ccKVS-SC and ccKVS-Lin deployment of up to 40 servers. For example, a ccKVS-SC deployment with 20 servers will yield the same performance as Uniform at a write ratio of $8\%$. As expected the break-even write ratios of ccKVS-LIN are consistently lower than ccKVS-SC. The reason behind this is that a write in ccKVS-Lin translates into more consistency messages, because per-key Linearizability requires a two-phase protocol that contains a round of invalidations and acknowledgements before the update.

Additionally we note that, as the number of servers increases the break-even write ratio decreases in both consistency models. The reason this happens is because the consistency traffic increases linearly with the number of servers, since a write to a hot object must be propagated to all servers. With 40 servers the break-even write ratio is almost $4\%$ for ccKVS-SC and $1.7\%$ for ccKVS-Lin. This indicates that in a moderately sized deployment ccKVS outperforms the baseline for moderate write ratios, while maintaining strong consistency guarantees.\vasilis{it may be good to add that this study is independent of the skew}

\end{comment}

%We note that the break-even write ratio per-key SC decreases as the value size increases, because the consistency consists of solely big messages(i.e. broadcasts). In contrast the break-even write ratio increases with per-key Linearizability when the value size increases, because in that case 2/3 of the consistency traffic is small messages (i.e. acknowledgements and invalidations).
\begin{comment}


\\
The parameters are: \\
\textit{N}: Number of Servers\\
\textit{wr}: Write Ratio\\
%f : cache hit ratio\\
Payloads:\\
\textit{Big}: Big message in Bytes (i.e. read reply, or write request)\\
\textit{Sm}: Small message in Bytes (i.e. read request, or write reply)\\
\textit{Avg}: Average of small and big messages in Bytes\\
\textit{HO}: Header only in Bytes (i.e. the credit message has no payload)\\
\textit{CD}: Credit Divider (i.e. how many credits in a credit update message)\\ 
\\
\end{comment}


\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|}  \hline
\multirow{1}{2em}{\textit{N}} & Number of Servers \\  \hline
\multirow{1}{2em}{\textit{Wr}}  & Write Ratio \\  \hline
\multirow{2}{2em}{\textit{Big}} & Big message in Bytes \\ & (read reply, or write request) \\  \hline
\multirow{2}{2em}{\textit{Sm}}  & Small message in Bytes \\  & (read request, or write reply)\\ \hline
\multirow{2}{2em}{\textit{Cub}}  & Credit Update Batch \\  & (credits in a credit update message)\\  \hline
\multirow{1}{2em}{\textit{Avg}}  & Average of Sm and Big \\  \hline
\multirow{1}{2em}{\textit{Ho}}  & Header only in Bytes \\ \hline
\end{tabular}
\caption{Parameters of the break-even write-ratio }
\end{center}
\end{table}



EC break-even write ratio : 
\begin{equation}
\label{eqC:EC_break_even}
 WR = \frac{Avg(1 - \frac{1}{N})} {(N - 1)(Big + (Ho/Cub))}
\end{equation}
\vasilis{TODO: Antonis will double check these, if we end up using them}
\\SC break-even write ratio :
\begin{equation}
\label{eqC:SC_break_even}
 WR = \frac{Avg(1 - \frac{1}{N})}{(N - 1)(Big + 2Sm + 3(Ho/Cub))}
\end{equation}
\begin{comment}

It is worth noting that the cache hit ratio is factored out of this equation. In other words the break-even write ratio is solely a function of the number of servers and the payloads and it is completely independent of the cache hit ratio. 


It is worth highlighting that the break-even write ratio refers to the point where Symmetric Caching breaks even with a baseline with uniform distribution. Therefore, even when the write ratio is at its break-even point, Symmetric Caching will yield better performance than no caching. 

%DEFEND THE SIZE OF THE BLACK BOX
Figure \ref{figC:break-even} shows the break-even write ratio of a black box with Symmetric caching varying the size of the black box from 5 up to 40 servers. There is no hard constraint on the size of the black box, rather each application can choose a different size according to its write ratio \antonis{and skew(?)} . For example, a KVS that fits in 80 servers can be split into 8 10-server black boxes or 4 20-server black boxes, depending on the write ratio. However, the popularity cache only stores data items that belong to the black box and thus, breaking up the KVS into multiple black boxes will have an effect on the hit ratio of the popularity caches. For a complete study on how the skew varies when decreasing the size of the black box we refer the reader to \cite{RNovakovic:2016}.
\end{comment}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/break_even_performance_study.pdf} 
  \caption{Break-even write-rate study. [$\alpha=0.99$]}
  \label{figC:break-even}
\end{figure}

==> Text/2-Lara/chapter.tex <==
\esquote{30}{Everything not saved will be lost.}{Nintendo "quit screen"}
\markedchapter{The LAW of Fault Tolerance}{The LAW of Fault Tolerance:\nextlinepdf Linearizable Local Reads \& Asynchrony}
\label{chap:lara}

\section{}
\subsection{Subsection first}
\subsection{Subsection second}
\section{Section second}

% \cref{tab:eval} below summarizes the read and write features of the evaluated systems.
% \input{Visuals/Tables/eval-table1.tex}

==> Text/3-Hermes/0_abstract.tex <==
\begin{abstract}
Today's datacenter applications are underpinned by datastores that are responsible for providing availability, consistency, and performance. For high availability in the presence of failures, these datastores replicate data across several nodes. This is accomplished with the help of a \emph{reliable replication protocol} that is responsible for maintaining the replicas strongly-consistent even when faults occur. Strong consistency is preferred to weaker consistency models that cannot guarantee an intuitive behavior for the clients. Furthermore, to accommodate high demand at real-time latencies, datastores must deliver high throughput and low latency. 


This work introduces Hermes\footnote{The name is inspired by the immortal Olympian figure, who was the messenger of the gods and a conductor of souls into the afterlife.}, a broadcast-based reliable replication protocol for in-memory datastores that provides both high throughput and low latency by enabling local reads and fully-concurrent fast writes at all replicas. Hermes couples \emph{logical timestamps} with cache-coherence-inspired \emph{invalidations} to guarantee linearizability,  avoid write serialization at a centralized ordering point, resolve write conflicts locally at each replica (hence ensuring that writes never abort) and provide fault-tolerance via replayable writes. Our implementation of Hermes over an \CAP{RDMA}-enabled reliable datastore with five replicas shows that Hermes consistently achieves higher throughput than state-of-the-art \CAP{RDMA}-based reliable protocols (\CAP{ZAB} and \CAP{CRAQ}) across all write ratios while also significantly reducing tail latency. At 5\% writes, the tail latency of Hermes is 3.6$\times$ lower than that of \CAP{CRAQ} and \CAP{ZAB}.
\end{abstract}

%%%% Abstract w/o Latex commands
% Today's datacenter applications are underpinned by datastores that are responsible for providing availability, consistency, and performance. For high availability in the presence of failures, these datastores replicate data across several nodes. This is accomplished with the help of a reliable replication protocol that is responsible for maintaining the replicas strongly-consistent even when faults occur. Strong consistency is preferred to weaker consistency models that cannot guarantee an intuitive behavior for the clients. Furthermore, to accommodate high demand at real-time latencies, datastores must deliver high throughput and low latency. 

% This work introduces Hermes, a broadcast-based reliable replication protocol for in-memory datastores that provides both high throughput and low latency by enabling local reads and fully-concurrent fast writes at all replicas. Hermes couples logical timestamps with cache-coherence-inspired invalidations to guarantee linearizability, avoid write serialization at a centralized ordering point, resolve write conflicts locally at each replica (hence ensuring that writes never abort) and provide fault-tolerance via replayable writes. Our implementation of Hermes over an RDMA-enabled reliable datastore with five replicas shows that Hermes consistently achieves higher throughput than state-of-the-art RDMA-based reliable protocols (ZAB and CRAQ) across all write ratios while also significantly reducing tail latency. At 5% writes, the tail latency of Hermes is 3.6X lower than that of CRAQ and ZAB.

==> Text/3-Hermes/3_misc/Evaluation-Table.tex <==

\begin{table}[h]
\centering

\begin{adjustbox}{max width=0.47\textwidth}

\begin{tikzpicture}

\node (table) [inner sep=-0pt] {
\begin{tabular}{l|c|c|c|c|c}
\rowcolor[HTML]{9B9B9B} 
\cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Local reads}} & \multicolumn{3}{c}{\cellcolor[HTML]{9B9B9B}\textbf{Writes}} \\ \cline{2-6} 
\rowcolor[HTML]{9B9B9B} 
\multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{System}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Consistency} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency (RTT) & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}Dec.} \\
\textbf{HermesKV} & one per RM & Lin & inter-key & 1 & \cmark \\
\textbf{rCRAQ} & one per RM & Lin & inter-key & O(\textit{n}) & \xmark \\
\textbf{rZAB} & none & SC & serializes all & 2 $\dagger$ & \xmark \\
\textbf{Derecho} & none & SC & serializes all & 1 $\ddagger$ & \cmark
\end{tabular}
};
\draw [rounded corners=.3em] (table.north west) rectangle (table.south east);

\end{tikzpicture}

\end{adjustbox}


\caption{
Comparison of read and write features for the evaluated systems. 
% Write concurrency and local reads lease usage and consistency for evaluated systems.
SC: sequentially consistent; RM: reliable membership; Dec: decentralized; \textit{n}: number of replicas; $\dagger$1 RTT for master's writes; $\ddagger$lock-step commit.}
% Protocols that provide SC cannot be deployed per-key since SC is not composable.}
\label{tabH:eval}
\end{table}

==> Text/3-Hermes/4_incl_graphics/eval-latency.tex <==

\begin{figure*}[t]
%%%%%%% Uniform Figure %%%%%%%%%
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{Graphs/write_rate_latency_study_uniform_out.pdf}
  \captionsetup{font=Big, width=0.85\linewidth}
  \caption{Uniform}
  \label{figH:latency-uni}
  \end{subfigure}%
%%%%%%% Skew Figure %%%%%%%%%
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{Graphs/write_rate_latency_study_skew_out.pdf}
  \captionsetup{font=big, width=0.85\linewidth}
  \caption{Skewed [Zipfian exponent 0.99]}
  \label{figH:latency-skew}
  \end{subfigure}
  \caption{Median and 99th\% latency while varying the write rate. [5 nodes]}
\end{figure*}

==> Text/3-Hermes/4_incl_graphics/eval-latency_xput.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Graphs/latency_vs_xPut_all_write_rate_5_line_plot.pdf} 
  \caption{Latency vs Throughput. [Uniform traffic, 5\% write ratio, 5 nodes]}
  \label{figH:latency}
\end{figure}

==> Text/3-Hermes/4_incl_graphics/eval-scalability.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Graphs/sclability_study_varying_write_rate_1_and_20_double_column.pdf} 
  \caption{Scalability study. [Uniform traffic] }
  \label{figH:scalability-line}
\end{figure}

==> Text/3-Hermes/4_incl_graphics/eval-table.tex <==
\begin{adjustbox}{max width=0.30\textwidth}

\begin{tikzpicture}
\centering
\node (table) [inner sep=-0pt] {
\begin{tabular}{l|l|l|l|l|c}
\rowcolor[HTML]{9B9B9B} 
\cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{local reads}} & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{writes}} \\ \cline{2-6} 
\rowcolor[HTML]{9B9B9B} 
\multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{systems}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Con.} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}DC} \\
\textbf{HermesKV} & single RM & Lin & inter-key & 1 RTT & \cmark \\
\textbf{rCRAQ} & single RM & Lin & inter-key & O(\textit{n}) & \xmark \\
\textbf{rZAB} & no need & SC & serializes all & 1.5 RTT & \xmark \\
\textbf{Derecho} & no need & SC & lock-step apply & 1.5 RTT & \cmark
\end{tabular}

};
\draw [rounded corners=.3em] (table.north west) rectangle (table.south east);

\end{tikzpicture}

\end{adjustbox}

\caption{
Leases and consistency (Con.) for local reads and write features of evaluated systems. 
% Write concurrency and local reads lease usage and consistency for evaluated systems.
SC is sequentially consistent, DC is decentralized, \textit{n} is number of replicas.
}
\label{tabH:eval}

==> Text/3-Hermes/4_incl_graphics/eval-triple-async.tex <==
\begin{figure*}[t]
\setkeys{Gin}{width=1.05\linewidth}
\begin{tabularx}{\linewidth}{XXX}
\includegraphics{Text/3-Hermes/1_figures/hermes_async.pdf}
\caption{Hermes vs. Hermes-async throughput [5 replicas, varying write ratio].}
\label{figCA:hermes_xput}

&
\includegraphics{Text/3-Hermes/1_figures/hermes_latency.pdf}
\caption{Hermes vs. Hermes-async latency [5 replicas, 2\% write ratio, varying load].}
\label{figCA:hermes_latency}

% &
% \includegraphics[width=0.325\textwidth]{Text/3-Hermes/1_figures/hermes_scalability.pdf}
% \caption{Hermes vs. Hermes-async scalability [2\% and 10\% write ratio, varying number of replicas].}
% \label{figCA:hermes_scale}
\end{tabularx}
\end{figure*}

==> Text/3-Hermes/4_incl_graphics/eval-triple-irrelevant.tex <==
% \begin{figure*}[t]
% \setkeys{Gin}{width=1\linewidth}
% \begin{tabularx}{\linewidth}{XXX}
% \includegraphics{Text/3-Hermes/2_graphs/sclability_study_varying_write_rate_1_and_20_double_column.pdf}
% \caption{Scalability study. [Uniform traffic] }
% \label{figH:scalability-line}
% &
% \includegraphics{Text/3-Hermes/2_graphs/derecho_comparison.pdf}
% \caption{Comparison to Derecho. [Uniform traffic, 5 nodes, write-only]}
% \label{figH:derecho}
% &
% \input{Text/3-Hermes/3_misc/Eval-failure.tex}
% \caption{HermesKV under failure. [Uniform traffic, 5 nodes, timeout=150ms]}
% \label{figH:failure-throughput}
% \end{tabularx}
% \end{figure*}


\begin{figure*}[t]
\setkeys{Gin}{width=1\linewidth}
\begin{tabularx}{\linewidth}{XXX}
% \includegraphics{Text/3-Hermes/2_graphs/sclability_study_varying_write_rate_1_and_20_double_column.pdf}
% \caption{Scalability study. [Uniform traffic] }
% \label{figH:scalability-line}
% &
\includegraphics{Text/3-Hermes/2_graphs/derecho_comparison.pdf}
\caption{Comparison to Derecho. [Uniform traffic, 5 nodes, write-only]}
\label{figH:derecho}
&
\input{Text/3-Hermes/3_misc/Eval-failure.tex}
\caption{HermesKV under failure. [Uniform traffic, 5 nodes, timeout=150ms]}
\label{figH:failure-throughput}
\end{tabularx}
\end{figure*}

==> Text/3-Hermes/4_incl_graphics/eval-write_only.tex <==
\begin{figure}[t]
  \input{Miscellaneous/Eval-write-only.tex}
  \caption{Write-only study. [Uniform traffic, 5 nodes] }
  \label{figH:write-only}
\end{figure}

==> Text/3-Hermes/4_incl_graphics/eval-xput-RMWs.tex <==
\begin{figure}[t]
%%%%%%% Uniform Figure %%%%%%%%%
%   \hspace{30pt}
  \centering
%   \begin{subfigure}[b]{0.72\textwidth}
  \includegraphics[width=0.70\textwidth]{Text/3-Hermes/2_graphs/write_rate_RMW_performance_study.pdf}
  \caption{Hermes writes vs. RMWs throughput while varying update ratio ($1\%$ to $100\%$). [uniform accesses, 5 nodes]\todo{remove -KV suffix from label, change color and markers to march next graph}}
  \label{figH:write-rate-RMW}
\end{figure}

==> Text/3-Hermes/4_incl_graphics/eval-xput-n-table.tex <==
% \begin{figure*}[t]
%   \begin{subfigure}[b]{0.20\textwidth}
  
%     \begin{adjustbox}{max width=0.99\textwidth}

%     \begin{tikzpicture}
%     \node (table) [inner sep=-0pt] {
%     \begin{tabular}{l|l|l|l|l|c}
%     \rowcolor[HTML]{9B9B9B} 
%     \cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{local reads}} & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{writes}} \\ \cline{2-6} 
%     \rowcolor[HTML]{9B9B9B} 
%     \multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{systems}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Con.} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}DC} \\
%     \textbf{HermesKV} & single RM & Lin & inter-key & 1 RTT & \cmark \\
%     \textbf{rCRAQ} & single RM & Lin & inter-key & O(\textit{n}) & \xmark \\
%     \textbf{rZAB} & no need & SC & serializes all & 1.5 RTT & \xmark \\
%     \textbf{Derecho} & no need & SC & lock-step apply & 1.5 RTT & \cmark
%     \end{tabular}
%     };
%     \draw [rounded corners=.3em] (table.north west) rectangle (table.south east);
%     % \caption{Leases and consistency (Con.) for local reads and write features of evaluated systems. 
%     % % Write concurrency and local reads lease usage and consistency for evaluated systems.
%     % SC is sequentially consistent, DC is decentralized, \textit{n} is number of replicas.}
%     % \label{tab:eval}
%     \end{tikzpicture}
%     \end{adjustbox}
%     % \captionsetup{width=0.85\linewidth}
%     \vspace{-0.25em}
    

%   \end{subfigure}
  
%   %
%   \begin{subfigure}[b]{0.32\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
%     \vspace{-0.9em}
%     \caption{Uniform}
%     \label{figH:write-rate}
%   \end{subfigure}
%   %
%   \begin{subfigure}[b]{0.32\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{2_graphs/skew_99_and_write_rate_performance_study.pdf}
%     \vspace{-0.9em}
%     \caption{Skewed [Zipfian exponent 0.99]}
%     \label{figH:skew-line}
%   \end{subfigure}
%     \vspace{-0.75em}
%   \caption{Throughput for $1\%$ to $100\%$ write ratio. [5 nodes]}
%   \vspace{-15pt}
% %   \vspace{-2.5em}
% %   \caption{Latency analysis. [5 nodes] }
% %   \vspace{-10pt}
% \end{figure*}



% \begin{figure*}[t]
% \setkeys{Gin}{width=1.05\linewidth}
% \begin{tabularx}{\linewidth}{XXX}
%     \begin{adjustbox}{max width=0.33\textwidth}
%     \begin{tikzpicture}
%     \node (table) [inner sep=-0pt] {
%     \begin{tabular}{l|l|l|l|l|c}
%     \rowcolor[HTML]{9B9B9B} 
%     \cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{local reads}} & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{writes}} \\ \cline{2-6} 
%     \rowcolor[HTML]{9B9B9B} 
%     \multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{systems}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Con.} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}DC} \\
%     \textbf{HermesKV} & single RM & Lin & inter-key & 1 RTT & \cmark \\
%     \textbf{rCRAQ} & single RM & Lin & inter-key & O(\textit{n}) & \xmark \\
%     \textbf{rZAB} & no need & SC & serializes all & 1.5 RTT & \xmark \\
%     \textbf{Derecho} & no need & SC & lock-step apply & 1.5 RTT & \cmark
%     \end{tabular}
%     };
%     \draw [rounded corners=.3em] (table.north west) rectangle (table.south east);
   
%     \end{tikzpicture}
%     \end{adjustbox}
%      \caption{Leases and consistency (Con.) for local reads and write features of evaluated systems. 
%     % Write concurrency and local reads lease usage and consistency for evaluated systems.
%     SC is sequentially consistent, DC is decentralized, \textit{n} is number of replicas.}
%     \label{tabH:eval}
% &
%     \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
%     \vspace{-0.9em}
%     \caption{Uniform}
%     \label{figH:write-rate}
% &
%     \includegraphics[width=0.9\linewidth]{2_graphs/skew_99_and_write_rate_performance_study.pdf}
%     \vspace{-0.9em}
%     \caption{Skewed [Zipfian exponent 0.99]}
%     \label{fig:skew-line}
% \end{tabularx}
% \vspace{-20pt}
% \end{figure*}

==> Text/3-Hermes/4_incl_graphics/eval-xput-triple.tex <==
\begin{figure*}[t]
\setkeys{Gin}{width=1.05\linewidth}
\begin{tabularx}{\linewidth}{XXX}
    % \begin{adjustbox}{max width=0.33\textwidth}
    
    \input{3_misc/Evaluation-Table.tex}
    % \input{4_incl_graphics/eval-table.tex}
    
&
    \input{4_incl_graphics/eval-xput.tex}
% 
 \end{tabularx}
\end{figure*}

==> Text/4-Zeus/0_abstract.tex <==
\begin{abstract}

State-of-the-art distributed in-memory datastores (FaRM, FaSST, DrTM) provide strongly-consistent distributed transactions with high performance and availability. Transactions in those systems are fully general; they can atomically manipulate any set of objects in the store, regardless of their location. 
To achieve this, these systems use complex distributed transactional protocols. Meanwhile, many workloads have a high degree of locality. For such workloads, distributed transactions are an overkill as most operations only access objects located on the same server -- if sharded appropriately.

In this paper, we show that for these workloads, a single-node transactional protocol combined with dynamic object re-sharding and asynchronously pipelined replication can provide the same level of generality with better performance, simpler protocols, and lower developer effort. 
We present Zeus, an in-memory distributed datastore that provides general transactions by acquiring all objects involved in the transaction to the same server and executing a single-node transaction on them. Zeus is fault-tolerant and strongly-consistent. 
At the heart of Zeus is a reliable dynamic object sharding protocol that can move 250K objects per second per server,
allowing Zeus to process millions of transactions per second and outperform more traditional distributed transactions on a wide range of workloads that exhibit locality.
\end{abstract}

==> Text/4-Zeus/3_misc/Sharding-backup.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{l|cccc}
\multicolumn{1}{c|}{} & \multicolumn{1}{l}{\textbf{directory}} & \multicolumn{1}{l}{\textbf{owner}} & \multicolumn{1}{l}{\textbf{reader(s)}} & \multicolumn{1}{l}{\textbf{non-replica}} \\
\cline{2-5} 
data               &        & \cmark & \cmark &  \\
ownership metadata  & \cmark & \cmark &        &  \\
ownership levels & - & \textbf{w}/\textbf{r}    & \textbf{r}      & -                             
\end{tabular}
}
\mcaption{Nodes storing (meta)data and their access permissions.}
{Data and metadata stored by each node along with their read (r) and exclusive write (w) access permissions.}
\label{tabZ:shard_metadata}
\end{table}

==> Text/4-Zeus/3_misc/bech_table_backup.tex <==
\begin{table}[t!]
\centering
\resizebox{0.9\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{l|lrrrr}
 &
  \textbf{characteristic} &
  \multicolumn{1}{l}{\textbf{tables}} &
  \multicolumn{1}{l}{\textbf{columns}} &
  \multicolumn{1}{l}{\textbf{txs}} &
  \multicolumn{1}{l}{\textbf{read txs}} \\ \cline{2-6} 
\textbf{Handovers} & large contexts  & 5 & 36 & 4 & 0\%  \\
\textbf{Smallbank} & write-intensive & 3 & 6  & 6 & 15\% \\
\textbf{TATP}      & read-intensive  & 4 & 51 & 7 & 80\% \\
\textbf{Voters}    & popularity skew & 3 & 9  & 1 & 0\% 
\end{tabular}
}

\mscaption{Summary of evaluated benchmarks.}
\label{tabZ:bench}
\end{table}

==> Text/4-Zeus/4_incl_graphics/eval_sb_ho.tex <==
\begin{figure*}[ht]
\setkeys{Gin}{width=1.05\linewidth}

\begin{tabularx}{\linewidth}{XXX}
    \includegraphics{Text/4-Zeus/2_graphs/handovers_sharding.pdf}
    \caption{All-local (ideal) vs. Zeus for 2.5\% and 5\% handovers on 3 and 6 nodes.}
    \label{figZ:ho_total}
&
    \includegraphics{Text/4-Zeus/2_graphs/sb_locality.pdf}
    \caption{Smallbank while varying remote write transactions.}
    \label{figZ:eval_smallbank}
&
    \includegraphics{Text/4-Zeus/2_graphs/tatp_locality.pdf}
    \caption{\CAP{TATP} while varying remote write transactions.}
    \label{figZ:tatp_local}
\end{tabularx}

\end{figure*}


==> Text/4-Zeus/4_incl_graphics/eval_triple_vnf.tex <==
\begin{figure*}[ht]
\setkeys{Gin}{width=1.00\linewidth}

\begin{tabularx}{\linewidth}{XXX}

    \includegraphics{Text/4-Zeus/2_graphs/SPGW_throughput.pdf}
    \caption{Cellular packet gateway control plane performance.} 
    \label{figZ:spgw_thr}
&
    \includegraphics{Text/4-Zeus/2_graphs/SCTP_throughput.pdf}
    \caption{SCTP performance.}
    \label{figZ:sctp_thr}
&
    \includegraphics{Text/4-Zeus/2_graphs/Nginx_timeline.pdf}
    \caption{Nginx performance in a scale-in / scale-out scenario.}
    \label{figZ:nginx_time}
\end{tabularx}

\end{figure*}


==> Text/4-Zeus/4_incl_graphics/eval_voter_tatp.tex <==
\begin{figure*}[t]
\setkeys{Gin}{width=1.00\linewidth}

\begin{tabularx}{\linewidth}{XXX}

    \includegraphics{Text/4-Zeus/2_graphs/voter_moving_1m.pdf}
    \caption{Voter Performance when moving 1M objects across nodes.}
    \label{figZ:voter_mov_1}
&
    \includegraphics{Text/4-Zeus/2_graphs/voter_moving.pdf}
    \caption{Voter Performance when registering votes and moving objects.}
    \label{figZ:voter_mov_2}
&
    \includegraphics{Text/4-Zeus/2_graphs/cdf_latency.pdf}
    \caption{CDF of Zeus ownership request latency for Voter experiments.}
    \label{figZ:cdf}
\end{tabularx}

\end{figure*}


==> Text/4-Zeus/4_incl_graphics/fig_feature_sketch1.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.1\columnwidth]{Text/4-Zeus/1_figures/Feature-sketch.pdf}
  \caption{rVNF feature sketch.}
  \label{figZ:feature_sketch}
\end{figure}

==> Text/5-ccKVS-SC/1-Introduction.tex <==
\tsection{Overview}
\label{secC:intro}


Today's online services like search, e-commerce and social networking are underpinned by cavernous Key-value stores (KVS).
%satisfy user requests by serving data from a huge data set. Large scale data stores are the backbone of these online applications. 
Such KVS' must provide high throughput in order to serve millions of user requests simultaneously, while meeting 
%satisfyinf at low latency to meet  
online response time  requirements. 
%latency to serve millions of user requests simultaneously. 
In order to sustain these performance objectives, the dataset is typically maintained \emph{in memory} and is sharded across multiple servers using techniques such as consistent hashing~\cite{Karger:1997}.
%, by sharding the data across multiple servers using some form of consistent hashing. 

%In order to meet the high throughput requirements these systems are usually designed using memory resident distributed key-value stores (KVS) that shard data among individual servers by using some form of consistent hashing.

Although sharding data among individual servers enables massive parallelism, such a design can suffer from hot spots.  This is because the popularity distribution of objects is highly skewed, typically following power law distributions~\cite{Atikoglu:2012,Novakovic:2016,Huang:2014,Volos:2017}. In other words, in the presence of skew, the server(s) serving the most popular objects will become saturated, thus becoming a bottleneck and limiting the throughput of the entire KVS. 
%Indeed it has been shown that popularity distribution for data items for real-world large scale applications is skewed

The skew problem is well-established, and a number of techniques have been proposed to mitigate it. The techniques can be classified into two categories. 
%In the first, approaches like
%FASST~\cite{}, FaRM~\cite{Dragojevic:2014} and 
%State-of-the-art systems such as
The first class of techniques~\cite{Fan:2011,Li:2016,Jin:2017} uses a dedicated cache for storing popular keys to filter the skew.
The second class of techniques (FaRM~\cite{Dragojevic:2014} and RackOut~\cite{Novakovic:2016}) mitigate skew by evenly distributing read requests across all servers of the KVS regardless of the object's location.
%\vasilis{this is a very dangerous assessment, you would never get that idea from reading fasst or FaRM, they only use this notion because transactions request keys from multiple servers anyway}. 
For low latency, the servers use an RDMA-enabled interconnect to access objects that reside at other servers. 
%To enable this, they allow the servers of the KVS to serve objects sharded to other servers by communicating among themselves using an RDMA-enabled low latency interconnect. 
In essence, this class of techniques exposes a non-uniform memory access (NUMA) shared memory abstraction across the servers of the KVS.
%While these techniques successfully spread the CPU load, they are fundamentally network bound because the majority of requests require a remote access. 
%The second class of techniques~\cite{Fan:2011,Li:2016,Jin:2017} uses a dedicated cache for storing popular keys to filter the skew. 

The first approach is not scalable because the limited computational resources of a single cache node may not be able to keep up with the load. In contrast, the second approach is scalable in its processing capability, but is network bound because the vast majority of accesses is serviced by remote nodes.

%\vasilis{disagree with processing as the bottleneck}



In this paper, we view skew as an opportunity and leverage it to improve KVS performance. Taking inspiration from the effectiveness of caches in shared memory multiprocessors, we propose a \emph{Scale-Out ccNUMA} architecture which augments \emph{each} server node in a distributed KVS deployment with a small cache of hot items. Because item popularity is a function of the entire dataset and not of individual shards, all cache instances maintain an identical set of objects, which are the most popular objects in the dataset. Such a {\em symmetric cache} not only ensures a high hit rate, but also relieves the clients from knowing which caches maintain what objects, and avoids the need for costly metadata to track sharers on the KVS side.

%in the NUMA domain 
%with a small cache that  caches the same set of hot objects. 
%Thus our \emph{symmetric cache} can effectively filter out accesses to hot objects; in doing so, we not only avoid the negative effects of skew, we are actually able to leverage skew to increase throughout. Indeed,  because of the zipfian nature of skew, a small cache in every node is able to filter out more than half of the remote accesses.
%reduces the load on the server caching the hottest data while allowing the requests to  be evenly distributed across all servers of the KVS. 
%Moreover, it avoids the single cache bottleneck problem by maintaining a cache at each server. 
%All the servers in a NUMA domain are connected via a low latency RDMA-enabled interconnect to enable fast remote accesses.  

Replicating data in multiple caches raises the problem of ensuring consistency in the presence of writes. 
While \emph{eventually consistent}~\cite{Burckhardt:2014} systems are thought to be beneficial performance-wise, they are difficult to reason about and can cause unexpected behavior for both developers and users. Meanwhile, 
%The Eventual consistency encompasses a set of commonly used weak consistency models which are hard to reason about. 
stronger consistency models require all sharers to agree on the order of writes; some models even require writes to be performed synchronously. We ask the question of whether aggressive replication through caching of popular objects can be achieved with strong consistency guarantees {\em and} high throughput. 

%Can we enforce such strong guarantees while sustaining high throughput? 

%The protocols used in shared memory multiprocessors serialize at designated primaries (e.g. directories) which can become a bottleneck in the presence of skew. 
%world to enforce these guarantees serialize at a central point (say directory) which can become a bottleneck. 
%In this work we employ fully distributed protocols to enforce two strong consistency models: \emph{per-key sequential consistency} (SC), 
%which is the strongest form of eventual consistency and 
%and \emph{per-key linearizability} (Lin). 
%We also verify these protocols for correctness using a model checker.

To answer this question, we study non-blocking, fully distributed consistency protocols that leverage logical timestamps to achieve two strong consistency guarantees: \emph{per-key sequential consistency} (SC) and 
%which is the strongest form of eventual consistency and 
\emph{linearizability} (Lin).
%formally verifying the latter using a model checking tool. 
We then develop {\em ccKVS} -- a distributed RDMA-based KVS that 
%implements an instance of Scale-Out ccNUMA, 
employs a Scale-Out ccNUMA architecture, featuring symmetric caching with consistency guarantees enforced via the two protocols.
%\vasilis{removed the Skew-Aware Cocurrency control introduction here}
%To resolve the tension between between synchronization overhead and concurrency, ccKVS implements a novel \emph{Skew-aware Concurrency Control} mechanism that uses a CRCW model at the cache layer and an EREW for the KVS. 
 
 
%In this paper, we develop \emph{ccKVS}, an RDMA-based KVS that adopts out proposed scale-out ccNUMA architecture, by employing a symmetric cache in each node of the KVS. 
%We deploy non-blocking distributed consistency protocols that leverage Lamport timestamps to achieve two strong consistency guarantees: \emph{per-key sequential consistency} (SC) and which is the strongest form of eventual consistency and \emph{per-key linearizability} (Lin). 
%to leverages RDMA-enabled low latency interconnect for communication between its servers and deploys our distributed non-blocking protocols to enforce SC  and Lin.
%Furthermore, \emph{ccKVS} implements a novel \emph{Skew-aware Concurrency Control} mechanism that enhances throughput by resolving the tension between between synchronization overhead and concurrency.
%and a bunch of other optimizations including batching and thread partitioning to enhance the throughput of the KVS.

Our evaluation on a 9-node rack-based cluster shows that in comparison with a state-of-the-art KVS (Section~\ref{secC:method}), %\vijay{We should cite to the state of the art. If it is our own concoction then we must cite the section where we describe the state of the art.} 
\emph{ccKVS} achieves 
($2.2 \times$) $2.5 \times$ improvement in throughput for a workload with  $1\%$ writes while satisfying Lin (SC). 


%
%for a read-only workload and $2.2 \times$ improvement in throughput while guaranteeing strong consistency for a workload with $1\%$ writes, as compared to the state-of-the-art KVS \vasilis{compared to a similar shared-memory KVS without caching?}.
%
%\arpit{Should we use the term node or server uniformly, or is it fine to use them both?} yes!
%We build a symmetric cache on top of a KVS with shared memory abstraction similar to RackOut~\cite{Novakovic:2016}.
%
%
%data serving and what not
%Data serving is considered as one of the core utilities in a datacenter, as it constitutes the basic building block of many large scale applications such as e-commerce, social networking and electronic marketplaces\cite{DeCandia:2007, Atikoglu:2012,Bronson:2013}.
%such as services offered by Facebook, Amazon and Google\arpit{Not necessary to mention these applications}.
%Such applications, translate each user request into hundreds of smaller internal requests\cite{DeCandia:2007,Ousterhout:2011} to create on-demand personalized responses to their numerous users. As a result, the majority of requests that reach data serving systems refer to relatively small-sized objects\cite{Atikoglu:2012,DeCandia:2007}, while their traffic is commonly characterized as read-intensive\cite{Bronson:2013,DeCandia:2007}, e.g. Facebook reports that just 0.2\% of their traffic is writes. Consequently, these applications must store, process and serve tremendous amount of data, concurrently. Therefore, data serving systems require to offer high performance, while respecting tight latency guarantees aka service level objectives (SLOs) due to their user-facing nature.
%The users of these applications have integrated these services in their everyday lives, and they count on them to offer fast response times and large throughput.
%\arpit{rephrase the above sentence in terms of service level objectives (SLO). See rackout for reference}
%\antonis{I don't think that we should draw too much attention at SLOs since we do not focus on QoS/latency so much.}
%\arpit{I agree. We should not mention SLO or we should be very subtle about it.}
%The demands of these applications is that they must store, process and serve the data of millions (if not billions) of users, concurrently.  Consequently, these systems require very high performance and huge storage capacity~\arpit{Don't say storage and highlight that data needs to be kept in memory for performance reasons}.
%
%To satisfy those demands, data serving systems partition their dataset among multiple machines to increase storage capacity and serve independent requests in parallel. 
%However, even if  the dataset is evenly partitioned across the machines, the access patterns are skewed. More precisely, several studies have shown that real-world large-scale applications demonstrate data accesses that follow a power-law distribution\cite{Atikoglu:2012,Novakovic:2016,Huang:2014,Volos:2017}. In other words, just a few data items are responsible for most of the accesses.
%
%Naturally these goals are satisfied through large deployments that consist of multiple machines. The stored data is sharded among the nodes to achieve high capacity, while independent requests from different users can be served in parallel by different machines. 
%
%For over a decade, Key-Value Stores(KVS) has been the main paradigm  of high performance data serving systems [ref]. KVS is a distributed hash table that stores and accesses data using a unique key identifier assigned to each data item.  
%However, even if  the dataset were evenly partitioned across the machines, the data accesses are skewed. More precisely, several studies have shown that real-world large-scale applications demonstrate data access patterns that follow a power-law distribution[ref]. In other words just a few data items are responsible for most of the accesses.
%
%in-memory, RDMA, EREW
%For over a decade, distributed hash tables aka Key-Value Stores (KVS), is the main paradigm of high performance data serving systems\cite{DeCandia:2007,Su:2017}, where each object is stored and accessed using its unique key identifier. Commonly KVS designs employ numerous techniques to enhance performance. For instance all data resides in-memory to completely avoid the expensive disk accesses. Furthermore recent state-of-the-art systems leverage emerging networking features like RDMA[ref] to avoid inefficiencies of traditional TCP/IP \cite{Dragojevic:2014,Kalia:2014,Kalia:2016,Su:2017} and intelligent techniques such as fine grain partitioning\cite{Lim:2014}, to increase concurrency within a machine. 
%
% Approach 1st order
%
%Unfortunately most of these designs fail to address skew as an integral characteristic of the system. Instead the common wisdom is to deal with the skew as an afterthought, even though the skew is an inherent property of the workloads that greatly affects the performance of the system, if neglected. \arpit{Should we say instead: The common wisdom is to view skew as a problem and techniques have been proposed to minimize its performance impact [RackOut, SwitchKV,...]}
% Our perspective towards skew
%The common wisdom is to view skew as a problem and numerous techniques have been proposed to mitigate its performance impact\cite{RNovakovic:2016,Li:2016}. We take a radically different approach, we see skew as an opportunity to increase performance.
%\arpit{We should briefly highlight here our technique and also define all the terms that we use in contributions like black box abstraction, symmetric caching etc}
%\antonis{Since we have defined these things in bullets (that also provide a clear way of our contributions with references to their sections) I tried to avoid repeating these information here}
%\arpit{I think we should still introduce those things here because it helps with the flow. I view contribution bullets as a summary (so no new information) and as a means to highlight specific contributions.}
%\arpit{We should also mention the consistency challenge and our solution briefly}
%To accomplish this goal we adapt the approach of constructing data-serving systems that are constituted by groups (e.g. racks) of co-operative machines\cite{RNovakovic:2016}, where 
%load balance can be achieved since 
%each node is able to serve requests for every item that resides within its group.
%each node leverages efficient intra-group networking such as RDMA to serve requests for every item that resides within its group.
%, providing the notion and performance of scale-up nodes. 
%We enhance this load balancing design with \textit{Symmetric Caching}, a technique that combines the best of replication and caching. Finally, we efficiently solve the consistency problems that arise with writes, in the presence of replication.
%We build an RDMA-based KVS from the grounds up to tackle and leverage skew to greatly increase the throughput of the system. Our design exploits the skewed workload through \textit{symmetric caching} to achieve a throughput improvement of 2.85x using the most common exponent of skewed workloads: $a=0.99$ ~\arpit{We should not talk about exponents here.}. Furthermore we prove that the the benefit of the approach is independent of the implementation of the baseline. Rather, it solely depends on the skew exponent. 
%\sout{In summary, the  key contribution of the paper is Scale-Out ccNUMA, a new architecture which augments every server node of a KVS with a small strongly consistent cache. Specifically}:
%\boris{I found this redundant wrt both above and below. How about short and sweet:}


%For example HERD and MICA shard the KVS among the cores rather than the machines such that only a single core has permission to access a given data item. The net effect of this organization is that it eliminates concurrency control (locks etc). 

%However many of these approaches fail to consider that the access pattern is skewed rather than uniform, which means that a select, few, popular items make up for a big percentage of the total access patterns





==> Text/5-ccKVS-SC/1.5-Contributions.tex <==
\noindent In short, the main contributions of this chapter are as follows:

\squishlistContrib
    %Black Box
    %\item We built a black box abstraction of the KVS, such that the external clients can issue their requests to any server of the KVS. This way the request processing is load balanced among the servers of the KVS, the external clients can batch multiple requests for the entire KVS and they do not need to worry about locating the home server of the data item. The fast RDMA interconnect alleviates the overhead of the extra hop, that occurs when the KVS server that received a request is not the home server for that request.[section ref]
    %\antonis{Move this before contributions and rephrase by saying something like that our system provides the notion of scale-up data-serving nodes/islands}
    %being transparent to the clients and
    %combining the best attributes of traditional replication and caching, while
    %Symmetric Caching

    \item
    We introduce \textbf{\textit{Symmetric Caching}}: a novel and transparent caching strategy that replicates the most popular objects in all caches, thus enabling high throughput and load balance,
%    a novel  technique that couples the ideas of caching  and replication to offer load balance and reduce the number of extra hops, 
    while eliminating the costly requirement of tracking sharers. (Section~\textbf{\ref{secC:cache}})
    %by filtering a huge percentage of the accesses
    
  
    %we add a software cache in each server that stores the most popular data items of the KVS. All of the caches are identical and invisible to the external clients. 
    %The caches filter a huge percentage of the accesses, greatly increasing the throughput of each server 
    % Consistency
    \item In order to keep the caches consistent, we employ two \textbf{\textit{fully distributed protocols}} that equally spread the cost of consistency actions by enabling writes to be performed directly in any replica. The first of the protocols guarantees per-key Sequential Consistency; the second guarantees per-key Linearizability, which we verify for safety and deadlock freedom in \CAP{$TLA^{+}$}. (Section~\textbf{\ref{secC:protocols}})
    
    %Write requests to hot data items pose a consistency challenge: the caches need to be kept coherent. We developed fully distributed protocols and implement them efficiently over RDMA. One that guarantees per-key Sequential Consistency and one that guarantees per-key Linearizability.
    
    % Incremental Locking 
%    \item \vasilis{removed the skew-aware concurrency control bullet}%We introduce \textbf{\textit{Skew-aware Concurrency Control}} : a hybrid synchronization scheme which offers maximum concurrency for popular objects and synchronization-free processing for the long tail of the popularity distribution. 
    %where an object according to its popularity can be benefited either by the lack of synchronization overheads or by the concurrency offered by optimistic concurrency control methods. 

%the hot items are accessed with sequential locks that allow for lock-free reads and the cold items are accesses without any concurrency control. The KVs that serves the requests to the cold data items is partitioned at a core granularity, such that each cold data item has a home core instead of a home server, this way there is no need for concurrency control.
    % ccKVS KVS
    \item We build \textbf{\textit{ccKVS}}: an RDMA-based KVS that implements symmetric caching with our fully distributed protocols and achieves a throughput improvement of
 $2.2 \times$ ($2.5 \times$) over a state-of-the-art RDMA KVS for a workload with modest write ratios while satisfying Lin (per-key SC).
    %7x over the state-of-the-art RDMA KVS and 
    %up to 2.85x over the upper bound of state-of-the-art skew-mitigation techniques. 
    %in a read-only setting.
    %over the baseline. 
    (Section \textbf{\ref{secC:eval}})
    
\squishend


==> Text/5-ccKVS-SC/10-Related.tex <==
\tsection{Related Work} 
\label{secC:Related}

%There has been several works which are trying to alleviate the problem of skew. These techniques include caching, replication and 



%Although, most of the works assume that a cache resides on a more powerful component than the rest of the dataset, Symmetric caching is able to achieve this load balancing applied on a homogeneous set-up.
%
%is not the case with Symmetric Caching which is applied on homogeneous set up.

%proves the effectiveness of a small popularity cache, that can fit in the LLC of scale-up server acting as a load balancer.
%In-memory caches[] are usually used to filter skew on top of ssd/disk based designs. Some of them such as the SwitchKV \cite{Li:2016} provide efficient routing exploiting SDN switches.


%Such a design increases the required hops to serve a user request. Additionally, in the common case where the request traffic is huge, a single load balancer is a potential bottleneck, degrading system's performance, since it has receive and processes every request in the system. 

%Furthermore, Bronson et al.\cite{Bronson:2013} propose a design where a similar small cache resides on every client node, even though all cache hits have to be sent to the next layer in order to validate that the value is not stale. As a result, the response time of a request is not reduced and the skew is not filtered by the caches.\antonis{We need to confirm this!}

%Moreover, Li et. al. \cite{Li:2016} discuss a technique that leverages SDN switches 

%in order to efficiently route requests to the cache or the backend nodes

%Caching by itself is not an effective solution to skew if it is not applied on a more powerful machine/component than the original.

%Either on the network \cite{Li:2016,Liu:2017} or even in-memory key value stores\cite{Lim:2014,Kalia:2014}, which are usually used as a cache to filter skew on top of disk based deployments. However, caching by itself is not an effective solution to skew if it is not applied on a more powerful node or component than the original.

% Network

%However caching is vulnerable to hot-spots since 

%In fact, in-memory key value stores such as Memcache\cite{} usually operate as a cache of disk based / storage systems. There are several other works tha works [] that argue about. However, caching by itself is not an effective solution to skew if it is not applied on a more powerful machine/component than the original. 
\noindent{\bf Data replication} is often used by service providers to improve system performance, particularly due to load imbalance. While conceptually straight forward -- replicating hot data across some number of servers~\cite{Hong:2013,Huang:2014} %\boris{refs 31, 32 in Rack-Out} 
-- it comes with a number of practical shortcomings as detailed in~\cite{Novakovic:2016}. These include determining the appropriate level of replication granularity (object, partial shard or entire shard), tracking replicas, maintaining replicas consistent, and informing clients of the replica's locations. The latter can be particularly onerous if the number of clients is much greater than that of servers, which is often the case. In practice, these problems tend to have ad-hoc solutions requiring complex engineering and with significant system-level overheads, hence spurring the recent work on alternative approach using fast remote access and caching, as discussed in Section~\ref{secC:existing}. 

Our work takes the best features of replication, caching and fast remote access. Compared to traditional replication, our solution allows fine-granularity replication of individual keys and does not require client-side knowledge of replicas while affording strong consistency across all replicas.
%symmetric caching can be applied an approach where servers can be grouped similar to \cite{Novakovic:2016} can be used to form multiple symmetric caching groups. %,  can be used in conjunction with techniques proposed in this paper. 
%proposes an effective solution to these challenges in the form of symmetric caching, which allows fine-granularity replication and does not require client-side knowledge of replicas while affording strongly consistency across the caches. 


%

\vspace{0.04in}
\noindent{\bf Distributed Shared Memory (DSM)}. In principle, a distributed KVS is not all that different from a DSM~\cite{Stets:1997, Keleher:1994, Carter:1995, Li:1989}.
%\vijay{cite ivy, munin, treadmarks, cashmere}.
The underlying problem boils down to enforcing a consistency model in the presence of replication.  However, there is one important difference: the workloads. Whereas the goal of DSM is to support scalable parallel programs, the goal of KVS is to support data-serving workloads. Whereas the former is characterized by CPU-intensive programs that ideally do not spend all their time waiting for memory, the latter does little more than data accesses to main memory. 
%\sout{Whereas the former is a latency limited system, the latter is throughput limited.} \boris{That's crazy. If anything, I'd say a KVS is latency-limited while a batch parallel job is only throughput (IPC) limited. I think we should drop this point completely - it's highly disagreeable.}
Whereas locality in DSM is because of program working sets, locality in a KVS can be explained by a skewed access distribution. 
%\antonis{former and latter is used 3 times in a row and its difficult to make sense.} \boris{I agree, but if we drop the sentence I picked on, it gets a bit easier to parse.}

These workload differences and differences in sharing patterns translate into significant differences in the design of caches and the consistency protocols. Particularly, the popularity skew naturally dictates that only the popular items should be cached. Similarly, it dictates that there is no need to have different items in different caches, thus avoiding the need to track sharers (e.g., through a directory) or migrate pages. 
%\vasilis{We got the following comment on this: "The architecture proposed make sense not because of the skew, but because of the write ratio: parallel program intensively write memory, which explains why a write-through cache is inefficient for these applications."}
%For example, the symmetric nature of the skew motivates our symmetric cache, and because we are throughput limited we cannot afford the serialization bottlenecks in directory based protocols common in DSM world. 

%These differences greatly affects the design of ptackled byThe goal of software DSM  is to leverage fast networking to connect a bunch of clusters together and provide a software layer that presents a programmable shared memory abstraction. To ensure performance, they had to replicate data (especially read-only), and to ensure consistency they relied on software based coherence protocols. Thus, their goals were very similar to the goals of this work. 


%\boris{CAP, Latency theorem???}
%\antonis{I don't see CAP as related work. Except if you want to stress that we do not support/argue about failures.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COMMENTED OUT (old text on Caching and Replication)
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{0.04in}
\noindent{\bf Cache Coherence}. In shared memory multiprocessors, the local caches of each processor are typically kept coherent using hardware based coherence protocols~\cite{Vijay:20}. Our approach is inspired by the effectiveness of coherent caches in such architectures. 
%In fact, because the consistency guarantees we offer in this work are on a per-key basis
Furthermore, the per-key consistency guarantees we offer are similar to the per-memory location guarantees offered by coherence protocols.\footnote{The per-key linearizability guarantee is analogous to physical time SWMR and per-key sequential consistency is analogous to logical time SWMR~\cite{Vijay:20}} 
%which also offer consistency guarantees on a per-memory location basis.\footnote{The per-key linearizability guarantee is analogous to physical time SWMR and per-key sequential consistency is analogous to logical time SWMR~\cite{sorin2011primer}.} 
On the other hand, as discussed in Section~\ref{secC:case}, the protocols we employ (update based, full distributed) are very different from the ones typically employed in shared memory multiprocessors (invalidation based, serializing). 

\begin{comment}
\textbf{Caching}. Existing approaches are applying caching to filter the skew of the workload.
%, using various architectures and in several different locations between the clients and the servers.
More precisely, the work by Fan et. al. \cite{Fan:2011} talks about a cache that resides in the Last Level Cache (LLC) of a load balancer. Several other works \cite{Atikoglu:2012,Bronson:2013} provide various architectures where in-memory caches filter the skew of disk based systems, while a recent approach \cite{Li:2016} leverages SDN switches to achieve this efficiently. Finally, Jin et. al. \cite{Jin:2017} implement a novel key-value cache in a high-performance switch to filter the skew of in-memory designs. However, this solution requires expensive hardware, it is limited to small data items and it can not support batching.

In general, caching by itself is not an effective solution to skew if it is not applied on a more powerful machine/component than the original.Thus, most of the works assume that a cache resides on a more powerful component than the rest of the dataset, while Symmetric Caching is designed to be applied even on a homogeneous set-up.

\textbf{Replication} is the most commonly used method, that targets the problem of skew in in-memory data serving. In this method all data items are initially serviced by their home nodes and once load spikes the most popular items are replicated to other nodes.
However, the conventional approach can not provide a deterministic way to predict the location of the items once replication actions have occurred; thus a dynamic global map that locates the keys in the system has to be known. This is usually accomplished by either providing the location of replicas to the clients, or by steering all the client requests through load balancers, which requires more resources and increases the total number of hops. Additionally, a lot of meta-data are required in order to track the accesses and the placement of individual items, thus data are usually grouped in shards\cite{Huang:2014,Bronson:2013} to reduce this overhead. However, this increases the cost of replication since a single popular key leads into a replication of its whole shard. \\
Hong and Thottethodi \cite{Hong:2013} propose an elegant deterministic method that leverages the existing API and consistent hashing in order to provide replication. Although this approach minimizes the cost of tracking sharers, by just tracking the number or replicas, the client is still required to be notified about which replica to access. Furthermore, this method replicates an item to an other node, without considering any important factors such as the location or the load. Finally, both for the conventional and SPORE's clever approach, offering strong consistency guarantees is a burden. In both cases due to the replica placement, where they might end up being far away, achieve that cost-effectively is not feasible, especially when TCP/IP protocol is used. \\
In contrast, Symmetric Caching it does not require to track any sharers and is transparent to the clients, while it is intentionally applied in groups of closely coupled servers. Therefore it is able to
leverage fast intra-group interconnection such as RDMA for consistency maintenance, offering strong consistency guarantees without compromising performance.

%, which keep these information or by managing and communicating such state to each client.

%
%In this technique, each key is initially services 
%(SPORE, TAO)

%Common replication techniques require to track replica sharers, which is usually achieved either by every node keeping meta-data of every other sharer or by having a centralized meta-data server that 


%More precisely, Symmetric Caching totally avoids the cost of tracking replica sharers, which is usually done by either every replica or by a meta-data/load balancer server that works a directory kee

% Tracking Replicas --> Communicate Replicas to the client or by pass the requests through a load balancer / Transparency
% Consistency 




%\textbf{Blackbox Architecture}

\boris{Isn't this the same as fast remote access - FaRM and Rack-Out?}

%To our knowledge the only work that targets skew leveraging the black box design is RackOut\cite{RNovakovic:2016}. This approach is able to mitigate load imbalances in terms of processing and reach up to 80\% of the uniform performance bounded by the uniform, without the burdens of replication. However, as we have already mentioned in the background this approach is not sufficient to solve the load imbalance in the network; and thus it is capped by the performance of the uniform workload.


%\textbf{RDMA KVs}
%Finally, someone could argue that RDMA KVs\cite{Dragojevic:2014,Kalia:2014} are alleviating the problem of skew by replacing the computation of the heavy TCP/IP stack. However in this case the skew moves towards the network 
%(FaRM,MICA etc..)
\end{comment}



==> Text/5-ccKVS-SC/11-Conclusion.tex <==
\tsection{Summary}
\label{secC:conclusion}

Popularity skew is a well-known bottleneck in existing KVS deployments. Existing skew-mitigation techniques are limited in their efficacy when applied to a distributed in-memory KVS. This work embraces skew as an opportunity through aggressive caching of popular items across all nodes of the KVS. While aggressive replication is generally thought to be a challenge in scale-out settings due to the perceived cost of keeping replicas consistent, we show otherwise. Using a low-overhead {\em symmetric cache} architecture combined with two fully-distributed variants of strongly consistent protocols, we show that our prototype ccKVS outperforms a state-of-the-art KVS on workloads with a moderate write ratio. This strong result paves the way for future work on enforcing strong consistency without sacrificing performance in scale-out settings.  


%Presence of skew in the access patterns for large scale data stores is a well known fact.
%Previous studies have viewed skew, which results in load imbalance in the system, as a problem and have designed a number of techniques towards mitigating it. In this work we took a radically different approach by embracing skew as an opportunity to boost performance.
%Towards that effort we proposed a Scale-Out ccNUMA architecture with symmetric caching, which combines caching with the ability to distribute requests evenly across all nodes. Furthermore, we deployed fully distributed consistency protocols to provide strong consistency guarantees. We designed ccKVS, a KVS based on Scale-Out ccNUMA architecture and evaluated it on a 9-node rack with an underlying low-latency RDMA-enabled interconnect. Contrary to the conventional wisdom, our experiments show that even under strong consistency guarantees skew can be leveraged to increase performance. ccKVS consistently outperforms systems without symmetric caching for read-only workloads and even for workloads with moderate write ratios.


%% TODO these are only for testing (Comment please)
% \input{Miscellaneous/code_for_sequential.tex}
% \input{Miscellaneous/Fig_black_box_hierarchy.tex}
% \input{Miscellaneous/Fig_Design.tex}
% \input{Miscellaneous/Fig_life_of_a_req.tex}
% \input{Miscellaneous/Fig_symmetric_caching_and_blackbox.tex}


==> Text/5-ccKVS-SC/2-Motivation.tex <==
\tsection{Motivation}
\label{secC:motiv}

\tsubsection{Skew and Load Imbalance}
\label{secC:skew}

Prior research characterizing data access patterns in real-world settings has shown that popularity of individual items in a dataset often follows a power-law distribution~\cite{Atikoglu:2012,Novakovic:2016,Huang:2014,Bodik:2010,Yang:2016,Sharma:2011}. In such a distribution, a small number of hot items receives a disproportionately high share of accesses, while the majority of the dataset observes relatively low access frequency. The resulting {\em skew} can be accurately represented using a Zipfian distribution, in which an item's popularity, $y$, is inversely proportional to its rank
%\vijay{This is a bit unclear to me}
$r$:$y ~ r^{-\alpha}$. The exponent $\alpha$ is a function of the dataset and access pattern, and has been shown to lie close to unity. The most common value for $\alpha$ in recent literature is 0.99~\cite{Dragojevic:2014,RNovakovic:2016,Jin:2017,Hong:2013,Li:2016}, with 0.90 and 1.01 also frequently used and cited in KVS research~\cite{Armstrong:2013, Fan:2011}.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/sorted_server_load.pdf} 
  \caption{Load imbalance in a cluster of 128 servers caused by skewed workload with $\alpha=0.99$.}
  \label{figC:server_load}
\end{figure}

An important implication of popularity skew is the resulting load imbalance across the set of servers maintaining the dataset. As shown in Figure~\ref{figC:blackbox}a, the server(s) responsible for the hottest keys may experience several times more load than an average server storing a slice of the dataset~\cite{Novakovic:2016}. For instance, Figure~\ref{figC:server_load} shows an example deployment of 128 servers and a data-serving workload with an access skew of $\alpha=0.99$. As seen in the figure, the server storing the hottest key receives over 7x the average load in the system. %\antonis{Could add a single line output for the theoretical limit of such a system}


\tsubsection{Existing Solutions for Skew Mitigation}
\label{secC:existing}

%\boris{Shouldn't figure 2 be introduced and referenced throughout this section?}

Figures \ref{figC:blackbox}b and \ref{figC:blackbox}c depict two approaches for skew mitigation that have emerged in recent literature: caching and the NUMA abstraction. 

\input{Text/1-ccKVS/Miscellaneous/Fig_related_work.tex}


\noindent
{\bf Caching:} 
Noting that a small fraction of the keys are responsible for the load imbalance, recent work has suggested using a dedicated cache to filter the skew from the access stream before it hits the data serving nodes (Figure~\ref{figC:blackbox}b). Various flavours of the idea have been proposed, which are: (i) placing a cache at the front-end load balancer~\cite{Fan:2011}; (ii) using a programmable switch to steer requests for hot objects to the cache node~\cite{Li:2016}; and (iii) using a programmable switch as a cache node~\cite{Jin:2017}. 

These caching approaches suffer from two important limitations. First, they usually target storage clusters where the back-end nodes are limited by performance of the storage I/O~\cite{Li:2016}. Thus, a powerful server with an in-memory object cache is sufficient to keep up with the load. %\antonis{That's not true for the 3rd flavour.}
The same is not true if the data store is in-memory, in which case the high request rate it can sustain would overwhelm a single cache node. 
%\vijay{But it may not be the case with.....a line would be good here?}\boris{OK -see previous sentence. } 
Secondly, these approaches do not offer a viable strategy to scale the cache beyond a single node to accommodate larger deployments. True, simple partitioning of hot keys across servers is one way to scale to multiple cache nodes; in the limit, however, this strategy is fundamentally limited by the ability of the cache node with the hottest key to keep up with the load. 


\vspace{0.04in}
\noindent
{\bf NUMA abstraction:} Pioneered in FaRM~\cite{Dragojevic:2014} and leveraged in RackOut~\cite{RNovakovic:2016}, this approach offers a NUMA-like shared memory abstraction across the servers storing the dataset via remote access primitives over a low-latency RDMA-enabled network, as shown in Figure~\ref{figC:blackbox}c. More specifically, the one-sided RDMA reads allow any server to directly access the memory of any other server in the deployment. The design exploits this remote access capability to offer a {\em black-box abstraction} %\vijay{I wonder whether there is a need to use black blox abstraction; can't we not simply reuse shared memory abstraction in all places} 
to the outside world -- a client can send a request to any node in the deployment without regard to the data's location. By allowing requests for any object to be evenly distributed across the entire deployment, load imbalance is mitigated in the face of a skewed access distribution.
%Following work in 
% \vasilis{i think we should drop the following 2 sentences as such}

%\boris{I find this paragraph distracting. It doesn't add anything to discussion and breaks the flow. Plus, it seems to be a repeat of the next one. Can we drop it?}
%FaSST~\cite{F-Kalia:2016} improved on the network performance of such systems by replacing the one-sided primitives with two-sided RDMA communication, showing that the performance of the NUMA shared memory abstraction is ultimately bottlenecked by the available network bandwidth. Novakovic et al.~\cite{Novakovic:2014} demonstrated that integrated on-chip NICs can enhance performance by lowering the remote access latency.
% \sout{FaSST~\cite{F-Kalia:2016} improved on the network performance of such systems by replacing the one-sided primitives with two-sided RDMA communication, showing that the performance of the NUMA shared memory abstraction is ultimately bottlenecked by the available network bandwidth.
% Novakovic et al.~\cite{Novakovic:2014} demonstrated that integrated on-chip NICs can enhance performance by lowering the remote access latency.}%~\cite{Novakovic:2014}.

%\vijay{The flow is not great here; can we talk about FaSST and Novakovic after introducing the limitation and conclude nevertheless, remote accesses are a problem?}
The key limitation of this approach is that the vast majority of requests require remote access. Indeed, the fraction of requests satisfied locally is inversely proportional to the number of servers in a deployment. Subsequent work (FaSST~\cite{F-Kalia:2016}) improved on the network performance by replacing the one-sided primitives with two-sided RDMA communication, reducing the overall network overhead of the approach.
%showing that the performance of the NUMA shared memory abstraction is ultimately bottlenecked by the available network bandwidth.
Novakovic et al.~\cite{Novakovic:2014} demonstrated that integrated on-chip NICs can further enhance performance by lowering the remote access latency.
Nevertheless, network bandwidth has persisted as the main performance limiter of the NUMA shared memory abstraction~\cite{F-Kalia:2016}. 
%\vasilis{disagreement:bandwitdh of the hottest sFasst~\cite{F-Kalia:2016} improved on the network performance of such systems by replacing the one-sided primitives with two-sided RDMA communication, showing that the performance of the NUMA shared memory abstraction is ultimately bottlenecked by the available network bandwidth. Novakovic et al.~\cite{Novakovic:2014} demonstrated that integrated on-chip NICs can enhance performance by lowering the remote access latency.erver is the bottle neck}
%\vasilis{this is like saying,that the intra-rack RDMA network is slower than the Ethernet network. E.g. the RDMA is with 56Gbit and the Ethernet is with 100Gb}
%\arpit{Can we just say that the network bandwitdh of the hottest server is the bottle neck and not the network in general?}
%\vasilis{that would answer the question of the bottleneck in a skewed scenario, which is what we care about, we can say above that fasst proves that the bottleneck is the network in the (uniformly accessed) shared memory abstraction}
%\vasilis{Dragojevic feels very strongly about the CPU being the bottleneck in FaRM and not the network, we should not cite him here} \boris{Sure, can you please find a better citation.}\vasilis{\cite{F-Kalia:2016} says the network is the bottleneck in FaSST , we can cite him implicitly assuming that the RDMA is smaller than the Ethernet}
%\antonis{http://sites.computer.org/debull/A17mar/p3.pdf page 6 (40 Gbit)NIC network bound}



\vspace{0.08in}
\noindent
To summarize, existing skew mitigation techniques either (1) use a powerful cache node to filter the skew from the access stream before it hits the storage nodes, or (2) exploit a NUMA-like shared memory abstraction that relies on remote access primitives to distribute the load across all servers. The first approach is processing bound because a single cache node may not be able to keep with the load, which makes it applicable mainly in a disk-based cluster environment. Meanwhile, the latter approach is scalable in its processing capability, but is network bound because the vast majority of requests requires a remote access. 



 

%To summarize, existing skew mitigation techniques either use (1) a NUMA-like shared memory abstraction that relies on remote access primitives to distribute the load across all servers, or (2) exploit a powerful cache node to filter the skew from the access stream before it hits the storage nodes. The first approach is scalable in its processing capability, but is network bound because the vast majority of requests requires a remote access. Meanwhile, the latter approach is processing bound because a single cache node may not be able to keep with the load, which makes it applicable mainly in a disk-based cluster environment. 
%\vasilis{disagreement: cpu is not the bottleneck}%{again, processing is not a good argument there, these caches handle only reads for some tenths of MBs(our cache is 16MB), they should be able to saturate whatever kind of NIC}

==> Text/5-ccKVS-SC/3-Case.tex <==
\tsection{Scale-Out ccNUMA}
\label{secC:case}

The central thesis of this work is that \emph{
a small cache of hot items at each data serving node can effectively shave the skew while scaling cache throughput with the number of servers}. Figure~\ref{figC:blackbox}d demonstrates the proposed approach, which combines the best features of caching and the NUMA abstraction in an architecture we call {\em Scale-Out ccNUMA}. As shown in the figure, Scale-Out ccNUMA augments each node in a pure NUMA deployment with a cache of hot objects. Whenever a client request hits in a server's cache, that node can immediately return the data, thus avoiding a remote access to the node containing the corresponding shard. %\hl{We note that the KVS is sharded across the nodes and thus, any given node acts as the single owner of its allocated shard and is responsible for handling requests to keys belonging to that shard. } \vasilis{the purpose here is to be "explicit" about the sharding}




Intuitively, the proposed approach has the following benefits:

\squishlist

\item Compared to existing cache proposals that have a centralized cache at a load balancer or a network switch~\cite{Fan:2011, Li:2016, Jin:2017} and are thus limited by the throughput of that cache, the per-node cache naturally scales its throughput with the size of the deployment. Moreover, the per-node cache avoids the need for heterogeneous or exotic hardware required by prior work, such as more powerful server in the cache node~\cite{Fan:2011, Li:2016} and/or programmable network switches~\cite{Li:2016, Jin:2017}. Avoiding hardware heterogeneity in a datacenter setting is beneficial from a cost, maintenance and engineering (programmability) perspective. 

\item Compared to a pure NUMA abstraction (e.g., FaRM~\cite{Dragojevic:2014}, Rack-Out~\cite{Novakovic:2016}, FaSST~\cite{F-Kalia:2016}),  %\boris{should we have FASTT here?} \vasilis{sure}
adding a cache to each node can significantly lower the incidence of remote accesses. As Figure~\ref{figC:cache-opportunity} shows, for a zipfian skew with an exponent $a=0.99$ and a cache storing as little as 0.1\% of the hottest data, 65\% of requests will hit in the cache. Thus, only the remaining 35\% of the accesses (i.e., cache misses) may require remote access. 

Critically, the use of caching does not compromise the black-box abstraction presented by the NUMA shared memory architecture. Thus, any client can send a request to any server in the deployment without the knowledge of the data's location. By load balancing the requests across the nodes and avoiding the majority of remote accesses, co-locating a cache with each node naturally improves the scalability of the shared memory architecture. 

%\item Compared to existing cache proposals that have a centralized cache at a load balancer or a network switch~\cite{Fan:2011, Li:2016, Jin:2017} and are thus limited by the throughput of that cache, the per-node cache naturally scales its throughput with the size of the deployment. Moreover, the per-node cache avoids the need for heterogeneous or exotic hardware required by prior work, such as more powerful server in the cache node~\cite{Fan:2011, Li:2016} and/or programmable network switches~\cite{Li:2016, Jin:2017}. Avoiding hardware heterogeneity in a datacenter setting is beneficial from a cost, maintenance and engineering (programmability) perspective. 
%Finally, by co-locating a cache with each node, the proposed approach side-steps the challenge of ensuring that the cache is in the path between a client and the data serving nodes.\vasilis{disagreement:the last benefit should be dropped}

% \boris{this last benefit seems really weak.. should we drop it?}
% \antonis{We could instead point out that the cache miss is really cheap because of local kvs hit or a low over head RDMA access.}\vasilis{we should drop it, it's hard to make that argument because of the TOR} \boris{TOR only applies for switch-based caches, which are a subset of all possible single-node cache solutions.}\vasilis{well yes but it applies to both net cache and switchKV(2/3 citations) and SwitchKV positions itself as an improvement on small Cache, it is a hard argument to make, we would have to elaborate }

\squishend

% \vspace{0.05pt}
Despite the benefits, the proposed approach introduces a significant challenge in requiring the caches to be consistent with respect to each other whenever a write occurs. The consistency challenge can further be broken down into two components. 

The first is how to determine which caches store what items. This is necessary to find the set of replicas, which is needed for consistency-preserving actions (e.g., an invalidation or an update). Consistency protocols used in scalable multi-processors use a directory to track replicas; however, the node holding the directory can potentially become a performance bottleneck.
%as all consistency actions would serialize through it. 
While a directory can be distributed, a skewed access distribution would naturally make certain directory nodes more loaded than others, potentially negating the benefits of caching. 

The second challenge relates to write-serialization, which is an important consistency requirement: all sharers must agree on the order of writes. Scalable multi-processors accomplish this by physically serializing at the directory, which again can cause a bottleneck in our setting. 

Finally we note that in addition to the consistency challenges, Scale-Out ccNUMA also introduces the need for \emph{update} based protocols. Protocols used in scalable multi-processors tend to employ {\em invalidating} protocols, meaning that a writer will invalidate all sharers, which then must re-read the item to bring it back into the cache. This strategy is aimed for parallel workloads where, for example, a variable can be updated multiple times before being read by another thread.
%reducing bandwidth usage, particularly in workloads with high write ratios, since not all processors that accessed a block before the write would necessarily access it again soon after the write. \boris{does this make sense?}
In contrast, with read-intensive workloads that are the target of this work, an item that was updated will very likely be read in the nearest future at other nodes. %\antonis{Isn't this more because of read-intensiveness than hotness?} %Moreover, data serving workloads tend to have very low write ratios~\cite{??,??}.  
This motivates the need for an  updating protocol, since it proactively pushes the updated object to all of the caches.


%but again this must be achieved without  \boris{what are the protocol properties we want?? - please complete.}
%\antonis{The other challenge is that all of the sharers must agree to the same (global) sequence of writes, traditionally this and the directory-requirement are achieved by serializing the writes through the home node as you described earlier.Finally our strong protocol guarantees write atomicity (once somebody reads a value at $t_1$ none in the system can read a previous value at $t_2 > t_1$) achieved via the 2-phase protocol}
%\vspace{0.05in}

In the next two sections, we describe a cache organization, followed by two consistency protocols that address the challenges outlined above. 
%\input{Miscellaneous/Fig_protocols.tex}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/Effectiveness_of_Caching_100.pdf}
  \caption{Effectiveness of caching under popularity skew.}
  \label{figC:cache-opportunity}
\end{figure}

==> Text/5-ccKVS-SC/4-Cache.tex <==
\tsection{Symmetric Cache}
\label{secC:cache}

We exploit a simple insight in designing a scalable cache architecture that helps address the concerns outlined in the previous section. Specifically, we observe that the most popular items are, by their very nature, the most likely ones to be accessed; hence, despite the fact that there are multiple cache nodes, they should all cache the same set of items -- the most popular ones. This idea, which we call {\em symmetric caching}, is illustrated in Figure~\ref{figC:blackbox}d.

Despite its apparent simplicity, the symmetric cache architecture turns out to be extremely powerful, as it naturally resolves a number of challenges. For one, because all caches keep the same set of items, there is no need to inform clients of which node caches what items. Thus, clients can leverage the black-box abstraction and send requests to any node in the data serving deployment, with probability of a cache hit being dependent solely on the requested key and not the choice of the node. This ensures both a load balanced request distribution and a high cache hit rate. 

Another advantage of the symmetric cache is that a node can find out which, if any, nodes cache an item just by querying its local cache; if an item is found there, then {\em all} nodes have it; otherwise, none do. 
Such ability to query a local cache to learn the status of an item naturally avoids the need for a directory, whose role in  cache-coherent multiprocessors is to track the set of caches that have a copy of a cache block. By not having a directory through which consistency actions would need to serialize, the symmetric cache eliminates a potential serialization bottleneck and enables fully distributed consistency protocols, described in the next section.

An important feature of symmetric caching is that the caches are write-back. This means that writes to an item residing in the symmetric cache do not update the underlying KVS until the item is evicted from the cache. This feature is critical in avoiding a throughput degradation at the home node of a popular item, whenever writes follow a skewed distribution. Because all caches maintain the same set of items in the cache, on eviction, only the node containing the shard with the evicted key needs to check if the item has been modified and, if so, update the underlying KVS. 
%\antonis{Add a paragraph arguing that push/pull based approach is orthogonal.}

%\boris{Highlight this paragraph for Kim}
%\hl{
%Kim's comment: "The first part – the identification of the hot items – seems to use a previously published approach [31]. We want your paper to be self-contained (i.e., readers shouldn’t have to read [31] to understand how your caching scheme works), so you should include a few-sentence description of how this approach works. Similarly, you should include a sentence or two describing how the coordinator’s decisions get propagated and the other caches filled (e.g., does the coordinator broadcast the cache entries out to the other nodes? Broadcast the key and let each node cache the entry upon the next access it sees to that KV pair?)"
%\vasilis{I fear we may be overcommiting on this, }
In order for the symmetric cache to be effective, it is essential to be able to identify the most popular items with minimal overhead.
%Nevertheless, we consider the algorithm that detects the popularity distribution orthogonal to our work and thus we resort to existing proposals to perform the task.
%On this work we rely on existing proposals to track the popular items seeing as a policy to detect the popularity distribution is out of the scope of this paper.% and therefore we %. In this work we choose to focus solely on investigating the benefits of symmetric caching and tackling its associated consistency challenges.%, while relying on existing proposals for tracking the popular items.  
This problem has been well-researched with highly-efficient solutions proposed in recent work. 
%We believe that a deployment that employs symmetric caching can seamlessly adopt the approach
A particularly attractive approach for symmetric caching is one
proposed by Li et al.~\cite{Li:2016}, which relies on memory-efficient top-k algorithms~\cite{Cormode:2008, Metwally:2005} to dynamically learn the popularity distribution. In the algorithm proposed by Li et al.~\cite{Li:2016}, each server maintains a key-popularity list with $k$ entries, approximating the popularity of the $k$ hottest keys, and a frequency counter that keeps track of recently visited keys, such that newly popular keys can be detected.
The scheme uses an epoch-based approach, whereby the key-popularity list gets updated and propagated to the cache at the end of each epoch. Finally, request sampling is used to alleviate the performance impact of updating the frequency counter upon each request.
%\boris{The sentence starting with ``At that point'' is confusing. What do you mean proposes? So servers are distributed and the cache is centralized? I got very confused here. Try to resolve this by avoiding detail that may be confusing to readers of our paper.}. \vasilis{is this any better?} \boris{much better. Can we add ``... gets updated and propagated to the cache'' ?}

Conveniently, because symmetric caching exposes a NUMA abstraction, whereby clients spread their requests across all servers, each server sees the same access distribution as do the other servers in the deployment. Therefore, in our setting (and in contrast to ~\cite{Li:2016}), it is sufficient % cordinator
for just a single server to act as the cache coordinator, responsible for identifying the most popular items and informing the other nodes.
%a popular item, with the guarantee that the item is popular across the entire deployment. 
Centralizing the process of classifying an item as popular not only reduces the overhead of tracking hot items, but also naturally alleviates the burden of reaching a consensus on which items are popular, thus simplifying the entire process. While our evaluation does not consider shifts in popularity skew, we expect the set of most popular keys to evolve slowly, with only a handful of keys removed/added to the cache every few seconds~\cite{Li:2016}.
%We note that we do not evaluate the process of updating the cache, but we deem its performance impact negligible, because the expectation is to have a handful of cache changes at the granularity of seconds~\cite{Li:2016}.
%\boris{I rephrased the highlighted part- please check.} \vasilis {Changed 'Several seconds' to 'few seconds' because the citation changes 200 keys every 1 or 10 seconds}
%\vasilis{we need some lines here to address Kim's comments}
%}

\begin{comment}
In order for the symmetric cache to be effective, it is essential to identify most popular items with high precision and low latency, in case the popularity distribution shifts. Fortunately, this problem has been well-researched with highly-efficient solutions proposed in recent work. We adopt an approach proposed by Li et al.~\cite{Li:2016}, which relies on memory-efficient top-k algorithms~\cite{Cormode:2008, Metwally:2005} to dynamically detect the popularity distribution in each server within a deployment. Conveniently, because symmetric caching exposes a NUMA abstraction, whereby clients spread their requests across all servers, each server sees the same access distribution as do the other servers in the deployment. Therefore, it is sufficient for a single server to locally identify a popular item, with the guarantee that the item is popular across the entire deployment. %\boris{what are the benefits - I can see it enabling lower detection latency or a simpler protocol (no need to rank popular items across all servers. Please comment here. } \vasilis{the algorithm needs to run only one a single node at any time, instead of on all of the nodes}
\end{comment}
%\input{Miscellaneous/Fig_symmetric_cache}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COMMENT (old text on symmetric caching
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
In this work we propose \textit{Symmetric Caching}: 
where each machine is equipped with an in-memory \textit{popularity cache} as shown in Figure \ref{figC:symmetric-caching}. Machines that belong in the same black-box have replicated or identical caches that contain the most popular items stored in the black-box.
%we insert a (software) \textit{popularity cache} in each of the KVS servers that stores the most popular data items, as illustrated in Figure  
Symmetric Caching enables all servers to concurrently access the hot data items, avoiding hot spots in the system and load balancing both the request processing and the network bandwidth consumption.
As Figure \ref{figC:caching} illustrates,the effectiveness of the popularity caches: under a skewed workload with exponent $\alpha= 0.99$, a popularity cache that contains a small subset of the entire dataset, stored in a black-box, (e.g. 0.1\%) can achieve a substantial cache hit rate (e.g. 65\%) exploiting the skewed access pattern. \arpit{Is it really $65\%$ at $0.1$. Does not seem so from the figure.}
\antonis{It's 63\% not 65\% so we should correct this.}
%\antonis{should we change the huge cache hit with more than half or requests? since maybe huge cache hits may someone}\vasilis{RESOLVED}

\input{Miscellaneous/Fig_symmetric_caching_and_blackbox}

% SYNERGY WITH RACKOUT
This idea works in synergy with the black box architecture: since the majority of the incoming requests may refer to remote keys but the server will still be able to serve most of them locally using the popularity cache. This  further alleviates the drawback of the initial design, which is the extra hop most requests would require in the absence of the popularity caches.
Furthermore, the popularity cache filter the skew out of the access pattern: requests that refer to cold data items and miss in the popularity cache, will follow a distribution very close to uniform, bringing balance to the load in both the network and the CPU of the servers. 
Finally the addition of Symmetric Caching to the black-box architecture demotes the one-sided semantics from necessary to optional. Remember that the one-sided semantics are a mandatory requirement in the original architecture, to unburden the host CPU of the hot server; that is not the case when Symmetric Caching is applied.



% TRANSPARENCY 
%\antonis{The following paragraph about transparency should probably be moved to Related Work}
In contrast with, other caching or replication techniques that demand the intervention of client, Symmetric Caching has the advantage that it can be adopted transparently. Existing solutions usually push complexity to the client-side, by either relying on the clients to handle cache misses or by requiring them to communicate with the back-end service and maintain an up-to-date location of replicas.


%IMAGE

%FEASIBILITY - HOTNESS DETECTION
One major limitation of existing replication techniques is the problem of tracking replica sharers both for dispatching the requests and for maintaining consistency among the replicas. In large-scale data serving environments, which are constituted by numerous nodes and an enormous amount of distinct data items, the complexity and cost of tracking sharers in key granularity is very challenging. On the other hand, Symmetric Caching overcomes this obstacle since it does not require any meta-data for tracking replica sharers. This is due to the fact that once a key has been identified as hot, then a machine is a sharer if and only if it belongs in the same black-box with the home node of the key. 

Therefore, popularity caches always contain the hottest data items, thus they differ from the traditional designs that require bringing every data item in the cache before it gets accessed. This method avoids cache pollution with cold items which are not accessed frequently.

\vasilis{This is very important. We need to find it a home}
The feasibility of caching the most popular items in a single machine in-memory has been explored in previous research work. Fan et.al \cite{Fan:2011} have shown that a small, software cache, in the order of tens to hundreds of MBs, is enough to cache the hottest data items of a large data set.

However, the popularity caches require a way to identify the hottest keys and update the contents of the caches on demand. Li et al\cite{Li:2016} have already tackled this problem in designing SwitchKV, which we discuss analytically in section \ref{secC:Related}\antonis{do we?}.  Li et al. leverage memory-efficient top-k algorithms (\cite{Cormode:2008, Metwally:2005}) to dynamically detect the popularity distribution in each server. The same mechanisms can be used in our design without any changes. However, in our design a server receives requests that refer to the entire -box. Therefore, unlike SwitchKV, in our design it is sufficient for a single server to sample the incoming requests. When that server detects that a data item needs to be evicted or inserted to the cache due to a change in the popularity distribution, it broadcasts a message to all servers notifying them of the change.


\end{comment}


==> Text/5-ccKVS-SC/5-Protocols.tex <==
\tsection{Enforcing Cache Consistency}
\label{secC:protocols}

%\boris{Somewhere, need to discuss three basic things: \\
%1) serializing on a write is intuitive (in fact, that's what FaRM %does), but has bad performance in the presence of skew. \\
%2) we choose an updating, rather than invalidating, protocol. \\
%3) we don't update the home when an item is in the cache (i.e., the %cache is write-back). 
%}

With symmetric  caching, whilst we are able to serve a significant chunk of read requests (the cache hits) locally,
ensuring consistency in the presence of writes is  challenging. To ensure this, a consistency protocol must propagate writes that hit in one cache to all of the caches. What determines \emph{when} and \emph{how} writes are propagated is the consistency model.

A plethora of weaker consistency models abound  under the umbrella of \emph{eventual consistency}. The only requirement is that all replicas must eventually converge on a value in the absence of new updates, allowing for writes to be propagated asynchronously in any order. Performance-wise, this is beneficial, but eventual consistency can be be hard to reason about and can cause nasty surprises for both developers and clients~\cite{Vogels:2009}.
%\arpit{Do we need a reference here?} \vasilis{ this seems appropriate\cite{Vogels:2009}}

More intuitive models mandate \emph{write serialization}: all sharers must agree on the order of writes to a single key. Stronger yet models mandate that writes must propagate synchronously, i.e. in a blocking fashion. Enforcing such strong guarantees in a high-throughput fashion is challenging. One natural way to enforce write serialization is to employ passive replication (also known as primary-backup replication), where writes of a specific key serialize at a designated primary, as shown in Figure~\ref{figC:protocols-design}a. Such passive protocols are commonly used in shared memory multiprocessors~\cite{Vijay:20} and other distributed systems~\cite{Dragojevic:2015} that demand strong consistency. In the same spirit, distributed systems can opt to achieve write serialization through a sequencer, as shown in Figure~\ref{figC:protocols-design}b, which assigns monotonically increasing timestamps to writes and their consistency actions (i.e. invalidations, updates). 

However, in the presence of skew, the primary (or sequencer) in the two approaches could easily become a hotspot on writes to a hot item, as consistency actions related to that item must serialize through it. We address this issue by employing fully distributed protocols that achieve write serialization in a fully distributed manner, shown in Figure~\ref{figC:protocols-design}c, while still guaranteeing strong consistency. We elaborate on the protocols specifics below.%Thus, we want protocols that do not force serialization through any one node, while still guaranteeing strong consistency. 
% \boris{This is great imo. Tweak wording in the last paragraph - please check}

%that concurrent writes (to same key) serialize in the same order from the perspective of every client. 
%However, enforcing write serialization in a high-throughput fashion without inducing spots in the protocol is challenging. Yet stronger models mandate that writes must propagate synchronously; to achieve this efficiently, the protocol must  minimize write propagation delay (e.g. by reducing costly hops).

%the   serialize stronger consistency models require the writes to propagated both \emph{synchronously} (in the critical path of the write) and \emph{atomically} (appearing as a single event).
%Intuitively, a read should always return the latest copy of the data regardless of which replica  serviced the read - an invariant called \emph{strong} consistency. Ensuring strong consistency necessitates that writes are propagated to all replicas \emph{synchronously} (in the critical path of the write) and \emph{atomically} (appearing as a single event).  
%a write to a cached object poses a problem. To ensure data consistency, such writes must be propagated to all of the caches. When and how the writes must be propagated is mandated by the consistency model. 
%In order to ensure high throughput, it is imperative for the consistency protocols  to be fully distributed (e.g. by avoiding protocol serialization points). The protocol must also minimize write propagation delay (e.g. by reducing costly hops) whenever possible. Because of tricky corner cases and race conditions, these protocols are often hard to get right; for this reason, it would be desirable to formally verify that the protocols in fact enforce the promised consistency model.    
%-- the protocol must avoid serialization points as that could become a hotspot. reduce the write propagation delay (e.g. by reducing costly hops) whenever possible. The protocols must also be fully distributed to avoid potential hot-spots -- ensuring that writes appear atomic without throughput-limiting protocol serialization is a challenging problem. Finally, these protocols can be hard to get right, and it would desirable to show that the protocol in fact enforces the promised consistency guarantee. 

%While a plethora of weaker consistency models abound in this space under the umbrella of \emph{eventual consistency}, they are hard to understand and reason about. 
%some applications do require stronger guarantees. 

In this work we consider two strong models: \emph{per-key sequential consistency} (SC) and \emph{per-key linearizability} (Lin). 
%consistency models: strong consistency (per-key linearizability), and a reasonably strict interpretation of eventual consistency (per-key sequential consistency).  
We employ fully distributed protocols that enforce the models efficiently.
%Since such protocols can be tricky to get right, we formally verify the Lin protocol  for safety and deadlock freedom with the help of a model checker. 
In the rest of the section,  we first introduce the two consistency models, then briefly overview existing protocols and their limitations, and finally describe the protocols in depth. 
\input{Text/1-ccKVS/Miscellaneous/Fig_protocols}

%\boris{ } \\
%- Why writes are a problem? \\
%- Terminology \\
%- Existing techniques: why or why not? (serializing actions, blocking - this sort of discussion)
% Overview

\tsubsection{Consistency Models}
For this discussion, let us assume that a number of clients (modelled as \emph{sessions}) are interacting with a replicated data store by issuing get and put requests~\cite{Burckhardt:2014}. The \emph{session order} is a per-session total order which represents the order in which gets and puts appear in each session. A put writes the provided object (abstracted as a value) of the corresponding key, whereas a get reads and returns the value. 
%Each operation (get or put) in this model is identified by a \emph{session}, which abstracts the client that issued this operation. 

A consistency model must formally specify what value a get must return. \emph{Since we are considering data serving applications, our focus is on consistency models that provide guarantees on a per-key basis~\cite{DeCandia:2007}; there are no guarantees between gets and puts of different keys}. 
%\boris{can we cite good work that provides the same guarantee only?}\vasilis{Dynamo is a good choice \cite{DeCandia:2007}}
We focus on
%a strict interpretation of eventual consistency that guarantees 
SC and Lin, the latter strictly stronger than the former.  
%the latter strictly stronger than the former. 
It is worth noting that in both of the above models, updates to any object must happen atomically;  
%puts must appear to perform atomically; in other words, 
a get must return a value written in its entirety by exactly one put -- it cannot return a mishmash of the values written by two different puts.

%discuss 3 progressively stronger consistency guarantees, with each guarantee also satisfying the prior ones. 

%\noindent{\bf Atomic put.} This basically says that a put must appear to perform atomically; in other words, a get must return a value written by a put in its entirety, it cannot return a mishmash of the value written by two different puts.


%\boris{can we introduce abbreviations (say, PSC/PL or SC/LIN) and use them throughout?}

\noindent{\bf Per-key Sequential Consistency.} 
Informally, SC allows for writes to propagate asynchronously, as long as all sessions can \emph{agree on the order of writes to the same key} . 
The following sequence of operations to key K, depicted in Figure~\ref{figC:consistency-example-1}, does not violate SC. Session A writes a value of 1  at real time $t_0$, then reads its own write at time $t_1$. Later, at time $t_2$, it is permissible for session B to read the old value of 0, since SC does not mandate that write must happen synchronously. 
However, the following sequence illustrated in Figure~\ref{figC:consistency-example-2} is not allowed. There are two concurrent puts to same key (from sessions A and D). From the point of view of session B, the put from session A appears to perform before that of session D. Session C, however, observes a different order. Since the two sessions don't agree on the order of puts, there is a SC violation. 

\input{Text/1-ccKVS/Miscellaneous/Fig_consistency_example_1.tex}
\input{Text/1-ccKVS/Miscellaneous/Fig_consistency_example_2.tex}

%There are a number of consistency models grouped under the umbrella of eventual consistency -- 
%We use a strict interpretation of eventual consistency from Burckhardt~\cite{Burckhardt:2014} that guarantees sequential consistency on a per-key basis. 
Formally, SC mandates that: (i) every put must eventually propagate (i.e. it must be made visible) to all sessions;
(ii) all sessions must agree on the order of puts to the same key (writes must serialize) and (iii) gets and puts from the same session to the same key must appear to take effect in session order.
More formally, gets and puts of the same key from all sessions must appear to perform in some total order that is consistent with the session order. 
%This has been formalized by Burckhardt as \emph{basic eventual consistency}. 
It is worth noting that a similar guarantee has been formalized as \emph{coherence}  in the world of shared memory multiprocessors~\cite{Alglave2014a}. 


%In order to understand the guarantee better, let us consider the example shown in Figure. 
%that illustrates a violation of this consistency guarantee.
%As we can see 



\noindent{\bf Per-key Linearizability.} Informally, the data store must behave as if there exists only a single copy of every object in the data store, and at any time-step at most one session may issue an operation (get or a put) in session order.
%(once that operation is completed, the next session is chosen to issue an operation). 
Thus, Lin preserves real-time behaviour, with each call to get and put appearing to take place some time between their invocation and completion. Therefore, the behavior shown in Figure~\ref{figC:consistency-example-1} is impossible in a system that guarantees Lin. Lin must satisfy all the constraints of SC along with two additional conditions: (i) a put must return only after the value written has become visible to all sessions 
%\antonis{Isn't more accurate to say "only after other sessions are not able to read the previous value"? (ones you have received all the acks)}
(writes are synchronous); (ii) a get may return a value only after the put (from which it reads its value) has become visible to all sessions. 

%In order to understand the guarantee better. let us consider the example shown in Figure which shows a put from session 1 returning at time $t_1$ (real time) and get from session 2 returning at time $t_2$ ($t_2 > t_1$). With linearizability it is not possible for the get to see the earlier value, whereas with sequential consistency it is allowed. 
%It is worth noting that a similar correctness criterion to linearizability (single writer multiple readers invariant~\cite{sorin}) is often used as a correctness specification for cache coherence protocols in multiprocessors (although they technically require only a weaker per-location sequential consistency guarantee).  

\tsubsection{Protocols}
\label{secC:dist-protocols}
%{\bf The Challenge.} As noted earlier, protocols that achieve guarantees similar to SC are commonplace in shared memory multiprocessors (coherence protocols~\cite{sorin2011primer}). Although there are an astonishing number of variants of these protocols, they all generally operate as follows: each write serializes at a pre-defined home for that address (known as the home directory), which then broadcasts invalidate messages to all of the nodes that are currently caching the address. 
%While such protocols work well in the multiprocessor context, 
%(ample on-chip network bandwidth and CPU intensive workloads), 
%they don't translate well to the data serving setting. The chief reason is that the home directory responsible for hot items can become a hotspot due to the highly skewed popularity distribution, and can thus become a performance bottleneck. 
%Additionally, each write would have to incur an extra hop to the directory which would unnecessarily increase bandwidth consumption and the write's latency. 

%\sout{Also, updates are preferred to invalidates in our setting because the hot keys are likely to be accessed soon. Thus, we would need fully distributed update based protocols for our context.} \boris{rewrote:}
%Another important difference is that protocols used in shared memory multiprocessors tend to employ {\em invalidating} protocols, meaning that a writer will invalidate all sharers, who then must re-read the item to bring it back into the cache. This strategy is aimed for
%parallel workloads where, for example, a variable can be updated multiple times before being read by another thread.
%reducing bandwidth usage, particularly in workloads with high write ratios, since not all processors that accessed a block before the write would necessarily access it again soon after the write. \boris{does this make sense?}
%In contrast, popularity skew that is the target of this work implies that a hot item will very likely be accessed in the nearest future. %Moreover, data serving workloads tend to have very low write ratios~\cite{??,??}.  
%This motivates the use of an {\em updating} protocol, since it proactively pushes the updated object to all of the caches.
%thus avoiding the latency cost of a cache miss, without incurring much bandwidth overhead due to the low write ratios. 
%Next, we describe two protocols that satisfy the requirements of being fully distributed and updating. 

%One way to achieve Write Serialization is for writes to serialize at a pre-defined home for the key, similar in spirit to distributed directory based protocols. Each write serializes at the home, which then broadcasts invalidates to all nodes. 
%There is a number of problems with this approach. Firstly, every write needs to serialize at the home, which can become a bottleneck for hot keys. Additionally, each write would have to incur an extra hop, that would unnecessarily increase bandwidth consumption and the write's latency. Finally, updates are preferred than invalidates because the hot keys are by default likely to be accessed.

\noindent
\textbf{SC Protocol.}
%To address these three concerns 
We adapt the update-based protocol developed by Burckhardt~\cite{Burckhardt:2014} that uses Lamport timestamps for achieving write serialization.
% EVENTUAL STORE
%The assumption of Eventual Store is that all machines of the deployment store the exact same data, which is the case with our popularity caches. 
Each object in the symmetric cache is tagged with a Lamport logical clock~\cite{Lamport:1978}, along with the session id of the last writer. (Together, the clock and session id are referred as Lamport timestamp.) On a put that hits in the cache, the writer: (1) increments the Lamport clock, (2) writes the new value, and (3) broadcasts an update that contains the new value and the timestamp. 
%The field \textit{timestamp} represents  both the Lamport clock (i.e. field \textit{lclock}) and  the   the machine id of the writer (i.e field \textit{last\_writer}). %Note how the code locks the key before performing any update to its state or its value, guaranteeing that all changes happen atomically.

On receiving an update, a node will apply the change only if the received value has a bigger Lamport clock than the stored Lamport clock. If the two Lamport clocks are equal, the session ids are used as tie breakers. 
%Note that the pseudocode treats the combination of the Lamport clock and the last writer id as one value: the \textit{timestamp}. 
%The stored timestamp will be smaller than the received timestamp iff it has a smaller \textit{lclock}, or an equal \textit{lclock} but a smaller \textit{last\_writer}. Finally on a get, the machine simply reads the stored value. 

%It is worth noting that the protocol is fully distributed; 
Figure \ref{figC:protocols-design}c shows the fully distributed nature of the protocol, where write serialization is achieved via the use of Lamport timestamps, thus avoiding the use of serialization points (Figures \ref{figC:protocols-design}a and \ref{figC:protocols-design}b). The protocol is non-blocking: writes are asynchronous and can be locally applied immediately (on any replica), allowing for reads following the write to return the new value without waiting for the broadcast. 

%The only state kept along with each key is a Lamport clock and the id of the last writer to the value. The value cannot be in an Invalid state or any other state and thus, reads are never stalled, while all writes can immediately be locally applied an propagated to the rest of the caches.


% WHY DOES EVENTUAL STORE HONOUR THE GUARANTEES
%This protocol guarantees Write Serialization, by enforcing a global rule to determine the stronger write in the case of multiple concurrent writes.
\noindent\underline{Invariant.} Each write is tagged with a Lamport clock and the session id of the writer, which gives a unique timestamp for every write. 
%no two writes to the same key can ever have the same timestamp.
This is the invariant that ensures write serialization. The reader is referred to Burckhardt~\cite{Burckhardt:2014} for a formal proof.

%the combination forms a unique id for each write: the \textit{timestamp}; no two writes to the same value can ever have the same timestamp. That is the invariant enforced by the protocol: each write has a unique timestamp and there is a global way to compare the timestamps, therefore all machines will always agree on which write is the latest. That invariant guarantees write Serialization, as all machines agree on a global order for all writes to the same data. Read my writes is trivially enforced. Eventual propagation is ensured because we assume a reliable broadcast. 
\input{Text/1-ccKVS/Miscellaneous/Fig_consistency_actions}
\noindent
\textbf{Lin Protocol.}
Recall that with Lin, a put can return only after it has propagated to all sessions. This 
%Guaranteeing synchronous writes 
calls for a two-phase protocol: the writer needs to broadcast invalidations and get an acknowledgement from every other sharer; only then can the value  be broadcast. 
Of course, there can be multiple puts happening concurrently and all sessions need to agree on the same order. Therefore, in the first phase invalidations are tagged with Lamport timestamps to achieve write serialization. Figure \ref{figC:consistency-actions} illustrates the phases involved. 

\todo{UPDATE!}\\
The protocol we use is an adaptation of the one proposed by Guerraoui et al.~\cite{Guerraoui:2007}. Because writes are synchronous (blocking), there are situations when the protocol is waiting for an event and must deal with intervening requests correctly, without violating safety or causing deadlocks. Thus, we must account for and handle such \emph{transient} states.
%and verify the protocol using a model checker. 
%in the system, before broadcasting an update. That guarantees that everyone will have invalidated the old value, before anyone can read the new value.

 %% Protocol - INVARIANT

% PROTOCOL
% perform write
\noindent\underline{Protocol actions.}
A session that performs a put increments its Lamport clock and transitions the state of the cached object to a transient  \textit{Write} state (indicating that it is waiting for acknowledgements). It then broadcasts invalidations that include the key, and its Lamport timestamp. 
%its Lamport clock and its own machine id. Similarly to the Eventual Store protocol, the machine id and the Lamport clock compose the timestamp of the invalidation (i.e. the unique id of the write).
% receive invalidation
When a node receives an invalidation, it compares the incoming timestamp with the stored timestamp. If the received timestamp is greater, the machine transitions the state of the cached object to \textit{Invalid} and responds to the writer with an acknowledgment. 
%Alternatively, if the received timestamp is smaller than the stored timestamp, then the receiver discards the invaldiation and does not respond to the machine. The reason why no response is required in that case, is simple: if one server has seen a write, sooner or later all servers will see the same write, more importantly, if one server thinks that timestamp A is greater than timestamp B, then all servers agree on that comparison. Therefore a negative acknowledgement would be redundant: the sender of the invalidation, is guaranteed to see an invalidation for the stronger write and will transition to an \textit{Invalid} state.
% receive acknowledgement
When a node receives an acknowledgement, it increments a counter that holds the received acknowledgements for the relevant key. When the counter indicates that all nodes have acknowledged the invalidation, the cached object is transitioned to  \textit{Valid} state and the new value and its timestamp are broadcast.  
%broadcasts an update message with the new value and the write's timestamp to all of the machines. 
%receive update
Upon receiving an update, a node will check whether the relevant key is currently in \textit{Invalid} state, waiting for the particular update (checked via comparing the timestamps); 
%To verify the latter, the node checks if the stored timestamp is equal to the received timestamp. if both conditions hold true, 
if the timestamps match, the update is applied and the object transitions to \textit{Valid} state, otherwise the update is discarded. 
%Either way, the server never responds to receiving an update.

%\boris{Highlight this paragraph for Kim}
\noindent \underline{Verification.} 
%\hl{
The Lin protocol has one stable state and two transient states, making it more complex than the SC protocol, which has only one stable state and no transient states and has been formally shown to be correct by Burckhardt~\cite{Burckhardt:2014}. Therefore, we wanted to formally verify the Lin protocol. To this end, we expressed the Lin protocol in the model checker Mur$\varphi$~\cite{Dill1996} and verified the protocol for safety and the absence of deadlocks. For safety, we verified two invariants. First, the \emph{single-writer-multiple-reader} invariant (SWMR)~\cite{Vijay:20}: at any given time there can be exactly one writer that can update an object (multiple readers can safely read an object). Second, the \emph{data value invariant}: if an object is in a valid state (that can be read), then it must hold the most recent value that was written to that object.  Our Mur$\varphi$ model allows for the number of processors, addresses, and timestamp size to be configured. We have verified with three processors, two addresses and timestamp of size two bits. A detailed state transition table as well as the Mur$\varphi$ model is available online.\footnote{ 
\label{footC:link}\href{http://s.a-phd.com}{http://s.a-phd.com}} 
%}

%This protocol is similar to work done by Guerraoui et al \cite{Guerraoui:2007}. We specify all the transient states of the protocol and we have verified its correctness with a model checker.



\begin{comment}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.4\textwidth]{Figures/Write-Atomicity.pdf} 
  \caption{Violation of  Write Atomicity in a deployment with 4 machines \vasilis{TODO:let's put a time arrow on these, if we keep them} \antonis{An example with multiple keys here may confuse since we are not guaranteeing per key ordering.}}
  \label{figC:write_atomicity}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/Write-serialization.pdf} 
  \caption{Violation of  Write Serialization of writes to key A, in a deployment with 4 machines}
  \label{figC:write_ser}
\end{figure}
\end{comment}
%\input{Miscellaneous/code_for_sequential}

%--------------------------------------------------------------------------------------
%-----------------------------------------OLD STUFF------------------------------------
%--------------------------------------------------------------------------------------

\begin{comment}

\tsubsection{Consistency} 
\label{secC:Protocols}
%Problem with Writes 2 flavours to deal with it: SC and EC:
%Symmetric Caching comes with a challenge: writes to the hot data items must be propagated to all the nodes of the black box to ensure that the caches are coherent. However, this limitation is not as devastating as one may think. The write rate (i.e. the percentage of writes) is typically very low in data serving systems (e.g. 0.2\% in Facebook's TAO \cite{Bronson:2013})
%Although data-serving accesses are characterized as read-mostly, when replication is applied handling writes is a major factor that determines system's performance. In a replicated environment reads can be served efficiently, in contrast to writes that require special actions to ensure consistency among the replicas. According to multiple studies, consistency maintenance is challenging\cite{Ajoux:2015} or almost impossible to be achieved\cite{Fan:2011} in non-trivial scenarios. However, we show that this is not true when \textit{Symmetric Caching} is applied;
%considering the write rate (i.e. the percentage of writes) is typically very low in data serving systems (e.g. 0.2\% in Facebook's TAO \cite{Bronson:2013}) and that
%the KVS needs to only offer per-key guarantees(\vasilis{citation}). In other words, the ordering of reads and writes to different keys is irrelevant. 
Although data-serving accesses are characterized as read-mostly, when replication is applied handling writes is a major factor that determines system's performance. In a replicated environment reads can be served efficiently, in contrast to writes which require special actions for ensuring consistency among replicas. According to multiple studies, consistency maintenance is challenging~\cite{Ajoux:2015} or almost impossible to be achieved~\cite{Fan:2011} in non-trivial scenarios. However, we show that this is not true when \textit{Symmetric Caching} is applied.

Consistency maintenance of the replicated keys in Symmetric Caching can be reduced to the problem of keeping the caches within a group (e.g. black box) coherent, similar to traditional hardware caching. Thus, protocols for coherency actions are likewise required. However, data-serving systems have to apply such actions through software, over slower interconnects and at a larger-scale. As a result, there is a need to a) reduce the costly hops and b) make the protocols as distributed as possible, to avoid potential hot-spots.


With these principles in mind and considering that
the KVS needs to only offer per-key guarantees (\vasilis{citation}), we address this challenge by supporting two flavours of Consistency models: per-key Sequential Consistency \arpit{Eventual?}\vasilis{The terms per-key SC, per-key linearizability, write serialization and write atomicity are all placeholders, I just do not know what we are gonna call these things, so i picked some names. Per-key SC refers to Eventual, yes.} and per-key Linearizability. Both models guarantee that writes happen atomically, i.e. a read can never return a partial write or a combination of two concurrent writes. The implementation details of how concurrent requests are handled to ensure atomic writes are discussed in section \ref{secC:Concurreny}. For each of the models we develop a fully distributed and scalable protocol over RDMA, where writes can be directly executed from any replica.

% TRACKING SHARERS

\tsubsection{Consistency models}

\tsubsubsection{Per-key Sequential Consistency}
%% GUARANTEE: WRITE SERIALIZATION
\textbf{Guarantees.}
Per-key Sequential Consistency(per-key SC) guarantees that all writes to the same key-value pair are globally serialized. In other words, all servers agree on the order of writes to the same key. We call this guarantee \textit{Write Serialization}, as it is called in the multiprocessor world~\cite{Adve:1996}. As an example, Figure \ref{figC:write_ser} illustrates a violation of write serialization. Machine 1 (M1) performs a write concurrently with machine 4 (M4); machine 2 serializes the write from machine 4 (i.e. A=2) after the write from machine 1 but machine 3 serializes the writes in the reverse order. That violates write serialization, because at least two of the machines disagree on the order of writes to the same data.




%% PROTOCOL: HOW IT GUARANTEES WRITE SERIALIZATION

% PROTOCOL NEEDS TO BE DISTRIBUTED
One way to achieve Write Serialization is for writes to serialize at a pre-defined home for the key, similar in spirit to distributed directory based protocols. Each write serializes at the home, which then broadcasts invalidations to all nodes. There is a number of problems with this approach. Firstly, every write needs to serialize at the home, which can become a bottleneck for hot keys. Additionally, each write would have to incur an extra hop, that would unnecessarily increase bandwidth consumption and the write's latency. Finally, updates are preferred than invalidates because the hot keys are by default likely to be accessed. %\antonis{I don't see invalidate vs update protocol this as the second problem. I would argue that the second problem is the 1 extra hop that is required ;)} \vasilis{good point, RESOLVED}
To address these three concerns we adopt a fully distributed update-based protocol developed by Burckhardt\cite{Burckhardt:2014}: \textit{Eventual Store}. 


% EVENTUAL STORE

\textbf{Protocol.} The assumption of Eventual Store is that all machines of the deployment store the exact same data, which is the case with our popularity caches. Each item in the popularity cache is stored along with its own Lamport clock \cite{Lamport:1978} and the machine id of the last machine that updated that value. On a write to a hot item the writer 1) increments the Lamport clock 2) stores the new value and 3) broadcasts an update that contains: the new value, the new Lamport clock of the value and its own machine id. The function \textit{perform\_write()}, in the pseudocode of listing \ref{lstC:write-atomicity}, demonstrates what happens on a write. The field \textit{timestamp} represents  both the Lamport clock (i.e. field \textit{lclock}) and  the   the machine id of the writer (i.e field \textit{last\_writer}). Note how, the code locks the key before performing any update to its state or its value, guaranteeing that all changes happen atomically.

On receiving an update, a machine will apply the change only if the received value has a bigger Lamport clock than the stored Lamport clock. If the two Lamport clocks are equal, then the machine ids are used as tie breakers. The function \textit{perform\_update()} showcases the actions on receiving an update. Note that the pseudocode treats the combination of the Lamport clock and the last writer id as one value: the \textit{timestamp}. The stored timestamp will be smaller than the received timestamp iff it has a smaller \textit{lclock}, or an equal \textit{lclock} but a smaller \textit{last\_writer}. Finally on reading a value, the machine simply reads the stored value. 

The only state kept along with each key is a Lamport clock and the id of the last writer to the value. The value cannot be in an Invalid state or any other state and thus, reads are never stalled, while all writes can immediately be locally applied an propagated to the rest of the caches.


% WHY DOES EVENTUAL STORE HONOUR THE GUARANTEES
%This protocol guarantees Write Serialization, by enforcing a global rule to determine the stronger write in the case of multiple concurrent writes.
\textbf{Invariant.} In Eventual Store each write is tagged with a Lamport clock and the id of the writer; the combination of the two ids, forms a unique id for each write: the \textit{timestamp}; no two writes to the same value can ever have the same timestamp. That is the invariant enforced by the protocol: each write has a unique timestamp and there is a global way to compare the timestamps, therefore all machines will always agree on which write is the youngest. That invariant guarantees Write Serialization, as all machines agree on a global order for all writes to the same data. 

\vasilis{the architecture can also gives us monotonic reads and  Read My Writes on top of the protocol's guarantees}

%One minor fix for fairness: we publish new priorities randomly for fairness. 

%Corner cases and transient states: 
%What do we do when there is a get for the key while the update in progress? Go ahead and do the get.. Why?
%What do we do when there is a put for the key while the update in progress? Go ahead and do the next update. Why? 
\input{Miscellaneous/code_for_sequential}
\input{Miscellaneous/Fig_consistency_actions}

\tsubsubsection{Per-key Linearizability}

% GUARANTEES
\textbf{Guarantees.} In most cases the guarantees offered by per-key SC are sufficient. However, for the cases where stricter guarantees are required, we offer a protocol for Per-key Linearizability. Similarly to  per-key SC, Per-key Linearizability guarantees Write Serialization and that all writes are atomic (even between multiple nodes). The additional guarantee is that under per-key Linearizability \textit{a read is not allowed to return an old value, after an earlier read has returned a new value}\cite{Guerraoui:2007}. In other words, a machine cannot read a new value, if that value is not yet visible to all machines. The combination of this property with Write Serialization is commonly known as \textit{Write Atomicity} in the multiprocessor world \cite{Adve:1996}. 

Figure \ref{figC:write_atomicity} illustrates a violation of Write Atomicity. Initially all values are equal to zero, then machine 1(M1) writes A = 1. Machine 2 (M2) reads the write to A and then writes to B. Then machine 3(M3) reads B and then A; machine 3 sees the new write to B, but not the write to A. This is a violation of Write Atomicity, because machine 2 can read the write to A, but machine 3 cannot. This violation occurs when a write propagates to different machines at different times. This problem calls for a two-phase protocol: the writer needs to broadcast invalidations and get an acknowledgement from every other sharer in the system, before broadcasting an update. That guarantees that everyone will have invalidated the old value, before anyone can read the new value.




 %The protocol for per-key linearizability needs to adhere to the same principles as the Eventual Store,
 
 %% Protocol - INVARIANT
 \textbf{Protocol.} We couple a two-phase protocol with Eventual Store to build  a fully distributed, update-based, two-phase protocol that guarantees per-key Linearizability. In that protocol, Write Serialization is guaranteed by the invariant that each write is coupled with a unique id (i.e. its timestamp), while Write Atomicity is guaranteed by the two-phase aspect of the protocol: a machine needs to broadcast invalidations and gather all acknowledgements before it is able to broadcast the update. Figure \ref{figC:consistency-actions} demonstrates the coupling of the 2 protocols. In per-key Linearizability, the writer needs to perform all 3 of the illustrated actions: 1) broadcast invalidations 2) gather acknowledgements and 3) perform the write locally and broadcast updates, while under per-key SC, the writer performs only the third action.

% PROTOCOL
% perform write
\textbf{Protocol actions.}
A machine that performs a write to a key-value pair increments its Lamport clock and transitions the key-value pair to a transient  \textit{Write} state; then it broadcasts invalidations that include the key, its Lamport clock and its own machine id. Similarly to the Eventual Store protocol, the machine id and the Lamport clock compose the timestamp of the invalidation (i.e. the unique id of the write).

% receive invalidation
When a machine receives an invalidation, it compares the timestamp of the invalidation with the stored timestamp. If the received timestamp is greater, then the machine transitions the state of the key to \textit{Invalid} and responds to the writer with an acknowledgment message. Alternatively, if the received timestamp is smaller than the stored timestamp, then the receiver discards the invaldiation and does not respond to the machine. The reason why no response is required in that case, is simple: if one server has seen a write, sooner or later all servers will see the same write, more importantly, if one server thinks that timestamp A is greater than timestamp B, then all servers agree on that comparison. Therefore a negative acknowledgement would be redundant: the sender of the invalidation, is guaranteed to see an invalidation for the stronger write and will transition to an \textit{Invalid} state.

% receive acknowledgement
When a machine receives an acknowledgement, it increments a counter that holds the received acknowledgements for the relevant key. When the counter indicates that all machines have acknowledged the invalidation, then the server transitions the key to a \textit{Valid} state and broadcasts an update message with the new value and the write's timestamp to all of the machines. 

%receive update
Upon receiving an update, a server will check whether the relevant key is currently in \textit{Invalid} state and it waits for that particular update. To verify the latter, the server checks if the stored timestamp is equal to the received timestamp. if both conditions hold true, the update is applied and the key transitions to \textit{Valid} state, otherwise the update is discarded. Either way, the server never responds to receiving an update.

This protocol is similar to work done by Guerraoui et al \cite{Guerraoui:2007}. We specify all the transient states of the protocol and we have verified its correctness with a model checker.
%At that point there two possible outcomes. The first is that writer will receive an acknowledgment from every machine in the system, in which case it will commit the write and it will broadcast the new value to all machines The second case is that another "stronger" write has happened concurrently or it will receive an invalidation with a higher Lamport clock (or machine id, in case the Lamport clocks are equal) in which case it will cancel its write,  it will traverse the key to a transient 'Invalid' state and it will respond to the writer with an acknowledgement. 

\end{comment}

==> Text/5-ccKVS-SC/6-Design.tex <==
\tsection{ccKVS}
\label{secC:design}

In order to understand the benefits and limitations of the proposed Scale-Out ccNUMA architecture, we build ccKVS, an in-memory RDMA-based distributed key-value store which combines a NUMA abstraction~\cite{Dragojevic:2014} %\boris{or black box?? We should probably drop black box from the paper.} \antonis{It's the same we should just choose one}
with the consistent symmetric cache. The code of ccKVS is available online.\textsuperscript{\ref{footC:link}}

Each node in ccKVS is composed of two entities: a shard of the KVS and an instance of the cache; each of the entities has an object store and a dedicated pool of threads for request processing. As described in Section~\ref{secC:cache}, the content of all caches is identical, composed of the most popular items in the dataset. The caches are kept consistent using the fully-distributed protocols described in Section~\ref{secC:protocols}. The nodes of a ccKVS deployment are connected via RDMA with two-sided primitives used for communication. Clients load balance their requests (both reads and writes) across all nodes in a ccKVS deployment, e.g., by picking a server at random or in a round-robin fashion.

\tsubsection{Functional overview}
\label{secC:overview}
% \vasilis{there has been no discussion about cache-threads so far, they are introduced later in thread partitioning}
{\bf Reads:}
When a client request arrives at a ccKVS server, the server probes its instance of the symmetric cache. If the requested key is found, the associated object is retrieved from the cache and the server directly responds to the client. In case of a miss, the server determines whether the key belongs to a local or remote KVS partition. If remote, the server issues a remote access to the server containing the requested key using a two-sided RDMA primitive. On the destination side, the server picks up the remote access and responds with the data to the requesting server. Once the object is available, either by virtue of being in the local partition or through a remote access, the server handling the request responds to the client. 

%In ccKVS, a read request is served as follows: a client issues a request, which according to a load balancing method (e.g. round-robin) is dispatched to a server. The server receives and propagates the request through its symmetric cache. For the majority of the requests that hit in the cache, the server directly responds to the client; otherwise it locates the home node of the requested data item. The home node can be either the same server that received the request or, more commonly, a remote server. If the former is true, the server probes its own KVS partition and responds back to the client. Alternatively, if the data item resides in another node, the server issues a low-overhead RDMA request to the home node. Finally, the home server that receives the request does not probe its own cache, rather it immediately accesses its portion of the KVS to serve the request. 


\noindent{\bf Writes:}
Similar to reads, write requests are also load balanced across all nodes in a ccKVS deployment, thus avoiding write-induced load imbalance. If the write request hits in the cache, the server handling the request executes the steps necessary to maintain consistency across all symmetric caches in accordance with the chosen consistency protocol. In brief, for the SC protocol, this means immediately propagating the new data to all of the caches, whereas for the Lin protocol, it requires first invalidating the caches and then propagating the new data. Regardless of the protocol, the communication required for maintaining consistency relies on two-sided RDMA primitives. 
If the write request misses in the cache, the server forwards it to the home node (if remote), which performs the write. 
%\antonis{add a sentence about what happens on eviction.}

% An important feature of Scale-Out ccNUMA implemented in ccKVS is that the caches are write-back. 
% \boris{Is it an important feature of SO-ccNUMA, Symmetric caching, or ccKVS? If either of the former, this information should appear in the respective sections (Sec 3 or 4). Only information specific to ccKVS should be here.}
% This means that writes to an item residing in the symmetric cache do not update the KVS until the item is evicted from the cache. This feature is critical in avoiding a throughput degradation at the home node of a popular object whenever writes follow a skewed distribution. Because all caches maintain the same set of objects in the cache, on eviction, only the node containing the shard with the evicted key needs to check if the object has been modified and, if so, update the KVS. 
%\antonis{Aren't we sending the writes to every server? + our resilience point is that the write is propagated somehow to the KVS which could have its own (replication?) mechanism for fault tolerance}
% LIFE OF A REQUEST

%\input{Miscellaneous/Fig_Design.tex}



\tsubsection{Cache and KVS Implementation Details}
\label{secC:design-cache-kvs}

%\boris{changed the sec title - added Implementation Details}

% \vasilis{Changed the sections "Thread Partitioning" and "Skew-Aware Concurrency Control" to replace EREW with CRCW}
% CACHE AND KVS THREADS
\noindent
\textbf{Thread Partitioning.}
 %\boris{I believe this paragraph is entirely subsumed by the read/write overview above. On the other hand, if the inter-thread communication is messy (which it might be based on what you just told me), then may be simplify that discussion and keep this para.}
%  \vasilis{this is my question exactly.... should we keep this or take it above?}
The threads inside a machine in ccKVS are partitioned into two pools: cache threads and KVS threads. 
The cache threads receive the requests from the outside clients and are responsible for the cache accesses. % \boris{Accesses are not symmetric. The cache is. Order of words matters.} accesses to the symmetric cache.
The back-end KVS is handled by the KVS threads; thus, in case of a cache miss the request must be propagated from a cache thread to a KVS thread (local or remote). Finally, the cache threads also communicate with each other to exchange consistency messages: updates in SC;  invalidations, acknowledgements and updates in Lin. Notably, the KVS threads do not communicate with each other.

\noindent
\textbf{Concurrency Control.}
Among the cache threads (threads responsible for servicing requests to the most popular items in the request stream) ccKVS leverages the Concurrent Read Concurrent Write model (CRCW): any cache thread can read or write any item in the cache. Despite the mandatory  synchronization overheads, we find that this design maximizes throughput given the demand for the most popular keys in the dataset. 

%\boris{I reworked this paragraph}
The KVS design is more involved. Conventional wisdom~\cite{Lim:2014} is that when the requests are load balanced across all machines, it is beneficial to partition the KVS at a core granularity (i.e. Exclusive Reads Exclusive Writes - EREW) to avoid inter-thread synchronization on data accesses. Our design, however, employs the CRCW model for the KVS, despite the fact that, with the skew shaved by the caches, KVS accesses enjoy an access distribution that closely approaches uniform. 

%\sout{This is} \boris{Don't use This.}
The reason we choose CRCW is that %\sout{because, even though the CRCW model mandates the usage of a locking scheme,} 
it allows us to minimize the connections among the cache threads and the KVS threads in the deployment. Our experiments show that this is a favourable design choice, as the benefits of limiting the connectivity, among threads on different machines, trump the overhead of the concurrency control in CRCW. We elaborate on these benefits in section~\ref{secC:design-perf}. Finally, the CRCW concurrency model in KVS increases the ability of cache threads to batch multiple requests in a single packet, alleviating  network-related bottlenecks. We explore the benefits of this optimization in section~\ref{secC:coalesc-perf}.




\begin{comment}
% CACHE AND KVS THREADS
\noindent
\textbf{Thread Partitioning.}
 %\boris{I believe this paragraph is entirely subsumed by the read/write overview above. On the other hand, if the inter-thread communication is messy (which it might be based on what you just told me), then may be simplify that discussion and keep this para.}
%  \vasilis{this is my question exactly.... should we keep this or take it above?}
The threads inside a machine in ccKVS are partitioned into two pools: cache threads and KVS threads. 
The cache threads receive the requests from the outside clients and are responsible for the symmetric cache accesses. The back-end KVS is handled by the KVS threads; thus, in case of a cache miss the request must be propagated from a cache thread to the appropriate KVS thread (local or remote). More precisely, since the KVS is partitioned at a per-core granularity (i.e. EREW), each cache miss needs to be sent to the specific KVS thread that has access to the requested key. Finally, the cache threads also communicate with each other for exchanging consistency messages: updates in per-key sequential consistency;  invalidations, acknowledgements and updates in per-key Linearizability. Notably, the KVS threads do not communicate with each other.

\noindent
\textbf{Skew-Aware Concurrency Control.}
ccKVS utilizes a hybrid concurrency control approach. Among the cache threads, which are responsible for servicing requests to the most popular items in the request stream, ccKVS leverages the Concurrent Read Concurrent Write model (CRCW): any cache thread can read or write any item in the cache. Despite the required synchronization overheads, we find that this design maximizes throughput given the demand for the most popular keys in the dataset. Meanwhile, with the skew shaved by the caches, KVS accesses enjoy an access distribution that closely approaches uniform. Given that, KVS threads employ the EREW model that has been shown to be superior for a balanced access distribution~\cite{Lim:2014}


% \noindent 
% \textbf{CRCW.} 
% We identify the CRCW(Concurrent Reads Concurrent Writes) organization as the best candidate for the symmetric cache. In other words, each cache-thread has both read and write access for all items of the symmetric cache. The conventional wisdom, when dealing with skewed access pattern, is to disallow concurrent writes by opting for a CREW organization, where each thread can read all the data items but can write only its dedicated subset of them. CREW is typically preferred because it has less stringent synchronization demands\cite{Li:2016}, since it does not need to arbitrate between concurrent writes, which is intuitive since writes to the same data can never happen in parallel, anyway. 

% Applying CREW in our symmetric caches would require incoming writes to be steered to particular cores, or even worse the cores would have to send the writes as RPCs within the same machine, using shared memory communication. Additionally, the core responsible for writing the hottest partition would be heavily imbalanced, as it would have to issue and accept all coherence traffic for that partition, limiting the performance of the system. By using CRCW, we avoid load imbalance and complexity, all together, while we introduce a very lightweight locking primitive to minimize the synchronization overhead.


%\vijay{There is a tension between synchronization overhead and skew tolerance: with EREW there is no synchronization overhead but suffers from skew; it is the opposite with CREW. With our Skew-aware concurrency control we achieve best of both worlds. We use CREW for the symmetric cache which is going to be highly contended; having filtered the skew, we use EREW for the backend KVS. In the following we discuss the details of our implementation.}

%Inside a single node concurrency for an object can be offered through efficient synchronization methods. Modern data-serving systems [19, 18] utilize optimistic concurrency control to offer concurrent (lock-free) reads,which increase the performance in the presence of skew. Nevertheless, a recent study[35] argues about the cost of synchronization and proposes to partition the address space in core granularity instead of a node. Despite the fact that this technique leads to exclusive reads and exclusive writes(EREW) model, which performs poorly with a skewed workload, it totally eliminates the requirement of synchronization, thus it can achieve better performance in the ideal case of uniform workloads.

%ccKVS exploits the fact that the most popular objects are decoupled from the rest of the dataset, implementing the  synchronization scheme that we call \textit{Skew-aware Concurrency Control}. Specifically, the symmetric cache, which serves the hottest keys is efficiently shared among multiple threads; utilizing efficient synchronization methods that enable  concurrent (lock-free) reads. On the contrary, the back-end (KVS) system, which receives requests only for cold objects, can leverage the core-granularity dataset partitioning (i.e EREW), similarly to \citep{Lim:2014}, to avoid any synchronization costs. Consequently, an object according to its  popularity  can  be  benefited  either  by  the  lack  of synchronization overheads or by the concurrency offered in the caches. 
\end{comment}
To ensure high read/write performance under the CRCW model, ccKVS synchronizes accesses using \textit{sequential locks} (seqlocks)~\cite{Hemminger:2002, Lameter:2005}, which allow lock-free reads without starving the writes. 
The seqlock is composed of a spinlock and a version. The writer acquires the spinlock and increments the version, goes through its critical section,  increments the version again and releases the lock. Meanwhile, the reader never needs to acquire the spinlock; the reader simply checks the version right before entering the critical section and right after exiting. If in either case the version is an odd number, or if the version has changed, then a write has happened concurrently with the read and thus the reader retries. 

The seqlocks are implemented in the header of each object. The header contains a version number that has a dual role: it is used both to implement seqlocks and as the Lamport clock for the consistency protocols. Therefore, we only need to add one Byte to the header to implement the spinlock. 
%Accesses to the symmetric cache are synchronized through \textit{sequential locks}(seqlocks)~\cite{hemminger:2002, lameter:2005} that allow lock-free reads without starving the writes. 
%\vijay{I feel we are going a bit detailed here -- candidate for editing.}\vasilis{edited}
%A seqlock is composed of a spinlock and a version, both of which we implement in the header of each object. %\boris{could we use ``object'' from here onward? Objects have headers; values are just numbers.}. 
%We implement the version by overloading the header field that contains the Lamport clock, required by both of our consistency protocols. Therefore, we only add one more byte to the header for the spinlock. 
Our seqlock implementation is inspired by the OPTIK design pattern~\cite{Trigonakis:2016}.

%


All consistency messages are treated as writes, as they need to modify metadata in the header of the key-value pair. Meanwhile, reads to the cache do not modify state and thus they happen ``lock-free'' and in parallel. 



%On the contrary, the back-end system, which receives requests only for cold objects, can leverage the core-granularity dataset partitioning or EREW architecture, similarly to \citep{Lim:2014}, to avoid synchronization costs. As a result, an item that is initially cold is served fast by a single core without any synchronization costs, and once its popularity reaches a threshold, it is replicated and moved on the symmetric caches, where lock-free reads provide higher concurrency and increase performance.

%Traditional implementations of data-serving applications apply common fine-grain locks to handle synchronization. Although this ensures correctness and enables any core to serve a request for a local object, it does not allow concurrent requests for the same item to proceed; instead it serializes them. Consequently, in the presence of skewed accesses, such systems consume multiple cores in order to serve requests for hot keys serially.

%However, inside a single node concurrency for an object can be offered through efficient synchronization methods. Modern data-serving systems \cite{Fan:2013,Dragojevic:2014} provide concurrent (lock-free) reads that benefit the performance in the presence of skew. Nevertheless, a recent study\cite{Lim:2014} argues about the cost of synchronization and proposes to partition the address space in core granularity instead of a node also known as exclusive reads and exclusive writes (EREW). Despite the fact that this technique limits the concurrency, and thus performing poorly with a skewed workload, it eliminates the requirement and cost of synchronization. Consequently, it can achieve better performance in the ideal case of uniform accessed workloads.

%{\bf Skew-aware Concurrency Control:}
%One more benefit of symmetric caching is that it enables the architecture of systems, with the synchronization scheme, that we call \textit{Skew-aware Concurrency Control}. This attribute achieves the best of both worlds, by exploiting the fact that the most popular objects are decoupled from the rest of the dataset. Therefore, caches, which are benefited by concurrent accesses since they serve the hottest keys,
%utilize sequential locks (seqlock)\vasilis{maybe this should not be here after all}  to enable 
%provide lock-free parallel reads, within multiple cores. 
%the CREW architecture.
%On the contrary, the back-end system, which receives requests only for cold objects, 
%can leverage the core-granularity dataset partitioning or EREW architecture, similarly to \citep{Lim:2014}, to avoid synchronization costs. As a result, an item that is initially cold is served fast by a single core without any synchronization costs, and once its popularity reaches a threshold, it is replicated and moved on the symmetric caches, where lock-free reads provide higher concurrency and increase performance.


% \vasilis{Changed the subsections "Symmetric Cache" and "KVS" to reflect reviews and CRCW}

\noindent
\textbf{KVS.}
 We use MICA~\cite{Lim:2014} as a state-of-the-art KVS and leverage the source code for EREW found in \cite{Kalia:2016} to build our KVS. Since ccKVS adopts the CRCW model, the KVS is concurrently accessed by all KVS threads; therefore, we implement seqlocks over MICA. Our evaluation considers both EREW and CRCW design choices.
 Finally, we note that Scale-Out ccNUMA and symmetric caching are not tied to any particular KVS.
 %and can be applied over any existing KVS. 
 %Notably the structure of the KVS is orthogonal to Symmetric Caching, which can be deployed as effectively over any existing KVS.

\noindent
\textbf{Symmetric Cache.}
%The symmetric cache is a data structure that is concurrently accessed by all the cache threads within a node;
%it inherits its structure from EREW MICA (as found in \cite{Kalia:2016}), on top of which, we have implemented the synchronization (i.e. seqlocks) to convert it to CRCW. 
The symmetric cache is a data structure that is concurrently accessed by all the cache threads within a node; it inherits its structure from our KVS (and thus by extension from MICA \cite{Lim:2014} %\boris{why are you citing this and not [32]?} \vasilis{they made the C code available in the Herd project...}
), and also implements appropriate support for SC and Lin. We extend the KVS's API and functionality to provide support for the consistency protocols (i.e. stable and  transient states) and the consistency related operations (i.e. updates, invalidations and acknowledgments). For example, a read request under Lin may hit in the cache but it may not succeed, if the key-value pair is in Invalid state.

Each key-value pair stored in the cache has an 8B header, where the necessary metadata for synchronization and consistency are efficiently maintained. The metadata include: the consistency state (1B, only used in Lin), the version (i.e. Lamport clock, 4B), the id of the last writer (1B), a counter for the received acknowledgements (1B, only used in Lin) and the spinlock required to support the seqlock mechanism (1B). 

%Each value stored in the cache contains a 16B header that consists of its key (8B) and the necessary metadata for synchronization and consistency actions that is efficiently squeezed in the remaining 8 bytes.The metadata include: the consistency state (1B -only used in per-key Linearizability), the version (i.e. Lamport clock-4B), the id of the last writer (1B), a counter for the received acknowledgements (1B-only in per-key Linearizability) and the spinlock required to support the seqlock mechanism (1B). 




%Each KVS thread owns its own portion of the EREW KVS and uses the API provided by MICA to propagate the requests and receive responses from it. % that miss in the symmetric cache.
%We build ccKVS on top of MICA, taking advantage of optimizations like software prefetching and core-granularity partitioning. 


\begin{comment}
\noindent
\textbf{Symmetric Cache.}
The symmetric cache is a data structure that is concurrently accessed by all the cache threads within a node;
it inherits its structure from MICA, but it also implements appropriate support for consistency and synchronization (using seqlocks). Each value stored in the cache contains a 16B header that consists of its key (8B) and the necessary metadata for synchronization and consistency actions that is efficiently squeezed in the remaining 8 bytes. 

%The metadata include: the coherence state (1B -only used in per-key Linearizability), the version (i.e. Lamport clock-4B), the id of the last writer (1B), a counter for the received acknowledgements (1B- only in per-key Linearizability) and the spinlock required to support the seqlock mechanism(1B). 



\noindent
\textbf{KVS.}
The structure of the KVS is orthogonal to our work, as Symmetric Caching can be deployed as effectively over any existing KVS. We identify MICA as a state-of-the-art KVS and we utilize the source code for EREW found in \cite{Kalia:2016} to build our KVS. Each KVS thread owns its own portion of the EREW KVS and uses the API provided by MICA to propagate the requests and receive responses from it. % that miss in the symmetric cache.
%We build ccKVS on top of MICA, taking advantage of optimizations like software prefetching and core-granularity partitioning. 
\end{comment}

\tsubsection{Communication Layer} \label{secC:communication}

\noindent
\textbf{RDMA.}
There are two prevalent techniques to build an RDMA-based KVS: (i) using RDMA Reads via one-sided primitives, similar to FaRM \cite{Dragojevic:2014} or (ii) with Remote Procedure Calls (RPCs) over Unreliable Datagram Sends (UD Sends) similarly to FaSST~\cite{F-Kalia:2016}. We choose the more general RPCs over UD Sends approach, but note that the Scale-Out ccNUMA paradigm is not constrained by the choice of the communication primitive and could equally work with one-sided accesses. For convenience, we utilize the elegant RDMA wrappers built by Kalia et al. in \cite{Kalia:2016}, modifying them wherever more fine-grained control is required.

%, as we believe them to be a better-suited paradigm for the KVS requirements. Additionally, the RPCs can be used irrespective of the KVS implementation, allowing us to adopt a state-of-the-art legacy KVS (i.e. Mica). However, we note that the Symmetric Caching technique would be equally effective with either choice, as it is completely orthogonal to the communication primitives.

%RDMA requires a fat initialization phase to initialize all Queue Pairs, and exchange the necessary information between all nodes, to commence communication. We utilize the elegant RDMA wrappers built by Kalia et al. in \cite{Kalia:2016} to implement this layer, modifying them wherever more fine-grained control is required.


% We acknowledge the fact that RDMA Reads are very promising, but we believe that the RPCs are a better-suited paradigm for the KVS. 
 %The RPCs  and secondly
%Unlike RDMA Reads, RPCs do not impose any constraints on the implementation of the KVS\cite{Su:2017} allowing us to leverage a legacy KVS.\vasilis{RPCs are orthogonal to the KVS implementation, RDMA Reads are not: they need specific hash structure, specific per-key and per-data metadata. I guess since we are not discussing these stuff, we should not imply them either  } 
%We also utilize the open source  RDMA wrappers , on top of which we build our communication.


%Partitioning the threads with respect to their responsibilities and then limiting the connectivity between the system's threads, alleviates the all-to-all communication pattern within the black box, offering scalability with respect to RDMA concerns.




%In comparison to the CREW optimistic concurrency control implemented in Mica, the seqlocks only incur a small penalty of locking, when performing writes and a trivial space overhead (1B per key) for the lock; meanwhile the reads have the exact same software stack.

\noindent
\textbf{Flow Control.}
The communication between cache threads and KVS threads is facilitated by a credit-based flow control mechanism~\cite{Kung:1994}. The cache threads have a number of credits for each remote KVS thread, and the KVS threads have a matching amount of buffer space for each remote cache thread.  Each time a cache thread sends a request, the credits for the receiving KVS thread are decremented. Similarly, the credits are incremented whenever the KVS responds.
%a response from the KVS is received. 
%Therefore the cache threads always have enough information about buffer availability for all KVS threads. 
Because a request always receives a response, the flow control does not require additional credit update messages; the responses to the requests are implicitly used as credit update messages.


In contrast, the communication between cache threads on consistency actions requires explicit credit updates because not all messages receive a response. For example, a cache thread that broadcasts updates to all other machines does not receive acknowledgements for those updates. Thus, ccKVS uses explicit credit update messages to inform cache threads of buffer availability across the symmetric cache nodes. 
%and thus, without credit update messages, the cache thread would have absolutely no information about the buffer availability in all destinations.
%Consequently, ccKVS uses a credit-based flow control mechanism for the consistency traffic, such that each type of consistency message has dedicated credits and buffers devoted to it, with explicit credit update messages used to . Therefore, in addition to the coherence messages, the client-threads must also exchange credit update messages, to alert each other about their buffer availability. 
Section~\ref{secC:design-perf} describes optimizations to alleviate the network bandwidth overhead of credit updates. 


\begin{comment}
\vasilis{Added the sections "Large Payloads", I consider it prime candidate for removal, if we need space}
% Less verbose variation
\noindent
\textbf{Large Payloads.} 
In section~\ref{secC:value-perf} we demonstrate the performance of ccKVS when the size of the key-value pairs is increased (up to 1KB). Larger key-value pairs mandate larger RDMA message payloads, which alter the semantics of posting send work requests to the NIC (i.e. ibv\_post\_send()) from synchronous to asynchronous, as inlining must be disabled with payloads larger than a threshold (188 Bytes in our infrastructure). Interestingly, that detail changes the buffer space recycling pattern: to reuse a buffer slot there must be a guarantee that the NIC has read the stored message. That guarantee is not provided by ibv\_post\_send(), when inlining is disabled.

In response, we fine-tune our buffer recycling policy to match with the inlining policy, such that we can take advantage of the synchronicity when inlining is enabled and minimize the buffering overhead when inlining is disabled. Naturally, the same approach must be employed when coalescing requests/replies in a single message.



% Verbose Variation
\noindent
\textbf{Large Payloads.} 
In section~\ref{secC:value-perf} we demonstrate the performance of ccKVS when the size of the key-value pairs is increased (up to 1KB). Larger key-value pairs mandate larger RDMA message payloads, which bring about an interesting side-effect in the behaviour and the performance of the RDMA layer: inlining must be disabled when the payload of the message surpasses a threshold (188 Bytes in our infrastructure). The meaning of that is that the payload of the message is not inlined inside the Work Queue Element(WQE), but rather the WQE contains a pointer to the payload, that the NIC will use to issue DMA Reads for the payload. That means that the buffer that holds the payload must be registered with the NIC, increasing the pressure on the NIC's TLB and the IOMMU.

More importantly that alters the semantics of the sending function(i.e. ibv\_post\_send()), which forms the WQEs and makes sure that the NIC has received them. When inlining is disabled, ibv\_post\_send() is no longer synchronous, as the payloads are not included in the WQEs, rather the NIC asynchronously issues DMA Reads for the payloads after the function has returned. Interestingly, that small detail changes the buffer space recycling pattern: to reuse a buffer slot there must be a guarantee that the NIC has read the stored message. That guarantee is not provided by ibv\_post\_send(), when inlining is disabled. In response we fine-tune our buffer recycling policy to match with the inlining policy, such that we can take advantage of the synchronicity when inlining is enabled and minimize the buffering overhead when inlining is disabled. Naturally, the same approach must be employed when coalescing requests/replies in a single message.
\end{comment}


% \vasilis{Changed the section "Broadcast Primitive" to reflect new knowledge}
\noindent
\textbf{Broadcast Primitive.} 
To facilitate both protocols we implement a software broadcast, where the sender prepares and sends a separate message to each receiver. The application sends a linked list of work requests to the NIC as a batch; all work requests point to the same payload but each work request points to a different destination (i.e. Address Handle). When a cache thread intends to send more than one broadcast, we batch these broadcasts together to the NIC to amortize the PCIe overheads. 

% \vasilis{specified that this is only for SC, since we make the code public}
We also implement the broadcast primitive for SC using the RDMA Multicast, but do not observe any benefit. The semantics of the RDMA Multicast are that the sender node transmits a single message to the switch and the switch propagates it to all registered recipients. %The result from using RDMA Multicast was very unexpected:
%even though, ccKVS is bottlenecked by the network, and RDMA Multicast decreases the overall network utilization, we found that RDMA Multicast is not beneficial for ccKVS. 
%The reason is simple: 
Therefore, RDMA Multicast optimizes the send side, but the bottleneck persists in the receive side.  %Therefore, when using RMDA Multicast the machines decrease their send bandwidth utilization, but their receive bandwidth utilization stays constant. 
Thus, although machines have available send-bandwidth to send additional messages, they are still bandwidth-limited on the receive side. 
%\boris{I don't think we need the following sentence. I suggest removing:}
In practice, using RDMA Multicast slightly decreases ccKVS performance; we attribute this decrease to the switch's multicast implementation overheads.
%\vasilis{The reason I 'd like to have this, is because it is the actual result from implementing multicast. }

%In principle, while the network is the bottleneck, RDMA Multicast cannot yield better results than our software Broadcast. In practice, using RDMA Multicast slightly decreases performance; we attribute this decrease to the switch's multicast implementation overheads.% \antonis{Would it be better to replace send and receive bw with ingress and egress?}


\begin{comment}
\noindent
\textbf{Broadcast Primitive.} 
In this work we do not make use of the RDMA multicast primitive to maintain portability with RDMA deployments with switches that do not support the operation. Instead, we implement a software broadcast, where the sender prepares and sends a separate message to each receiver. The application sends a linked list of work requests to the NIC as a batch; all work requests point to the same payload but each work request points to a different destination (i.e., Address Handle). When a cache thread intends to send more than one broadcast, we batch these broadcasts together to the NIC to fully amortize the PCIe overheads. We note that our technique will be improved by applying the RDMA multicast, and thus, by not using it we take a more conservative and portable approach.\vasilis{we now know that is not true}
\end{comment}






% THIS IS COPY & PASTE FROM OUR CITATION
%Seqlocks are the most scalable form of locks that is useful if there are a large number of readers. The readers do not need to write to memory at all to handle this type of “lock”. Maybe one should not talk about acquiring a lock at all. Readers compare a counter before and after a critical section. If the counter did not change in the critical section then no writer was active and the outcome produced by the critical section is valid. If it has changed then the results of the critical section is discarded and it is run again

%A seqlock contains a spinlock which is used for mutual exclusion between writers. Writers increment the counter once on lock acquisition resulting in an odd count value. The readers know that the writer is in the critical section if they encounter an odd value and rerun the critical section. Writers increment the counter again on unlock so that it becomes even


% CIRCULAR BUFFERS
%Cold requests that can be served by the local portion of the KVS are communicated to the responsible KVS node through shared memory: each KVS thread maintains a circular buffer for each local cache-thread. Cold remote requests are sent to the appropriate remote KVS-threads through RDMA UD Sends. Each KVS thread maintains a single circular buffer for remote requests. The KVS-thread maintains a push pointer for that circular buffer, that it uses to post RDMA Receives, and a pull pointer that it uses to poll for new requests. A cache-thread is allowed a fixed number of outstanding requests for each remote KVS-thread in the deployment. That number determines the size of the circular buffer and the required posted RDMA Receives.

% EXAMPLE CIRCULAR BUFFERS AND RDMA RECEIVES
%For example let's assume a 9-machine deployment, with 5 cache-threads and 5 KVS-threads in each machine, where each cache-thread is allowed 10 outstanding requests for each remote KVS-thread. Therefore each KVS-thread needs a circular buffer that can store 10 requests for each remote cache-thread; given that for each KVS-thread there are 40 remote cache threads, the size of the circular buffer must be at least 400 slots. The size of each slot is determined by the maximum size of a value similarly to Herd\cite{Kalia:2014}. 

% RDMA RECEIVES -PUSH POINTER
%This a sub-optimal practice that will cause serious fragmentation to the circular buffer; for example a read request only requires a handful of bytes, but it will be stored in a slot that can store a write request that can be in the order of kilobytes. 
%This problem exists, because the application needs to handle the push pointer of the circular buffer and it must post RDMA receives in advance that point to the next slot on the circular buffer. However, it is impossible to predict the size of future requests when posting Receives, and thus we have to assume the worst case. However, we believe that future NICs will solve this problem: the hardware can maintain the push pointer to the circular buffer and thus increment it knowing the size of the incoming message.




%\textbf{RDMA Read.} The biggest issue is that it is very challenging to read a remote key-value pair with a single RDMA Read. There are two reasons behind that: firstly in a hashtable it is not possible for the reader to know the exact location of a key-value pair; typically locating a key-value pair requires multiple reads. Therefore to read a remote key with RDMA Reads from a remote memory the server would have to issue multiple serialized RDMA Reads. 

%Secondly atomically reading a piece of data is also a challenge: some form of concurrency control is required to ensure that the host is not writing the data concurrently with an RDMA Read. Both locking and lock-free mechanisms typically require more than one serialized accesses e.g.(lock, read, unlock).

%FaRM\cite{Dragojevic:2014} implements clever, albeit convoluted techniques to alleviate these problems. They manage to read a key-value pair with a single RDMA Read most of the time, if the key-value pair is sufficiently small. However, there are some costs, associated with these techniques. To avoid multiple round-trips locating a key, FaRM reads two buckets of the hashtable that are likely to contain the key, significantly increasing the network bandwidth consumption. Interestingly this makes, atomically reading the value in a single round trip even more challenging: to avoid multiple round trips to atomically read a key, FaRM implements per-cache -line versions within each bucket as well as cross bucket versions. This technique is very CPU-intensive \cite{Daglis:2016} and it introduces false sharing, as a write from the host can cause a concurrent RDMA Read to restart, even if the accesses are to different keys. Finally, FaRM's techniques require an application-specific implementation of the KVS, making it impossible to use a legacy KVS. This suggests that perhaps RDMA Reads are not the most suitable candidate.

%\textbf{Remote Procedure Call.} On the other hand RPCs allow us to take advantage of an existing optimized KVS. We build ccKVS on top of MICA taking advantage of optimizations like software prefetching and core-granularity partitioning. Herd proposes a flavour of RPCs where the clients issue requests over RDMA Writes and the servers reply with UD Sends, arguing that it is very lightweight for the server to receive RDMA Writes and issue UD Sends. However, this approach fails to account for the performance of the client. One-sided primitives struggle to scale as the required metadata (i.e. Queue Pairs) that the NIC must hold in its cache scale linearly with the number of machines in the deployment, thrashing the NIC's cache. Sharing the QPs introduces undesirable CPU overheads due to the required synchronization to access them \cite{Dragojevic:2017}.
%FaSST \cite{Kalia:2016} is a black box system that rectifies this oversight, building the RPCS entirely over UD Sends.

    %, or read a large memory area, that is likely to hold the requested key if the key-value pair is sufficiently small (for FaRM that is 6 times larger than the key-value pair).
    % Atomically accessing a key-value pair

    
     
    
    %to read atomically big chunks of data with a single RDMA Read. However Daglis et al.\cite{Daglis:2016} conclude that this mechanism is very CPU-intensive, accounting for 10 to 50\% of the total RDMA Read latency for objects 128B to 8KB. More interestingly this problem is exacerbated by the previous challenge: if an RDMA reads multiple key-value pairs to avoid multiple round trips, then concurrency control must be extended across keys, introducing more metadata and false sharing. Finally even if a key-value pair is known to be very small, 
%

%RDMA READ challenges
%1 Scalability of metadata sharing QPs incurs a large CPU overhead
%2 Registering Memory
%3 Batching
%4 Locating a key-value pair
%5 Handling concurrency
%6 Non portable KVS
%Even though the RDMA Reads and Writes make for a very intuitive building blocks, over which to design the KVS, we argue that when using them a number of problems that were not originally obvious arise. The first problem is the Queue Pair scalability, the one-sided primitives need to set up a large number of QPs as each thread of the system needs a separate QP for each remote machine. The efforts to reduce the QPs by sharing, results in reduce

%Implementation Details
% UD Qps 1-sided vs 2-sided-- doorbell batching/multiple qps per thread/inline
% cache-- sw prefetching/ state-based protocols/ locking mechanism
% lamport clock same as versioning 
% sequential locks with lock-free reads (inspired by linux)
% connectivity- tie with EREW and CRCW 
% thread separation
% flow control credit
% saying about the KVS & the cache threads
%\subsection{Symmetric Cache}
%\label{sec:design-cache}


\tsubsection{Performance Optimizations}
\label{secC:design-perf}

% \vasilis{Changed "Reducing Connections to reflect CRCW"}
\noindent
\textbf{Reducing Connections.}
%\boris{Problem: you never explain why cache threads need to communicate. It's obvious that a KVS miss on local node needs to talk to KVS on another node, but why do cache threads need to communicate?}\vasilis{It is mentioned above, where the previous paragraph ends, the point is for it to lead here.You think it's not clear enough?}
One of our goals in implementing ccKVS is to maintain RDMA scalability by limiting the number of threads that communicate with each other. Despite using the more scalable UD transport, all-to-all communication at the thread level can still prove challenging to scale because of the required buffer space and the posted RDMA Receives that scale linearly with connection count~\cite{F-Kalia:2016}.

Partitioning the threads (Section~\ref{secC:design-cache-kvs}) works toward limiting the extent of all-to-all communication, as KVS threads of different nodes do not need to communicate with each other. Additionally, we bind each cache thread to exchange messages with just two threads in each remote machine: one cache thread and one KVS thread. This optimization is enabled by the use of the CRCW model in both the symmetric cache and the KVS, since each thread has full access to the dataset (cache or KVS, respectively).
%, since each cache (KVS) thread has full access to the symmetric cache (KVS). 

Reducing the connections minimizes the required posted RDMA Receives and the required buffer space that is registered with the NIC. As discussed in section~\ref{secC:design-cache-kvs},  transitioning the KVS from the EREW to the CRCW model incurs a concurrency control overhead. However in our experiments we measure a performance increase of up to 10\% when employing CRCW instead of EREW, which we attribute to the reduction of the connections between cache and KVS threads. 
%This improvement underlines the importance of trade-offs that favour the system's bottleneck (which is the network in the case of ccKVS). 
%\vijay{candidate for cutting} As a side note, we point out that reducing the connections is possible under the EREW model, via an extra redirection step through shared memory. However, such additional communication between threads would incur a far larger overhead than adding a locking mechanism to the KVS. 
%This constraint incurs no performance penalty, since each cache thread has full access to the symmetric cache thanks to CRCW. In summary, a KVS thread communicates only with cache threads on remote nodes, while cache threads communicate with all remote KVS threads and just one cache thread in each remote node. 

\begin{comment}
\noindent
\textbf{Reducing Connections.}
%\boris{Problem: you never explain why cache threads need to communicate. It's obvious that a KVS miss on local node needs to talk to KVS on another node, but why do cache threads need to communicate?}\vasilis{It is mentioned above, where the previous paragraph ends, the point is for it to lead here.You think it's not clear enough?}
One of our goals in implementing ccKVS is to maintain RDMA scalability by limiting the number of threads that communicate with each other. Despite using the more scalable UD transport, all-to-all communication at the thread level can still prove challenging to scale because of the required buffer space and the posted RDMA Receives that scale linearly with connection count\cite{F-Kalia:2016}.

Partitioning the threads (Section~\ref{secC:design-cache-kvs}) works toward limiting the extent of all-to-all communication, as KVS threads do not need to communicate with each other. Additionally, we constrain each cache thread to exchange consistency messages only with one cache thread at each remote node. This constraint incurs no performance penalty, since each cache thread has full access to the symmetric cache thanks to CRCW. In summary, a KVS thread communicates only with cache threads on remote nodes, while cache threads communicate with all remote KVS threads and just one cache thread in each remote node. 
\end{comment}

\noindent
\textbf{RDMA optimizations.}
% Doorbell Batching- Selective Signaling- Multiple QPs- FINE-GRAIN sizes on QPS and SS-Batches
Using the UD transports allows us to perform opportunistic batching in all communication with the NIC to amortize the PCIe overheads. We post Receive and Send work requests as linked lists and notify the NIC about their existence through an MMIO write. The NIC is then able to read these requests in bulk, amortizing the PCIe overheads. In order to additionally alleviate PCIe overheads, we inline payloads inside their respective work requests, whenever the payloads are small enough (less than 189 Bytes), such that the NIC does not need a second round of DMA reads to fetch the payloads after reading the work requests.

We follow the guideline to use multiple Queue Pairs (QPs) per thread~\cite{Kalia:2016}; for example, a cache thread uses different QPs for the remote requests, the consistency messages and the credit updates.  
%\boris{can't follow the next sentence. What is ``fine- vs coarse granularity'' referring to?}
%\vasilis{It may seem intuitive to set a very big size to all queues, so that you dont have to reason about what is the maximum allowed size for each queue; that is the coarse grain approach(Herd does that), we found that actually setting the queues to the minimum makes a big difference.} \boris{OK, but then can you explain this better? Why don't you reference Herd and explain how your experience differs. Also, the text still does not make it clear what fine vs coarse grain means. Bottom line: either rework or drop. Current sentence is not useful.}\vasilis{drop sounds fine, this is too detailed anyway}
%We found that setting the maximum size for the different QPs to the minimum required at a fine-granularity can increase throughput up to 20\% compared to a coarse-grained conservative approach. 
Furthermore, we utilize the capability to use Selective Signaling when sending messages: the sender needs to poll for only one completion every time it sends a fixed-size batch of messages. We get additional performance by fine-tuning the Selective Signaling batches to match the size of the queues, such that one completion is created every time the Send Queue is filled.

%Additionally we note that many RDMA structures like the work requests for the receive requests, the credit requests and the broadcasts, do not require any changes after initialization. We save valuable CPU time by setting them up in the initialization, instead of assigning them every time they are used, but we note this as a weakness of the verbs API. In the case of simple requests like the work requests for the RDMA Receives or our credits, we expect future NICs to provide some mechanism that will alleviate the fact that the NIC needs to read from the PCIe the exact same message billions of times.
\noindent
\textbf{Flow Control optimizations.}
To prevent flow control from becoming an important factor in network bandwidth consumption, we apply a batching optimization on the credit updates: we do not send a credit update for each received message; rather, we send a credit update after receiving a number of consistency messages to amortize the network cost %\boris{cost is vague. Can you be more specific? Is it network bandwidth, CPU processing?} 
of the credits. Additionally, the credit update messages have no payload (i.e. they are header-only %\boris{again random capitalization. Why not ``header-only''?}
messages), reducing the required PCIe transactions and network traffic for sending and receiving them. In Section \ref{secC:eval} we show that through these optimizations the overhead of the credit update message becomes trivial.%We investigated the possibility of opportunistically piggybacking credits on coherence messages to save network traffic, but the complexity of the mechanism was not worth it, as the network overhead of credit updates is trivial.

 %We also note that the switch could perform a reduction technique to reduce the bandwidth consumption of the acknowledgements by gathering all acknowledgements and sending a single message to the writer

% \noindent
% \textbf{Batching. }
% Batching is a recurring principle in our design. In both the symmetric cache and the KVS, we make heavy use of MICA's multi-stage prefetching: we batch requests (reads, writes and coherence messages) taking advantage of the available Memory-Level Parallelism. 
% \vijay{The following sentence does not make sense - rephrase or remove}
% However, we only perform the batching opportunistically: a KVS-thread never waits to amass a fixed-size batch of requests to propagate to MICA. Rather, the KVS-thread polls its circular buffers where requests from local and remote cache-thread arrive and it forms a batch of as many requests as it could find such that the effect on the latency is the minimum.

\begin{comment}


\tsubsection{Resilience}
\label{secC:design-resil}
In building ccKVS, we do not implement logic to detect and recover from failures. However, Scale-Out ccNUMA is not constrained by the choice of KVS, so existing resilience mechanisms, such as the one proposed in FaRM~\cite{Dragojevic:2015}, can be readily applied. 

More generally, we note that the principal objective of this work is to demonstrate that aggressive caching with replication presents a performance opportunity even with strong consistency models. Nonetheless, we agree that there is interesting interplay between replication, resilience and the strength of the consistency model, which we leave for future work to explore. 
\end{comment}
%In the future, we intend to inspect the actions require by the symmetric caches in case of a failure. On this work, our purpose is to investigate the performance limits of caching, while providing various consistency guarantees and thus we do not tackle fault related problems.
%In case of a detected failure, the Symmetric Caching layer only needs to take action in per-key Linearizability. The state of cached items must be inspected to ensure no cache-thread waits on a coherence message from the failed machine. Additionally, the number of the required acknowledgments before broadcasting an update must be decremented.

%FaRM2 techniques
%leases, cluster membership configuration, log reply, re[plication of lost data




% OUR USE OF BLACK BOX - SYNERGY WITH CACHES- one sided no longer necessary
%The black box interface goes against the traditional KVS design, where a client must identify the owner of a key and communicate directly with him. That is a reasonable design choice if the cost of the extra hop is very expensive, which is the case with TCP/IP networks. However the fast interconnect within the KVS motivates an alternative architecture design. The black box design works synergistically with the hotness caches; most of the incoming requests may refer to remote keys but the server will still be able to serve most of them locally using the hotness cache. This alleviates the drawback of this design, which is the extra hop most requests would need if not for the hotness caches.


%\item Hierarchy \& All to All connections
%\item RDMA --> 2nd hop is cheap
%\item Discussion about the exploiting the free cores (explaining why there is compute availiable for caching)
%\end{itemize}




% - coherence messages are a function of writes and number of servers
% - for EC
% - for EC with broadcasts
% - SC
%  -SC with broadcasts

% \begin{itemize}
% \item distributed write serialization
% \item EC vs SC protocols over RDMA
% \item Break-even study
% \end{itemize}

\begin{comment}
\tsubsection{Perspective-Summary on design}
%Replication is required
%Caching by itself is not an effective solution to skew if it is not applied on a more powerful machine/component than the original. Thus,
In order to serve heavily skewed large-scale workloads it is required to store the hottest data items in more powerful components/nodes than the initial. The only way to get more powerful resources is to either have a heterogeneous architecture or by grouping homogeneous parts together.

Essentially, the goal of our design is to provide the required resources using a common homogeneous setup without adding any further nodes, but by exploiting existing underutilized components.
This architecture provides the illusion of a scale-up load balanced component, constitute by a group of collaborative nodes that serve requests for the most popular data items, while each individual component is still responsible for serving requests for its own cold items.
Our design leverages the black box architecture and Symmetric Caching, which combines the best attributes of caching and replication with our efficient consistency protocols to accomplish that.
% Multi-black boxes architecture
MATRIX with Benefits of our approach.
\end{comment}
%Others have pointed out that fine-grain partitioning (e.g. at core granularity) is the best thing for a uniform workload. However, the opposite holds true for skewed workload, since the more coarse grain partitioning is alleviating the problem.

% Fine Grain Partitioning ---> Uniform Performance
% Collaboration ---> Skewed Performance
% Enough CPU resources usually network bounded

% Heterogeneity
% Replication & protocols

% What is the best picture for our design
% Numa like rack ?
% Scale-up out of Scale-out ? 

==> Text/5-ccKVS-SC/7-Methodology.tex <==
\tsection{Methodology}
\label{secC:method}

In this section, we first present the designs that we evaluate and then describe our evaluation infrastructure. 

\tsubsection{Evaluated Systems}
%We evaluate ccKVS by comparing it with KVS based on a state of the art design: FaSST~\cite{Kalia:2016}. 
%
%We recognize that the purpose of FaSST is to provide high transactional throughput, rather than tackle skew, but still, we utilize its principles to build the best possible shared memory baseline system.

We evaluate \emph{Scale-out ccNUMA} by comparing it with a state-of-the-art skew mitigation approach based on FaSST~\cite{Kalia:2016}. 
%\sout{, that employs NUMA abstraction by leveraging low-latency RDMA-based interconnect}.
%To evaluate Symmetric Caching we compare and contrast its performance with state-of-the-art skew mitigation approach that employs NUMA abstraction by leveraging RDMA-based networking. 
%We evaluate FaSST \cite{F-Kalia:2016} as the state-of-the-art RDMA-based NUMA system; FaSST is an RPC-based NUMA system that is built on top of UD Sends and employs a number of RDMA optimizations~\cite{Kalia:2016}.
Although FaSST is designed for transaction processing, it has two key attributes that make it a good baseline for a system to tackle skew: it offers a NUMA abstraction like FaRM~\cite{Dragojevic:2014} and RackOut~\cite{RNovakovic:2016}, and it leverages several design techniques to achieve high performance using RDMA~\cite{F-Kalia:2016}.
We modify FaSST to implement efficient single-key Get and Put operations by stripping off all of the transaction processing overheads.
We apply all of our optimizations (discussed in Section \ref{secC:design-perf}) to maximize the performance of this baseline and negate any implementation-specific advantages of ccKVS. The performance of our baseline system is on par with the reported FaSST results (subject to different evaluation setups).
%\arpit{Discuss with Vasilis/Antonios and modify this paragraph}
%
%Indeed, each server in the baseline black box system completes an impressive 23.9 million requests per second (mrps) and it comes within 10\% of the performance of a server in the same system with uniform access pattern (26,7 mrps).\antonis{I don't know if we should stress this, but if we do we should be clearer that the first number is under skewed workload} 
%
\begin{comment}

\boris{please use a bulleted list and present these in the following order: Base, EREW, Uniform. For Base, please explain that it's CREW, which is expected to be the highest-performing model under skew. Also, don't use 'machine' - we never use it elsewhere. Use node or server. }
\vasilis{on it}
The first is \textbf{Base-EREW},  The second is \textbf{Base}, which has its KVS partitioned at a machine granularity. We expect this system to significantly mitigate the skew, but it will still be limited by its hottest server. In order to get the upper bound of Base, we do not implement any concurrency control mechanism for writes, which improves the performance of this design by eliminating synchronization overheads. We expect Base have no sensitivity to the write ratio due to the complete lack of synchronization overheads. Finally, \textbf{Uniform} represents the performance of  Base-EREW under a uniform distribution. This system will serve as the upper bound of our baseline.
\end{comment}
%
\\We evaluate three flavours of the FaSST-based baseline design:
%textbf{Systems:}More precisely, we modified the open-source code of HERD\cite{Kalia:2014} to create three different variations of such a baseline system:

\begin{itemize}
\item \textbf{Base-EREW}: has its KVS partitioned at a core granularity similarly to MICA~\cite{Lim:2014}. We expect this system to suffer under a skewed distribution as the performance will be limited by the core responsible for the hottest shard.
\item \textbf{Base}: has its KVS partitioned at a server-granularity (CRCW). Compared to Base-EREW, we expect this system to perform better under skew, while still being bottlenecked by the server with the hottest shard.  
%In order to get the upper bound of Base, 
%We do not implement any concurrency control mechanism for writes, which overestimates the performance of this design by eliminating synchronization overheads. 
\item \textbf{Uniform}: represents the performance of Base under a uniform distribution. 
This establishes an upper bound on the performance of baseline designs.
%This system will serve as the upper bound of our baseline designs.
%Same as Base-EREW but when running a workload with uniform access pattern (no skew). This design represents the upper bound on the performance of a KVS with NUMA architecture without symmetric caching.
\end{itemize}

%\boris{I reworked this paragraph.}
We build ccKVS by adding symmetric caches on top of Base. More specifically, we add a cache to each node and implement a system as described in Section~\ref{secC:design} that supports the SC and Lin consistency protocols specified in Section~\ref{secC:dist-protocols}. 
We refer to these variants of ccKVS as \textbf{ccKVS-SC} and \textbf{ccKVS-Lin}, respectively.
We configure the symmetric cache size to 0.1\% of the total dataset (250K objects of up to 1KB each, with overall memory footprint of up to 1GB). In accordance with Figure~\ref{figC:cache-opportunity}, the expected cache hit ratio is 46\%, 65\% and 69\% for skew exponents of $\alpha$ equal to $0.9$, $0.99$ and $1.01$, respectively.  
%We evaluate two flavours of ccKVS: \textbf{ccKVS-SC} that guarantees SC and 
%which is the ccKVS with per-key Sequential Consistency, and 
%\textbf{ccKVS-Lin} that guarantees Lin. 
%which is ccKVS with per-key Linearizability.


\tsubsection{Evaluation Setup} \label{{secC:method-setup}}
\textbf{Infrastructure:} We conduct our experiments on an isolated cluster of 9 servers interconnected via a 12-port Infiniband switch (Mellanox MSX6012F-BS). Each machine runs Ubuntu server 14.04 and is equipped with two 10-core CPUs (Intel Xeon E5-2630) with 64 GB of system memory and a single-port 56Gb Infiniband NIC (Mellanox MCX455A-FCAT PCIe-gen3 x16) connected on socket 0. Each CPU\ has 25 MB of L3 cache and two hyper-threads per core. %while it is accessing only the 32 GiB of memory that belongs into its own NUMA socket. 
We disable turbo-boost, pin threads to cores and use huge pages (2MB) for both the KVS and the cache.

%Hyper-threading
\noindent\textbf{Workloads:} 
%We emulate incoming client requests to the system using traces.
%\antonis{If someone can make this more elegant please go for it.} 
Our evaluation is performed on workloads that follow a Zipfian access distribution. We use the skew exponent $\alpha=0.99$ as the default value (as used in YCSB~\cite{Cooper:2010}) and also study $\alpha=\{0.90,1.01\}$. For comparison, we also assess a uniform access distribution. We evaluate both a read-only workload and workloads with modest write ratios,
%($w=\{0.2,1,2,5\}$ \%), 
which are representative of large-scale data serving deployments (e.g. Facebook reports a write ratio of $0.2\%$~\cite{Bronson:2013}).
The KVS consists of 250 million distinct key-value pairs, thus making each node responsible for nearly 28 million keys. Unless stated otherwise, we use keys and values of 8 and 40 bytes, respectively, thus allowing a direct comparison with FaSST~\cite{F-Kalia:2016}. Finally, we apply a request coalescing optimization only in Sections \ref{secC:bottlenecks}, \ref{secC:coalesc-perf} and \ref{secC:perf-vs-latency}.

%We use values of 32 bytes, which accurately represent and we keep the 8 byte keys   but we similarly use final values of 40-bytes

%\begin{itemize}
%\item Uniform
%\item 250 Million keys
%\item Skewed: Zipfian a=0.90, a=0.99, a=1.01
%\item write rate = 0\%, 0.2\%, 1\%, 2\%, 5\%
%\item Talk about load balanced writes
%\item our cache size is 0.1\% of the whole dataset
%\item Sizes: keys--> 16B, Values--> 32,64,128 B
%\item machines: 3,5,7,9(?)
%\item Protocols for consistency EC, SC, SC stalling(?)
%\end{itemize}
\begin{comment}


\\\textbf{Parameters:}
%\textit{Cache size}: 0.1\% of the black box dataset \\
\textit{Client threads}: are just issuing requests to the system according to an access distribution and a write rate.

\textit{KVS threads}: in all of the experiments we spawn and pin 9 KVS threads, that are required to saturate the NIC, in the same socket that the NIC is attached.

\textit{Cache threads}: (only in ccKVS) same as the client threads but which send the requests directly to the cache instead of the KVS threads.
\end{comment}
%which are required to saturate the NIC, in the NUMA socket 0 to reduce the communication overhead between the CPU and the NIC.
%is connected. 
%In the case of cache we collocate KVS threads and cache threads

%Each server is For the evaluation we use ccKVS KVS to create the black box abstraction using 9 servers. We evaluate our technique in a cluster of 9 servers.

%. We disabled turbo-boost and enabled hyper-threading CPU has ...
%CPU, hyperthreading, cache, dram, sockets, NIC + PCIe
%-Workloads
%--trace generation, in-memory

==> Text/5-ccKVS-SC/8-Evaluation.tex <==
\tsection{Evaluation}
\label{secC:eval}
\begin{comment}
The purpose of this section is to evaluate the performance of ccKVS, explore its benefits and understand its limitations. In section ~\ref{secC:read-only} we evaluate ccKVS in a read-only setting and in section ~\ref{secC:write-perf} its performance under writes. In section~\ref{secC:value-perf} we vary the key-vale size,  in section~\ref{secC:bottlenecks} we identify the systems bottlenecks, in section~\ref{secC:coalesc-perf} we introduce and evaluate a request coalescing optimization, in section \ref{secC:perf-vs-latency} we analyze the request latency within ccKVS  and finally in section ~\ref{secC:analytical} we introduce an analytical model, used to investigate the scalability of ccKVS.
\end{comment}
%-System Throughput

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/zipf_read_only_performance.pdf} 
  \caption{Throughput comparison for a read-only workload with varying skew. [9 nodes]}
  \label{figC:varying-skew}
\end{figure}

\tsubsection{Read-Only Performance}
\label{secC:read-only}

%\vasilis{we must change all references to symmetric caching to symmetric caches somehow}
We first evaluate the performance of all the designs for a read-only workload. Figure \ref{figC:varying-skew} shows the performance of Base-EREW, Base and ccKVS under three different skewed distributions ($\alpha = 0.9, 0.99, 1.01$). The results are similar for all three distributions and thus we focus our discussion on $\alpha = 0.99$.
%, which is the most common. 
% \vaslis{its a little weird to say that we show uniform under skew distributions}

As expected, Base-EREW has poor performance and achieves only 95 million requests per second (MRPS), as the whole system is bottlenecked by the throughput of the core responsible for the hottest shard. On the other hand, Base achieves 215 MRPS, significantly mitigating the skew, as the bottleneck shifts from the hottest core to the hottest server. 
%is limited by the network bandwidth of the hottest server as expected,
In fact, the performance of Base is within 10\% of Uniform, which achieves 240 MRPS.
It is worth noting that this performance gap is strongly correlated with the skew exponent ($\alpha$) and the number of servers in the deployment. %Indeed, the performance gap between Base and Uniform increases or decreases as the skew increases ($\alpha = 1.01$) or decreases ($\alpha = 0.90$).

ccKVS achieves 690 MRPS, which is $3.2 \times$ higher than the throughput of Base and $2.85 \times$ higher than Uniform. 
%The fact that ccKVS achieves a much higher throughput than Uniform highlights the fact that baseline systems are network limited. 
The significantly higher throughput of ccKVS compared to Uniform highlights the fact that the baseline systems are network limited.
ccKVS is able to achieve considerably higher throughput by avoiding the need to access remote nodes for cached objects, thus reducing network bandwidth pressure. 
ccKVS also benefits from the fact that symmetric caches allow all the nodes in the KVS to serve requests for hot objects, thus distributing the load evenly among them. 


\begin{comment}
\vasilis{paragraph as submitted}
ccKVS achieves the highest throughput of 690 MRPS which is $3.2 \times$ the throughput of Base. The high performance improvement of ccKVS is because of the symmetric caches that allow all the nodes in the KVS to serve hot requests, thus distributing the load evenly among them. The fact that ccKVS achieves a much higher throughput than Uniform also highlights that baseline systems are network limited. ccKVS is able to serve a significantly higher number of requests by filtering the network bandwidth of cached objects and trading it off for compute resources in terms of accessing and serving those requests from the cache.
\end{comment}

To better understand the reasons behind the significant performance improvement provided by ccKVS, we analyze its throughput. Figure~\ref{figC:break-down} shows the breakdown of ccKVS throughput in terms of the number of cache hits and misses for a read-only workload with varying skew.
In general, as the skew increases, the cache hit rate will also increase. 
Cache hits require compute resources, whereas cache misses mostly require network resources due to remote KVS access. 
We observe that the cache-miss throughput of ccKVS is equal to the entire throughput of Uniform and that the cache-miss throughput stays constant even though the cache miss rate is higher with lower skew exponents. This leads to the conclusion that both ccKVS and Uniform are network bound. Meanwhile, the cache hit throughput increases as the cache hit rate increases, which hints that CPU is not the bottleneck. We confirm these hypotheses in section~\ref{secC:bottlenecks}. % \boris{Great job on this paragraph!!}
 
%This leads us to the conclusion that ccKVS is also network bound.
%\antonis{Now that Figure 8 is eliminated we need to rephrase this.}

\begin{comment}
%Base Uniform and ccKVS are both limited by the processing power of the NIC. That is expected as the size of the messages is relatively small. 
%\arpit{Any evidence for this?}
%\vasilis{lets see what other guys do}
%The throughput of ccKVS is 690 MRPS and is limited by the rate at which cache misses are served.%, which is equal to the throughput of Base Uniform.
%Approximately 65\% of the total requests hit in the symmetric cache in ccKVS and thus the cache misses make up for 35\% of the total accesses. 
%Therefore, 65\% of the ccKVS throughput comes from the cache hits on the symmetric caches and the rest 35\% comes from serving the cache misses; The rate at which ccKVS serves the cache misses is equal to the throughput of Base Uniform, since the cache misses represent the accesses to the KVS which are mostly remote accesses that follow a uniform distribution.  This phenomenon can be observed more clearly by looking at all three distributions: the performance of ccKVS increases as the skew increases because the percentage of cache misses reduces. 


%\boris{what is the evidence for NIC processing being the bottleneck?} \vasilis{its not the CPU  because caching works, its not the PCI or NIc bandwidth because we get better with bigger objects. In other papers people tend to say "this is the bottleneck" and not give any proof(let alone definitive proof), just because it's so hard to do it, i dont know if we want to do that, but it's certainly an option. }

 %However Base CREW, where the KVS is partitioned at a machine-granularity, comes within 10\% of Base Uniform, achieving 215 MRPS. Base CREW is limited by the network bandwidth of the hottest server; 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.5\textwidth]{Figures/read_only_performance_overide_values.pdf} 
%   \caption{Read-only workload performance.}
% \end{figure}
\end{comment}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/request_breakdown.pdf} 
  \caption{Break-down of completed requests in ccKVS for a read-only workload with varying skew. [9 nodes]}
  \label{figC:break-down}
\end{figure}





%\vasilis{the following paragraph needs serious refactoring}
%That is proof of the fact that the network is the bottleneck of the system and not the CPU: the cache misses require network bandwidth, as thy are served remotely, but the cache hits that are served locally, consume CPU. The cache miss throughput does not increase as the cache miss rate increases which indicates that there is no room for improvement( the cache miss rate is 30\% with $\alpha = 1.01$ and 56\% with $\alpha = 0.9$), but the cache hit throughput increases as the cache hit rates increases, which shows that the CPU is underutilized.

%\arpit{Define: miss throughput and hit throughput.}
%\arpit{Explain why the ratio of miss and hit throughput will always remain same in the total throughput}

\tsubsection{Performance under writes}
\label{secC:write-perf}
We now analyze the performance of ccKVS in the presence of writes.
Figure~\ref{figC:writes} shows the throughput of the evaluated systems for varying write ratios with $\alpha = 0.99$. 
%None of the baselines are sensitive to the write ratio, as they are all bottlenecked by the network, which remains constant across all write ratios.
None of the baselines are sensitive to the write ratio, as they are all bottlenecked by the network. Note that in the baseline design, the network traffic does not change with varying write ratio as remote read and remote write requests both consume the same amount of network bandwidth.
%, and therefore their throughput remains almost constant. %Base-EREW has no concurrency overhead by default since the KVS is partitioned at a per-core granularity. Base is implemented without any concurrency control mechanism and therefore it is also not affected by changing write ratio. 
In contrast, the throughput for ccKVS decreases with increasing write ratio. This decrease is caused by the additional consistency actions for every cache write, such as broadcasting updates over the network. These actions consume network resources and thus diminish the throughput of the system, which is network-bound even in the read-only case (Section~\ref{secC:read-only}). 
%Furhtermore, ccKVS-Lin is more sensitive to write ratios than ccKVS-SC as it has to perform writes synchronously.

However, for realistic write ratios, such as $0.2\%$ for Facebook workload~\cite{Bronson:2013}, both ccKVS-SC and ccKVS-Lin provide throughput within $3\%$ of a read-only workload. In fact, ccKVS outperforms Base even for write ratios as high as $5\%$, while providing the strongest consistency guarantee (per-key linearizability). This is a particularly important result which shows that \emph{contrary to conventional wisdom, it is possible to achieve high throughput in the presence of aggressive replication under strong consistency guarantees.}

To further analyze the throughput of ccKVS with increasing write ratios, we show the breakdown of the network traffic for ccKVS-SC and ccKVS-Lin for $1\%$ and $5\%$ write ratios in Figure~\ref{figC:network-break-down}.  As the write ratio increases, consistency actions (i.e. updates, invalidates and acks) claim an increasingly larger percentage of the available network bandwidth. As a result, less bandwidth is available for remote KVS accesses triggered by cache misses. Since the system is network-bound, a reduction in available bandwidth for remote KVS accesses proportionately lowers total system throughput. 
%of remote KVS accesses. 
%However, that is not the only factor contributing to throughput degradation. The other factor is the performance degradation because of synchronous writes for ccKVS-Lin because of which its throughput degradation is much severe as compared to ccKVS-SC. 
Finally, we note that, thanks to batching of credits (Section~\ref{secC:design-perf}), flow control consumes a negligible amount of bandwidth.
%the consumption of scarce network bandwidth for flow control is negligible even for a $5\%$ write ratio.



\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/write_rate_performance_study.pdf} 
  \caption{Sensitivity to write ratio. [9 nodes, $\alpha$ = 0.99]}
  \label{figC:writes}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/network_traffic.pdf} 
  \caption{Network traffic breakdown. [9 nodes, $\alpha$ = 0.99] }
  \label{figC:network-break-down}
\end{figure}




\begin{comment}
-Throughput with Read Only \\
-Writes \\
--Throughout \\
--Load balanced(?) \\
--Break-down \\
-scalability \\
-Break-even \\

\tsubsection{Results}
\end{comment}




%\begin{figure}[h]
%  \centering
%  \includegraphics[width=0.5\textwidth]{Figures/read_only_value.pdf} 
%  \caption{Varying object size  (Read-only workload).}
%\end{figure}
%\vasilis{Added this section}
\tsubsection{Sensitivity to Object Size}
\label{secC:value-perf}
We next study the performance of ccKVS with varying object sizes.
%In order to better evaluate the behaviour of our protocols, we measure the performance of ccKVS for different object sizes with the default skew exponent (i.e. $\alpha = 0.99$). 
Figure ~\ref{figC:varying-value-size} shows the throughput of ccKVS in comparison to Base for various object sizes with 0\% and 1\% writes and $\alpha = 0.99$. 

In the read-only scenario (0\% writes), the relative performance of Base and ccKVS follows the same trend irrespective of the object size: ccKVS still outperforms Base by over 3$\times$ for bigger objects. 
%In the read-only scenario (0\% writes) bigger object sizes behave exactly as the small objects: ccKVS outperforms Base by over 3$\times$. 
With writes, however, increasing the object size lowers the performance difference between ccKVS-Lin and ccKVS-SC. This occurs because with large object sizes, the bulk of network bandwidth is consumed by the data payloads and only a small fraction of the bandwidth is spent on consistency messages (i.e. invalidations and acknowledgements) inherent in ccKVS-Lin. This result demonstrates that \emph{for workloads with large objects, it is possible to provide stronger consistency guarantees at very low performance overhead}.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/value_size_no_coalescing_read_only_and_1_perf_double_column.pdf} 
  \caption{Read-only and 1\% writes while varying object size. [9 nodes, $\alpha$ = 0.99]}
  \label{figC:varying-value-size}
\end{figure}



\tsubsection{System Bottlenecks} \label{secC:bottlenecks}
In order to identify the system bottlenecks,
we analyze the hardware counters for the NIC, PCIe and memory%
\footnote{We used the Mellanox's NEO-Host suite \cite{NeoHost} for NIC profiling and Intel's pcm \cite{pcm} for the PCIe and memory measurements.}%
. We also profile ccKVS (using the Zoom profiler~\cite{Zoom}) and use busy-wait counters within the ccKVS. After inspecting all measurements, we observe that  bottleneck shifts depending on the network packet size. We identify two distinct cases: big objects that result in big packet sizes, and small objects that result in small packet sizes. 

For big objects, network utilization in ccKVS closely approaches the available network bandwidth, while the rest of the resources remain underutilized; thus, we can safely infer that the bottleneck in this case is the available network bandwidth. 
On the other hand, with small objects, CPU, PCIe, memory bandwidth and network bandwidth are all underutilized. To our surprise, the bottleneck in the case of small object sizes appears to be the packet processing rate of the switch.
%\vijay{can we wauntitatively say that utilization is lower}\vasilis{is it any better? }

To validate our claim, we conduct the following experiment: we measure the maximum packet rate using Mellanox's micro-benchmark (ib\_send\_bw), when connecting two machines directly (i.e. without the switch) and when connecting them through the switch. We observe that the maximum rate of sent/received packets per second is significantly higher (by up to $25\%$), when the servers are connected directly.\footnote{Our findings were confirmed by the manufacturer of the switch.} The results hold in ccKVS as well.

% Finally, we confirmed our findings via a communication with the manufacturer of the switch.

For simplicity, throughout the paper we assume that the bottleneck is in the network in both cases, as the limited switch processing rate for small packets can be viewed as an artificial network bandwidth limitation. 
%\boris{I found the following a bit confusing. Not sure if my fix is correct though..}\vasilis{can we just drop it?}
We measure the maximum achievable bandwidth to be around 21.5 Gbps for small packets, while the NIC nominally supports 54 Gbps. 
%We observe that limitation to be at around 22Gbps, while the network provides 54Gbps. 

\begin{comment}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/net_utilization_coalescing_read_only_performance_overide_values.pdf} 
  \caption{Network utilization of a read-only workload with different object size. solid bars: data payload, stripes: packet headers. [9 nodes, $\alpha$ = 0.99]}
  \label{figC:coalescing-net}
\end{figure}
\end{comment}


\begin{comment}

%However, with small key-value pairs ccKVS is far from fully utilizing the available network bandwidth and thus it is clear that this is not the bottleneck, when the key-value pairs have a small size (i.e. 48B). 
%\antonis{I think it's not obvious or clear about the bottlenecks as we state. we need to rephrase}


 


%We conclude that for small packet sizes the network bottleneck can be defined more precisely as a network packet processing rate limitation. More specifically, we pinpoint the problem to the inability of the switch to process small packets (e.g. 64B) at line rate. %, which we validated by reproducing the same results using Mellanox's micro-benchmarks. 



%and 2) identical for the same type of connection(i.e. direct/indirect). Observing the PCIe H/W counters, we conclude that when directly connecting two machines, the bottleneck moves from the switch to the PCIe bandwidth. 


More analytically under direct connection the maximum transmit packet rate we observe is 63 million packets per second (the receive rate is identical). When removing the switch from the connection, the maximum transmit packet rate climbs to 73 million packets and is bottlenecked by the PCIe bandwidth. When slightly decreasing the packet size such that all payloads are at most 28 Bytes
\footnote{A payload with more than 28 Bytes will cause a non-linear increase in PCIe traffic as the WQE header is 36 Bytes and the payload is inlined within the WQE header. Therefore a 29 byte payload would mean that the WQE spills into a second cache-line causing the non-linearity in the PCIe-bandwidth consumption.}, then the PCIe bottleneck is alleviated and the maximum packet send rate further increases to 80 million packets per second. We note that decreasing the payload in the indirect connection has no effect.
\end{comment}
 


\tsubsection{Request Coalescing}
\label{secC:coalesc-perf}
In order to demonstrate and alleviate the bottlenecks imposed by transmitting small packets, we enable \textit{request coalescing}, whereby multiple requests destined to the same node are opportunistically coalesced into a single network packet.
We only apply request coalescing to cache misses (requests and the associated responses), since these dominate the network traffic in ccKVS at modest write ratios.
%With request coalescing, the network traffic is dominated by big packets, irrespective of the key-value size, and as a result, the packet processing bottleneck is alleviated and the network headers are amortized.


Figure \ref{figC:coalescing-net} shows the network utilization of ccKVS with and without request coalescing. In the figure, the network utilization is broken down into packet header and payload (i.e. data traffic), illustrated with striped and solid bars respectively.
Coalescing multiple requests results in larger network packets, shifting the bottleneck from the switch's packet processing rate to network bandwidth. As a result, the optimized ccKVS that supports coalescing  increases the throughput by almost 3$\times$ for the 40B values.

For a fair comparison, we also add support for coalescing to Base and we present the optimized performance of ccKVS and Base in Figure \ref{figC:coalescing-perf}, for read-only and 1\% writes, while varying the object size. As expected, comparing the results presented in Figures \ref{figC:varying-value-size} and \ref{figC:coalescing-perf}, both ccKVS and Base enjoy increased throughput for small object sizes when coalescing is applied. However, for larger objects coalescing is less beneficial as the system is already bottlenecked by the network bandwidth. %\hl{Overall, request coalescing is an optimization which can significantly increase the throughput of network bounded systems, whenever small requests are dominating the network traffic.}

In detail, examining the effect of coalescing for small (40B) objects, we observe that the performance of Base is almost 950 MRPS for both read-only and 1\% writes workloads, which yields an improvement of over 4$\times$ relative to the no-coalescing Base. In turn, ccKVS achieves a 3$\times$ improvement in performance with coalescing enabled, delivering over 2 billion requests per second, which is more than twice the performance of Base with coalescing. 

The benefits of coalescing diminish in ccKVS on the 1\% writes workload, because a fraction of network traffic carries consistency messages, which we do not coalesce. Nonetheless, even with writes, request coalescing improves the performance of the SC (Lin) variant of ccKVS by 2.6$\times$ (2$\times$) over no-coalescing.

\input{Text/1-ccKVS/Miscellaneous/Eval_triple_coalescing}
\FloatBarrier

%That can yield multiple times the performance of.

%In the default setting (i.e. without coalescing)of ccKVS bigger object values are much closer to the network bandwidth limit as opposed to 40B values.


%same  as \cite{Dragojevic:2017}, that for small messages sizes the network bottleneck can be defined more precisely as limited by the NIC packet processing rate, which we validated by reproducing the same results using Mellanox's micro-benchmarks. 


\begin{comment}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Text/1-ccKVS/Figures/value_size_coalescing_read_only_and_1_perf_double_column.pdf}
  \vspace{-2em}
  \caption{Performance impact of coalescing for read-only and 1\% writes while varying object size. [9 nodes, $\alpha$ = 0.99]}
  \vspace{-1em}
  \label{figC:coalescing-perf}
\end{figure}
\end{comment}
 



\tsubsection{Latency}
\label{secC:perf-vs-latency}
%\begin{comment}

Figure \ref{figC:latency-perf} illustrates the average and the 95-percentile latency of a read-only workload (ccKVS) and a workload with 1\% writes (ccKVS-SC and ccKVS-Lin) with varying load and with request coalescing enabled.
We observe that, even at high loads, tail latency is about an order of magnitude lower than the target of 1ms for a typical KVS service~\cite{Leverich:2014}. % \boris{Can you state the actual latency per the reference? its 1ms according to the reference}
In fact, at maximum load, the 95th percentile of both read-only and ccKVS-SC (1\% writes) is quite close to the average latency. %\sout{by serving requests in less than $\SI{50}{\micro}s$, while operating at maximum load.} 
However, when ccKVS-Lin is at high load, its 95-percentile is noticeably higher than its average latency, which is expected 
% Nonetheless, the actual latency is still much lower than the typical QoS target. , and in par with our expectations, 
since writes in ccKVS-Lin are blocking (i.e. sending invalidations and waiting for acknowledgments is in the critical path).

\begin{comment}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Text/1-ccKVS/Figures/latency_performance_50_95_no_base-lines.pdf} 
  %\caption{50, 95 and 99-percentile latency vs performance for read-only and 1\% writes.}
  \vspace{-2em}
  \caption{95-percentile and average latency for different loads of read-only and 1\% writes workloads with coalescing. [9 nodes, $\alpha$ = 0.99, value-size = 40B]}
  \vspace{-1em}
  \label{figC:latency-perf}
\end{figure}
\end{comment}
%\end{comment}

\tsubsection{Analytical model} \label{secC:analytical}
%(from now on \emph{cold-request throughput})

Since our 9-machine deployment prevents us from directly evaluating the scalability of ccKVS, 
%In order to overcome this challenge,
we build an analytical model that models the throughput of ccKVS.
The model leverages the fact that ccKVS is bottlenecked by the network bandwidth (Section~\ref{secC:bottlenecks}); therefore, the throughput of ccKVS is inversely proportional to the overall network traffic.

There are two sources of network traffic. The first source is due to requests that miss in the cache, whose keys are mapped to a remote node.  
%Remote cache misses and hot writes generate traffic.
A request is a cache miss with probability $(1-h)$, where $h$ denotes the hit ratio; the cache miss is mapped to a remote node with probability $1 - \frac{1}{N}$, where $N$ denotes the number of servers. 
A remote request generates two messages: one request and one reply; the total size of these two messages, in bytes, is denoted as $B_{RR}$.
%these two messages require $B_{RR}$ transferred bytes over the network. %A GET request need only carry the key, a GET reply need only carry the value, a PUT request need to carry both the key and the value and a PUT reply need not have any payload. Therefore, any request-reply pair consumes 2 network headers and a key-value pair, worth of bytes, denoted by M\_{CM}. %(Small message) and one reply (Big message); in total, this amounts to $M_{Big} + M_{Sm}$ bytes.
On average, the cache miss-related traffic ($TR_{CM}$) generated per request is given by:
\vspace{-0.1in}
   \begin{equation}
    \label{Ccache-miss-traffic}
    %T = \frac{T_m}{m} 
    TR_{CM} = (1-h) * (1 - \frac{1}{N}) * B_{RR}
    %T_m = T * m
    \end{equation}
    
The second source of traffic are the messages for consistency actions, generated by hot writes (i.e., those writes that hit in the cache). Consistency actions vary depending on the protocol. 
Consistency actions in Lin include invalidations, acknowledgements and updates; these three messages amount to $B_{Lin}$ bytes, with each hot writing generating $(N-1)$ of each of these.
%; in total, this amounts to $(N - 1) * B_{Lin}$ bytes. 
Additionally, the probability of a hot write is given by $h * w$, where $w$ denotes the write ratio. 
Therefore the overall consistency-related traffic ($TR_{Lin}$) generated per request in ccKVS-Lin, is given by:
\begin{equation}
    \label{CLin-traffic}
    TR_{Lin} = h * w * (N - 1) * B_{Lin}
    \end{equation}

From \ref{Ccache-miss-traffic} and \ref{CLin-traffic}, each request in ccKVS-Lin generates $TR_{CM} + TR_{Lin}$ bytes worth of traffic.
Because ccKVS is network-limited, the throughput (i.e. the number of requests per second) of a ccKVS-Lin server can be computed as the available network bandwidth ($BW$) divided by the bytes required per request.  Naturally, to compute the total throughput ($T_{Lin}$) of ccKVS-Lin, we need to multiply by the number of servers as shown in equation \ref{eqC:Lin_throughput}. 
\begin{equation}
T_{Lin} =  N * \frac{BW}{TR_{CM} + TR_{Lin}} 
\label{eqC:Lin_throughput}
\end{equation}

In contrast to Lin, a hot write in ccKVS-SC generates only $(N-1)$ updates, where each update requires $B_{SC}$ bytes to be transferred over the network. In total, the traffic of a hot write amounts to $(N - 1) * B_{SC}$ bytes in ccKVS-SC. Therefore, the overall consistency related traffic $(TR_{SC})$ generated by a request in ccKVS-SC, is given by:
\begin{equation}
    \label{CSC-traffic}
    TR_{SC} = h * w * (N - 1) * B_{SC}
    \end{equation}

From \ref{Ccache-miss-traffic} and \ref{CSC-traffic}, we can compute the total throughput ($T_{SC}$) of ccKVS-SC as shown in ~\ref{eqC:SC_throughput}.
\begin{equation}
T_{SC} = N * \frac{BW}{TR_{CM} + TR_{SC}} \label{eqC:SC_throughput}
\end{equation}

In the Uniform design, network traffic is generated for requests that map to a remote node. Requests map to a remote node with the probability $1 - \frac{1}{N}$ and such requests generate a request and a reply message, similar to cache misses in ccKVS, that amount to $B_{RR}$ bytes transferred over the network. Therefore, the total traffic $(TR_{U})$ generated by a request in Uniform is given by:
\begin{equation}
    \label{CUni-traffic}
    TR_{U} = (1 - \frac{1}{N}) * B_{RR}
    \end{equation}
And the total throughput ($T_U$) of Uniform is as shown in Equation~\ref{eqC:Uni_throughput}.
\begin{equation}
T_{U} =  N *\frac{BW}{TR_{U}} \label{eqC:Uni_throughput}
\end{equation}


\begin{comment}
%that can predict the performance of ccKVS for larger deployments. 
%To this end, we start with a basic observation.
%We start by making two basic observations:
%For a given cache hit rate ($h$), 
%\begin{itemize}
    
    
%Let us consider a ccKVS configuration without a cache (i.e. similar to the baseline). In such a configuration, every request is (by definition) a cache miss; a majority of such cache miss requests will have to be served by a remote node and will have to traverse the network. Let us denote the throughput of this configuration as cache miss throughput ($T_m$). 





%Each request in ccKVS goes though one of two paths:  the fast cache hit path  and the slow cache miss path.
    %The total throughput of ccKVS can be expressed as a function of  the sum of throughput due to cache hits and cache misses.
    
    
    %we can conclude that the throughput of the KVS is  
    %and that only cache misses consume network bandwidth. 
    %Hence, the throughput of requests missing in the cache will be the rate determining factor for the total throughput in the system.
    
%\end{itemize}


    
%\begin{itemize}


%\arpit{Should we have this in terms of cache hit rate as that is what we use in subsequent equations.}

% \begin{equation}
%     T_m = T*m 
%     \end{equation}
   
    \begin{equation}
    \label{eqC:cold-throguhput}
    %T = \frac{T_m}{m} 
    T = \frac{T_m}{(1-h)} 
    %T_m = T * m
    \end{equation}
    



    \item  Under a read-only workload, ccKVS utilizes all the available network bandwidth only to serve cache misses. However, in the presence of writes, the consistency traffic generated because of write hits also consumes a fraction of the network bandwidth. This reduces the available network bandwidth to complete cache misses and thus decreases the cache-miss throughput. As a result, it proportionally lowers the total system throughput.
%\end{itemize}


    
    

The network traffic generated because of cache misses and writes that hit in the cache can be computed for both SC and Lin protocols as shown in Table~\ref{tabC:analytical-parameters}. 
%Moreover, a constant cache hit rate implies that the network bandwidth requirements for servicing cache misses do not change. 
Given the total bandwidth of the system, we can calculate the reduction in total system throughput by computing the reduction in the available network bandwidth for servicing cache misses because of the bandwidth consumed for servicing write hits.
%Fortunately, this decrease can be analytically computed for any given write ratio, because the \sout{worst-case} network traffic generated by each write to a hot item is deterministic for both SC and Lin protocols. Therefore, by computing the portion of the network bandwidth that is allocated to the consistency traffic \sout{for a given write ratio}, we are able to compute the reduction on the total system throughput.%the cache-miss throughput of ccKVS, and thus the overall throughput reduction in comparison to the read-only ccKVS throughput.
%Towards that goal, we build a simple analytical model that computes the slow-down of both ccKVS-SC and ccKVS-Lin, when introducing writes.  
%In order to derive this slow-down, the analytical model compares the transferred bytes per request, with and without writes, assuming that in both cases ccKVS is network-bound. 
%We expect the analytical model to be accurate, as long as ccKVS is network-bound.
Equations \ref{eqC:SC_throughput}, \ref{eqC:Lin_throughput} describe the model to compute the slow-downs $S_{SC}$ and $S_{Lin}$ of ccKVS-SC and ccKVS-Lin, respectively. 

\end{comment}


 \begin{comment}
 
 
 $M_{RO} = (1-h) * \frac{M_{Sm} + M_{Big}}{2} * (1 - \frac{1}{N})$
 

 $coherence_{SC} = h * W * (N - 1) * M_{Big}$
 
 $coherence_{Lin} = h * W * (N - 1) * (M_{Big} +2M_{Sm})$
 

\begin{equation}
\label{eqC:SC_throughput}
 S_{SC} = \frac{M_{CM}} {M_{CM} + M_{SC}}
\end{equation}



\vasilis{we need labels in the equations, either we split them in two lines or we do some hack (probably minipages)}
\begin{equation}
\label{eqC:analytical_model}
 S_{SC} = \frac{M_{CM}} {M_{CM} + M_{SC}},
 \quad %
 S_{Lin} = \frac{M_{CM}} {M_{CM} + M_{Lin}} 
%\end{equation}
\end{equation}


\begin{centering}
\begin{minipage}[c]{.24\textwidth}
%\vspace{-\baselineskip}
\begin{equation}
S_{SC} = \frac{B_{CM}} {B_{CM} + B_{SC}} \label{eqC:SC_throughput}
\end{equation}
\end{minipage} %\hfill
%\hfill\hfill and\hfill
\begin{minipage}[c]{.24\textwidth}
%\vspace{-\baselineskip}
\begin{equation}
S_{Lin} = \frac{B_{CM}} {B_{CM} + B_{Lin}} \label{eqC:Lin_throughput}
\end{equation}
\end{minipage}
\end{centering}
\end{comment}


\begin{comment}
\begin{centering}
\begin{minipage}[c]{.24\textwidth}
%\vspace{-\baselineskip}
\begin{equation}
T_{SC} =  \frac{N *BW}{B_{CM} + B_{SC}} \label{eqC:SC_throughput}
\end{equation}
\end{minipage} %\hfill
%\hfill\hfill and\hfill
\begin{minipage}[c]{.24\textwidth}
%\vspace{-\baselineskip}
\begin{equation}
T_{Lin} =  \frac{N *BW}{B_{CM} + B_{Lin}} \label{eqC:Lin_throughput}
\end{equation}
\end{minipage}
\end{centering}
\end{comment}


\begin{comment}

\begin{equation}
\label{eqC:SC_throughput}
\resizebox{0.80\hsize}{!}{%
 $S_{SC} = \frac{Avg(1 - \frac{1}{N})} {(1-Ch)Avg(1 - \frac{1}{N}) + ChWr(N - 1)Big}$
 }
\end{equation}

%\noindent ccKVS-Lin throughput T: 
\begin{equation}
\label{eqC:LIN_throughput}
 \resizebox{0.90\hsize}{!}{%
 $S_{Lin} = \frac{Avg(1 - \frac{1}{N})} {(1-Ch)Avg(1 - \frac{1}{N}) + ChWr(N - 1)(Big + 2Sm)}$
 }
\end{equation}
\end{comment}

\begin{comment}

Fortunately, this effect can be analytically computed for any given write ratio, because the worst-case network traffic generated by each write to a hot item is deterministic in both SC and Lin. Therefore, by computing what part of the network resources are allocated to the consistency traffic, we can compute the reduction on the cold-request throughput of ccKVS and thus the reduction in ccKVS throughput.

Towards that goal, we build a simple analytical model that computes the throughput of both ccKVS-SC and ccKVS-Lin given: the number of servers ($N$), the write ratio ($Wr$), the cache hit ratio($Ch$) the throughput of Uniform($T_U$) and the size($Big, Sm$) of all messages(in Bytes). We expect the analytical model to be accurate as long as the system is bottlenecked by the network. 

Equations \ref{eqC:SC_throughput}, \ref{eqC:LIN_throughput} describe the models to compute the throughput $T_{SC}$ and $T_{LIN}$ of ccKVS-SC and ccKVS-Lin, respectively. All the parameters are described in table~\ref{tabC:analytical-parameters}. These two equations comprise the analytical model, which we use to predict the ccKVS performance for deployments with more than 9 machines. In essence the model predicts the speed-up of ccKVS over Uniform; intuitively under both consistency models, the speed-up over Uniform(i.e. $T_{U}$) decreases as the write ratio increases(i.e. $Wr$). 



\begin{equation}
\label{eqC:SC_throughput}
\resizebox{0.80\hsize}{!}{%
 $T_{SC} = T_U\frac{Avg(1 - \frac{1}{N})} {(1-Ch)Avg(1 - \frac{1}{N}) + ChWr(N - 1)Big}$
 }
\end{equation}

%\noindent ccKVS-Lin throughput T: 
\begin{equation}
\label{eqC:LIN_throughput}
 \resizebox{0.90\hsize}{!}{%
 $T_{LIN} = T_U\frac{Avg(1 - \frac{1}{N})} {(1-Ch)Avg(1 - \frac{1}{N}) + ChWr(N - 1)(Big + 2Sm)}$
 }
\end{equation}





\begin{equation}
\label{eqC:SC_throughput}
 T_{SC} = T_U\frac{\frac{Big + Sm}{2}(1 - \frac{1}{N})} {(1-Ch)\frac{Big + Sm}{2}(1 - \frac{1}{N}) + ChWr(N - 1)Big}
\end{equation}

%\noindent ccKVS-Lin throughput T: 
\begin{equation}
\label{eqC:LIN_throughput}
 T_{LIN} = T_U\frac{\frac{Big + Sm}{2}(1 - \frac{1}{N})} {(1-Ch)\frac{Big + Sm}{2}(1 - \frac{1}{N}) + ChWr(N - 1)(Big + 2Sm)}
\end{equation}

\end{comment}

\begin{comment}

\begin{table} 
\begin{center}
\begin{tabular}{ |c|c|c|}  \hline
\multirow{1}{2em}{\textit{$N$}} & Number of servers \\  \hline
\multirow{1}{2em}{\textit{$w$}}  & Write ratio \\  \hline
\multirow{1}{2em}{\textit{$h$}}  & Cache hit ratio \\ \hline
\multirow{1}{2em}{\textit{$BW$}}  & Available Network Bandwidth \\ \hline
%\multirow{1}{2em}{\textit{$T_{U}$}}  & Throughput of Uniform \\ \hline %\\  & (cold-request throughput of read-only ccKVS) 
\multirow{2}{2em}{\textit{$M_{Big}$}} & Big message in Bytes  \\ & (read reply, write request, update) \\  \hline
\multirow{2}{2em}{\textit{$M_{Sm}$}}  & Small message in Bytes  \\  & (read request, write reply, inv, ack) \\ \hline \hline
\multirow{2}{2em}{\textit{$B_{CM}$}}  & $(1-h) * (1 - \frac{1}{N}) * (M_{Sm} + M_{Big})$ \\ & (Bytes sent per request for cache misses) \\ \hline

%\multirow{1}{6em}{$remotes_{ccKVS}$}  & $(1 - h) * remotes_{Base}$ \\ \hline

\multirow{1}{2em}{\textit{$B_{SC}$}}  & $h * w * (N - 1) * M_{Big}$ \\ &  (Bytes sent per request for coherence in SC) \\ \hline

\multirow{1}{2em}{\textit{$B_{Lin}$}} & $h * w * (N - 1) * (M_{Big} +2M_{Sm})$ \\ &  (Bytes sent per request for coherence in Lin)\\ \hline


%\multirow{1}{2em}{\textit{Avg}}  & Average of Big and Sm \\  \hline

%$remotes_{Base} = \frac{Sm + Big}{2} * (1 - \frac{1}{N})$
%\multirow{2}{2em}{\textit{Cub}}  & Credit Update Batch \\  & (credits in a credit update message)\\  \hline
%\multirow{1}{2em}{\textit{Avg}}  & Average of Sm and Big \\  \hline
%\multirow{1}{2em}{\textit{Ho}}  & Header only in Bytes \\ \hline
% \multirow{1}{2em}{$M_{RO}$}  & $(1-h) * \frac{M_{Sm} + M_{Big}}{2} * (1 - \frac{1}{N})$ \\ \hline

% %\multirow{1}{6em}{$remotes_{ccKVS}$}  & $(1 - h) * remotes_{Base}$ \\ \hline

% \multirow{1}{2em}{$M_{SC}$}  & $h * W * (N - 1) * M_{Big}$ \\ \hline

% \multirow{1}{2em}{$M_{Lin}$}  & $h * W * (N - 1) * (M_{Big} +2M_{Sm})$ \\ \hline
 
\end{tabular}
\vspace{-0.5em}
\caption{Parameters used in the analytical model} \label{tabC:analytical-parameters}
\vspace{-1.5em}
\end{center}
\end{table}
\end{comment}


\begin{comment}


%%% NEW TABLE JUST FOR BYTES %%%
\begin{table} 
\begin{center}
\begin{tabular}{ |c|c|c|}  \hline
%\multirow{1}{2em}{\textit{$N$}} & Number of servers \\  \hline
%\multirow{1}{2em}{\textit{$w$}}  & Write ratio \\  \hline
\multirow{1}{2em}{\textit{$h$}}  & $65\%$ Cache hit ratio \\ \hline
\multirow{1}{2em}{\textit{$BW$}}  & $21.5Gbps$ Network Bandwidth \\ \hline
%\multirow{1}{2em}{\textit{$T_{U}$}}  & Throughput of Uniform \\ \hline %\\  & (cold-request throughput of read-only ccKVS) 

\multirow{2}{2em}{\textit{$B_{RR}$}}  & $113 Bytes$ \\ & (Bytes sent per remote request) \\ \hline

%\multirow{1}{6em}{$remotes_{ccKVS}$}  & $(1 - h) * remotes_{Base}$ \\ \hline

\multirow{1}{2em}{\textit{$B_{SC}$}}  & $83 Bytes$ \\ &  (Bytes sent per request for coherence in SC) \\ \hline

\multirow{1}{2em}{\textit{$B_{Lin}$}} & $183 Bytes$ \\ &  (Bytes sent per request for coherence in Lin)\\ \hline

%\multirow{2}{2em}{\textit{$B_{U}$}} & $113 Bytes$  \\ & (Bytes sent per request for cache misses) \\  \hline
%\multirow{2}{2em}{\textit{$B_{Sm}$}}  & Small message in Bytes  \\  & (read request, write reply, inv, ack) \\ \hline \hline
%\multirow{1}{2em}{\textit{Avg}}  & Average of Big and Sm \\  \hline

%$remotes_{Base} = \frac{Sm + Big}{2} * (1 - \frac{1}{N})$
%\multirow{2}{2em}{\textit{Cub}}  & Credit Update Batch \\  & (credits in a credit update message)\\  \hline
%\multirow{1}{2em}{\textit{Avg}}  & Average of Sm and Big \\  \hline
%\multirow{1}{2em}{\textit{Ho}}  & Header only in Bytes \\ \hline
% \multirow{1}{2em}{$M_{RO}$}  & $(1-h) * \frac{M_{Sm} + M_{Big}}{2} * (1 - \frac{1}{N})$ \\ \hline

% %\multirow{1}{6em}{$remotes_{ccKVS}$}  & $(1 - h) * remotes_{Base}$ \\ \hline

% \multirow{1}{2em}{$M_{SC}$}  & $h * W * (N - 1) * M_{Big}$ \\ \hline

% \multirow{1}{2em}{$M_{Lin}$}  & $h * W * (N - 1) * (M_{Big} +2M_{Sm})$ \\ \hline
 
\end{tabular}
%\vspace{-0.5em}
\caption{Parameters used in the analytical model} \label{tabC:analytical-parameters}
\vspace{-1.5em}
\end{center}
\end{table}
\end{comment}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/performance_study_multiple_servers.pdf} 
  \caption{ccKVS scalability study using the model (dashed) and real-system validation (solid). [1\% writes, $\alpha$ = 0.99]}
  \label{figC:analytical-server}
\end{figure}

\tsubsubsection{\textbf{Scalability study}}
In the presence of writes, we anticipate the per-server throughput of ccKVS to degrade as the number of servers increase, due to the proportional increase in consistency traffic. 
We employ the proposed analytical model to conduct a scalability study and understand the extent of this degradation.
%In order to calculate the extent of this degradation, we employ our analytical model to conduct a scalability study. 
%We observe that the throughput of Uniform is equal to the cache-miss throughput of ccKVS under a read-only workload. 

%In order to make an estimation that can be validated with our existing setup, we feed the model with the same parameters as the ones observed in our measurements. 
To validate the model with our existing setup, we feed the model with the same parameters as in our implementation with request coalescing disabled. We set the cache hit ratio ($h$) to $65\%$ and we set the message sizes with the exact numbers used in our evaluation for small objects (Sections~\ref{secC:read-only},~\ref{secC:write-perf}): $B_{RR} = 113 $ bytes, $B_{SC} = 83$ bytes and $B_{Lin} = 183$ bytes (including network headers). Finally, we set the available network bandwidth ($BW$) at $21.5$ Gbps, which is the network bandwidth observed for the configuration with small objects (Figure~\ref{figC:coalescing-net}). 
%\arpit{I think we should just put in the numbers for B* parameters.}

%, and thus we also compute the throughput of Uniform to be used as a baseline. 
%Recall that Uniform represents an upper bound on the performance of baseline.
%as it assumes a uniform workload.
  %by estimating the throughput of Uniform and using it to compute the throughput of ccKVS.
Figure \ref{figC:analytical-server} shows the estimated throughput of Uniform, ccKVS-SC and ccKVS-Lin, when scaling the number of servers of the deployment from 5 to 40, while fixing the write ratio at $1\%$. 
%In an effort to validate the analytical model, 
As expected, the scaling of Uniform is almost perfectly linear. However, ccKVS-SC and ccKVS-Lin scale sublinearly with the number of servers; this is  because, as the number of servers increases, the consistency traffic increases too. ccKVS-Lin scales more poorly than ccKVS-SC, because ccKVS-Lin requires more consistency messages due to the two-phase nature of its protocol.

We also plot the measured throughput of our system for up to 9 machines (i.e. the size of our deployment). As we can see, the analytically computed throughput is similar to the measured throughput for both ccKVS and Uniform. %Slight discrepancies can be attributed to the fact that the network bottleneck imposed by the switch, varies with the number of servers in the deployment.
%We attribute this small discrepancy to the fact that the Uniform performance fed as an input into the model, is also slightly higher than the measured Uniform throughput.
%Let us examine ccKVS-SC more closely; 
With 9 servers, ccKVS-SC  and ccKVS-Lin are estimated to achieve $628$ MRPS and $554$ MRPS, respectively, which is within $2\%$ of the measured throughput in our implementation ($639$ MRPS for ccKVS-SC and $554$ MRPS for ccKVS-Lin).
%When doubling the number of servers to 18, the throughput improvement is $1.7\times$ (i.e. $1079$ MRPS). Further doubling the servers to 36 server yields a $1.6\times$ throughput improvement (i.e. $1786$ MRPS). 
%In general, with every added server, the consistency overhead increases and the scalability drops.
%In general it scales sublinearly because the consistency overhead increases with every additional server.

%When focusing on ccKVS-Lin, we observe the same phenomenon, but now each added server incurs a bigger penalty in scalability. That is expected as each write in ccKVS-Lin requires more consistency messages due to the two-phase nature of the protocol.

In general, we find that the analytical model predicts the performance of ccKVS designs with sufficient accuracy. Using the validated model, we find that the performance of both ccKVS-SC and ccKVS-Lin is significantly better than the upper bound for the baseline (i.e. Uniform) for moderately sized deployments with a $1\%$ write ratio.

 
%Based on the same analytical model we investigate the scalability of the ccKVS under a zipfian distribution ($\alpha = 0.99$) with 1\% write ratio.  The analytical model is in par with the results from our 9-machine deployment. Essentially, the network overhead of keeping the popularity caches coherent increases linearly with the number of servers. As the coherence traffic increases the servers have less network bandwidth available to serve the cache misses, thereby limiting the throughput of the entire system.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.5\textwidth]{Figures/read_only_scaling.pdf} 
%   \caption{Scaling machines (Read-only workload)\antonis{We should probably add writes(1\% EC \& SC)}.}
% \end{figure}


%\input{Sections/break-even-write-ratio}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/break_even_performance_study-32.pdf}
  \caption{Break-even write ratio model (dashed) and real-system validation (solid) for up to 9 nodes. [$\alpha$ = 0.99]}
  \label{figC:break-even}
\end{figure}

\tsubsubsection{\textbf{When does Symmetric Caching break even?}}  

%When applying Symmetric Caching, each write to a hot item generates consistency traffic. inside the black box. 
%Therefore, an increase in the write ratio results in an increase in consistency traffic, which leads to a decrease in the rate at which cache misses are handled. As discussed, the performance of ccKVS is determined by the rate at which it can serve the cache misses and therefore, a decrease in that rate can be directly correlated to the maximum performance that the system can achieve. 

%In order to provide some intuition about the settings for which Symmetric Caching can be beneficial
Next, we use our analytical model to answer the following question: for a deployment of X servers, what is the write ratio at which ccKVS yields the same throughput as Uniform.
We call this write ratio the \textit{break-even write ratio}. 
%
In order to calculate the break-even write ratio for ccKVS-SC, we equate the throughput of Uniform, $T_U$ (Equation~\ref{eqC:SC_throughput}), with the throughput of ccKVS-SC, $T_{SC}$ (Equation~\ref{eqC:Uni_throughput}), and solve for the write ratio. We follow the same procedure to calculate the break-even write ratio for ccKVS-Lin.
%Similarly to the scalability study, we set the size of Small and Big packets equal to 51 and 84 Bytes, respectively. We note that the cache hit ratio is factored out of the equations, leading to an important result: the computed break-even write ratios will hold true for any skew exponent or cache size.


\begin{comment}
\begin{equation}
\label{eqC:SC_break_even}
 Break\_even\_W_{SC} = \frac{\frac{M_{Sm} + M_{Big}}{2} * (1 - \frac{1}{N})} {(N - 1) * M_{Big}}
\end{equation}
%\vasilis{TODO: Antonis will double check these, if we end up using them}

\begin{equation}
\label{eqC:LIN_break_even}
 Break\_even\_W_{LIN} = \frac{\frac{M_{Sm} + M_{Big}}{2} * (1 - \frac{1}{N})}{(N - 1) * (M_{Big} + 2M_{Sm})}
\end{equation}


\begin{equation}
\label{eqC:SC_break_even}
 W_{SC} = \frac{Avg(1 - \frac{1}{N})} {(N - 1)Big}
\end{equation}
%\vasilis{TODO: Antonis will double check these, if we end up using them}

\begin{equation}
\label{eqC:LIN_break_even}
 W_{LIN} = \frac{Avg(1 - \frac{1}{N})}{(N - 1)(Big + 2Sm)}
\end{equation}
\end{comment}

Figure~\ref{figC:break-even} illustrates the break-even write ratio for ccKVS-SC and ccKVS-Lin deployments of up to 40 servers. For example, a ccKVS-SC deployment with 20 servers will yield the same performance as Uniform at a write ratio of $8\%$. Therefore, a 20-server deployment with write ratio below $8\%$ can benefit from employing ccKVS-SC. 

%\boris{Improved wording in the next 2 paragraphs. Please check. }
To validate the model, Figure~\ref{figC:break-even} also depicts the measured break-even write ratios for actual deployments of up to 9 machines. We observe that the trend is similar for both the model and actual measurements; however, the real system can sustain slightly higher break-even write ratios than what the model predicts. 
The reason behind this slight discrepancy is that, as noted in Section~\ref{secC:bottlenecks}, the actual bottleneck for small packets is in the switch packet processing %(and not the network bandwidth per se), 
and, because the update messages in Lin and SC are big (contain both key and value) the system achieves higher network bandwidth than predicted for  high write ratios. 

%the model makes a pessimistic, worst-case assumption for the amount of required consistency traffic for each write. In practice, the model and the real system differ when writes to the same key clash, in which case only the winning write (identified via a Lamport timestamp) generates the full consistency traffic. \arpit{Is this also true for SC? Seems not. Then let's just say something vague that holds for both SC and Lin.}\vasilis{can we omit giving a reason, and just say that the trends are similar. (the model is more pessimistic for higher write ratios, but we dont know why)}
%\arpit{I can't think of vague way of saying this. May be we can just leave this explanation for now and try to improve before camera ready.}

As expected, the break-even write ratios for ccKVS-Lin are consistently lower than those for ccKVS-SC. %, \sout{seeing as a write in ccKVS-Lin translates into more consistency messages, because Lin requires a two-phase protocol that contains a round of invalidations and acknowledgements before the update}.
Furthermore, as the number of servers increases, the break-even write ratio decreases in both consistency models. The decrease happens because the consistency traffic increases linearly with the number of servers, since a write to a hot object must be propagated to all servers. With 40 servers, the break-even write ratio is almost $4\%$ for ccKVS-SC and $1.7\%$ for ccKVS-Lin. This indicates that in a moderately sized deployment with low write ratios, ccKVS should outperform the baseline while maintaining strong consistency guarantees; however, at higher write ratios or in larger deployments, the performance benefit of ccKVS may vanish.%\vasilis{it may be good to add that this study is independent of the skew}


\begin{comment}

As discussed in Section~\ref{secC:write-perf}, the throughput of ccKVS is proportional to the proportion of data traffic in the network. 
Using this correlation, we build an analytical model that computes the throughput as the proportion of data traffic to the
%decrease in the rate at which cache misses can be serviced, 
consistency traffic changes, for both ccKVS-SC and ccKVS-Lin. 
Our primary goal is to answer this question: for a deployment of X servers what is the write ratio at which the ccKVS yields the same throughput as Uniform.
We call this write ratio the \textit{break-even write ratio}. Figure~\ref{figC:break-even} illustrates the break-even write ratio for a ccKVS-SC and ccKVS-Lin deployment of up to 40 servers. For example, a ccKVS-SC deployment with 20 servers will yield the same performance as Uniform at a write ratio of $8\%$. As expected the break-even write ratios of ccKVS-Lin are consistently lower than ccKVS-SC. The reason behind this is that a write in ccKVS-Lin translates into more consistency messages, because per-key Linearizability requires a two-phase protocol that contains a round of invalidations and acknowledgements before the update.

Additionally we note that, as the number of servers increases the break-even write ratio decreases in both consistency models. The reason this happens is because the consistency traffic increases linearly with the number of servers, since a write to a hot object must be propagated to all servers. With 40 servers the break-even write ratio is almost $4\%$ for ccKVS-SC and $1.7\%$ for ccKVS-Lin. This indicates that in a moderately sized deployment ccKVS outperforms the baseline for moderate write ratios, while maintaining strong consistency guarantees.\vasilis{it may be good to add that this study is independent of the skew}

\end{comment}

%We note that the break-even write ratio per-key SC decreases as the value size increases, because the consistency consists of solely big messages(i.e. broadcasts). In contrast the break-even write ratio increases with per-key Linearizability when the value size increases, because in that case 2/3 of the consistency traffic is small messages (i.e. acknowledgements and invalidations).
\begin{comment}


\\
The parameters are: \\
\textit{N}: Number of Servers\\
\textit{wr}: Write Ratio\\
%f : cache hit ratio\\
Payloads:\\
\textit{Big}: Big message in Bytes (i.e. read reply, or write request)\\
\textit{Sm}: Small message in Bytes (i.e. read request, or write reply)\\
\textit{Avg}: Average of small and big messages in Bytes\\
\textit{HO}: Header only in Bytes (i.e. the credit message has no payload)\\
\textit{CD}: Credit Divider (i.e. how many credits in a credit update message)\\ 
\\



\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|}  \hline
\multirow{1}{2em}{\textit{N}} & Number of Servers \\  \hline
\multirow{1}{2em}{\textit{Wr}}  & Write Ratio \\  \hline
\multirow{2}{2em}{\textit{Big}} & Big packet in Bytes \\ & (read reply, or write request) \\  \hline
\multirow{2}{2em}{\textit{Sm}}  & Small packet in Bytes \\  & (read request, or write reply)\\ \hline
\multirow{2}{2em}{\textit{Cub}}  & Credit Update Batch \\  & (credits in a credit update message)\\  \hline
\multirow{1}{2em}{\textit{Avg}}  & Average of Sm and Big \\  \hline
\multirow{1}{2em}{\textit{Ho}}  & Header only in Bytes \\ \hline
\end{tabular}
\caption{Parameters of the break-even write-ratio }
\end{center}
\end{table}
\end{comment}

\begin{comment}
\begin{equation}
\label{eqC:SC_break_even}
 Wr_{SC} = \frac{Avg(1 - \frac{1}{N})} {(N - 1)Big}
\end{equation}
\vasilis{TODO: Antonis will double check these, if we end up using them}

\begin{equation}
\label{eqC:LIN_break_even}
 Wr_{LIN} = \frac{Avg(1 - \frac{1}{N})}{(N - 1)(Big + 2Sm)}
\end{equation}


It is worth noting that the cache hit ratio is factored out of this equation. In other words the break-even write ratio is solely a function of the number of servers and the payloads and it is completely independent of the cache hit ratio. 


It is worth highlighting that the break-even write ratio refers to the point where Symmetric Caching breaks even with a baseline with uniform distribution. Therefore, even when the write ratio is at its break-even point, Symmetric Caching will yield better performance than no caching. 

%DEFEND THE SIZE OF THE BLACK BOX
Figure \ref{figC:break-even} shows the break-even write ratio of a black box with Symmetric caching varying the size of the black box from 5 up to 40 servers. There is no hard constraint on the size of the black box, rather each application can choose a different size according to its write ratio \antonis{and skew(?)} . For example, a KVS that fits in 80 servers can be split into 8 10-server black boxes or 4 20-server black boxes, depending on the write ratio. However, the popularity cache only stores data items that belong to the black box and thus, breaking up the KVS into multiple black boxes will have an effect on the hit ratio of the popularity caches. For a complete study on how the skew varies when decreasing the size of the black box we refer the reader to \cite{RNovakovic:2016}.
\end{comment}


==> Text/5-ccKVS-SC/9-Discussion.tex <==

\tsection{Discussion}
\label{secC:discuss}

\noindent{\bf Scalability.} We have established that the benefits of symmetric caching decrease with increasing size of the deployment. 
However, this constraint does not strictly prohibit the application of symmetric caching in large deployments.
To scale beyond a rack-scale or small cluster sized deployment, we believe our ideas can be applied by simply partitioning bigger deployments into smaller Scale-Out ccNUMA clusters, each of which can independently apply symmetric caching.  %\boris{it's really not clear how to do that. Either we provide detail (could be as little as citing prior work that does this) or we drop this point.}
%\vasilis{what about the following?}
%\boris{changed 9 groups to 5 groups, because we have 9 servers in our deployment, so it gets a bit confusing with 9's.}
For example, a KVS that spans 100 nodes can be split into five 20-machine groups (similar to~\cite{RNovakovic:2016}), where each group employs symmetric caching for its portion of the KVS. 
%\boris{I don't understand the following part, but perhaps we don't need it. Can we stop at the last sentence?}

%\subsection{}
\noindent{\bf Resilience.} 
%In building ccKVS, we do not implement logic to detect and recover from failures. 
We do not handle failures in the ccKVS design.
%However, Scale-Out ccNUMA is not constrained by the choice of KVS, so existing resilience mechanisms, such as the one proposed in FaRM~\cite{Dragojevic:2015}, can be readily applied. 
However, existing resilience mechanisms, such as the one proposed in FaRM~\cite{Dragojevic:2015}, can be readily applied to ccKVS, and, more generally, to Scale-Out ccNUMA. 
Most generally, we note that the principle objective of this work is to demonstrate that caching with aggressive replication presents a performance opportunity even with strong consistency models. Nonetheless, there is interesting interplay between replication, resilience and the strength of the consistency model, which we leave for future work to explore. 
\todo{rework / remove}
\begin{comment}

\begin{itemize}
%\item Epochs and Identify hot items through streaming algorithm
\item Enabler of our design: RDMA vs Protocols
\item Scalability: 
\end{itemize}

\tsubsection{ccKVS versus single cache node} \label{secC:eval-cache}
The caching technique is fundamentally limited by the network bandwidth of the node that acts as the cache. Let's understand this through an example: if the caching node has enough network bandwidth to deliver X throughput and it has to serve 50\% of the accesses, then the throughput of the entire system is capped at 2X, irrespective of how many nodes there are in the deployment. Similarly to Base, the throughput of the system is limited by the throughput of its hottest server. 
In a skewed distribution with $\alpha=0.99$, the hottest item receives approximately 5\% of the total accesses. Therefore, even in the edge case where  the caching server only caches a single item, then the system throughput will never be more than 20 times the throughput of the cache server. This is the key motivation behind replicating the caches, the hottest items must be served by multiple nodes to avoid hot servers that limit the the system's throughput.
\end{comment}

==> Text/5-ccKVS-SC/Miscellaneous/Eval_triple_coalescing.tex <==
\begin{figure*}[!ht]
  \centering
  \begin{subfigure}[b]{0.7\textwidth}
    \includegraphics[width=\textwidth]{Text/1-ccKVS/Figures/net_utilization_coalescing_read_only_performance_overide_values.pdf}
    \captionsetup{width=0.85\linewidth}
    \caption{Network utilization of a read-only workload with different object size. Solid bars: data payload, stripes: packet headers.}
    \label{figC:coalescing-net}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.7\textwidth}
    \includegraphics[width=\textwidth]{Text/1-ccKVS/Figures/value_size_coalescing_read_only_and_1_perf_double_column-mini.pdf}
    \captionsetup{width=0.85\linewidth}
    \caption{Performance impact of coalescing for read-only and 1\% writes while varying object size. \\}
    \label{figC:coalescing-perf}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.7\textwidth}
    \includegraphics[width=\textwidth]{Text/1-ccKVS/Figures/latency_performance_50_95_no_base-lines-mini.pdf}
    \captionsetup{width=0.85\linewidth}
    \caption{95th percentile and average latency for 40B objects at various load levels for read-only (ccKVS) and 1\% writes (ccKVS-SC/Lin) with coalescing.}
    \label{figC:latency-perf}
  \end{subfigure}
  \caption{Analysis of coalescing and latency. [9 nodes, $\alpha$ = 0.99]}
\end{figure*}

==> Text/5-ccKVS-SC/Miscellaneous/Fig_consistency_actions.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\textwidth]{Text/1-ccKVS/Figures/cckvs-protocols.pdf}
  \caption{Required write actions for each consistency model.} 
  \label{figC:consistency-actions}
\end{figure}

==> Text/5-ccKVS-SC/Miscellaneous/Fig_consistency_example_1.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/Lin-violation.pdf}
  \caption{Session B seeing the old value is a violation of Lin, but not SC.}
  \label{figC:consistency-example-1}
\end{figure}


==> Text/5-ccKVS-SC/Miscellaneous/Fig_consistency_example_2.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/SC-violation.pdf}
  \caption{Sessions B and C do not agree on the order of writes and hence this is a SC violation (also a Lin violation).} 
  \label{figC:consistency-example-2}
\end{figure}


==> Text/5-ccKVS-SC/Miscellaneous/Fig_protocols.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/cckvs-global-order.pdf}
  \caption{Design space for guaranteeing a single global order for writes on a per-key basis. }
  \label{figC:protocols-design}
\end{figure}


==> Text/5-ccKVS-SC/Miscellaneous/Fig_related_work.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\textwidth]{Text/1-ccKVS/Figures/ccKVS-design-space.pdf}
  \caption{Design space for skew mitigation techniques.}
  \label{figC:blackbox}
\end{figure}


==> Text/5-ccKVS-SC/Opportunity.tex <==
\subsection{Opportunity Analysis}
\label{secC:opportunity}

\boris{Should this be here or in Motivation?}
\vasilis{It was very challenging to analyze the opportunity, if we do not explain how symmetric caching works, i.e. black box, caches,life of a request}


To analyze the opportunity of Symmetric Caching, we investigate what is the maximum theoretical speed-up that can be achieved with this technique. Firstly we assume a black box architecture similar to RackOut, where the maximum throughput can be achieved under a uniform distribution.
%: the clients request data item from any server of the KVS independently of whether that server is the home owner of the requested data items.
%If a server is not the owner of the requested data, it in turn issues a request to the server which owns the data over RDMA network. Therefore each server in the KVS both issues and responds to requests. 
In this setup we will compare the performance of a baseline black box system when the access pattern is uniform and the same system with Symmetric Caching when the access pattern is Zipfian. 
\arpit{Should we briefly explain somewhere why is uniform distribution (the baseline) the best case scenario for the current state of the art.}\vasilis{The background section on RackOut explains this now}

In the baseline system caching would have no effect, since all data items are equally popular; the system is totally load-balanced and thus each server can service a fixed number of requests every second, that is ultimately limited by the hardware of the system (i.e. it can be CPU bound or Network Bandwidth bound).

%The first hypothesis of our analysis is that the  baseline system with no caching but with a uniform pattern access is botllenecked by the available network bandwidth. Under this assumption the maximum throughput in that system is achieved, without fully utilizing the CPU capabilities of the servers. Either not all cores are used or the cores are spending most of the time busy looping waiting for the requests.% 

In the caching system, if we assume a zipfian distribution with exponent $a=0.99$ and a software cache that stores the 0.1\% hottest data items of the workload, then 65\% of the total requests will be cache hits, according to Figure \ref{figC:caching}. The rest 35\% of the accesses are requests to cold objects, each of which needs to be propagated to the appropriate remote server within the KVS. The throughput at which the cold requests can be serviced is capped by the throughput of one server in the baseline system. Therefore, in our example the upper bound of the throughput that the caching server can achieve is 2.85 \footnote{$100/35 =2.85$} times the throughput of the baseline server. 

To achieve this upper-bound, two hypotheses must hold true: 
\begin{enumerate}
    \item The baseline system must be bottlenecked by the \antonis{internal} network. More precisely the baseline must under-utilize the CPU enough, such that accessing the hot items in the cache will be essentially free
    \item The accesses to the cold items that miss in the cache must follow a distribution that is close to the uniform
\end{enumerate}

Our evaluation proves both hypotheses. More precisely, we build ccKVS: a black box, RDMA-based KVS with Symmetric Caching that achieves 2.85x in throughput in comparison to a black box baseline under uniform distribution.
% 

==> Text/5-ccKVS-SC/break-even-write-ratio.tex <==
\subsubsection{When does Symmetric Caching break even?}  

%When applying Symmetric Caching, each write to a hot item generates consistency traffic. inside the black box. 
%Therefore, an increase in the write ratio results in an increase in consistency traffic, which leads to a decrease in the rate at which cache misses are handled. As discussed, the performance of ccKVS is determined by the rate at which it can serve the cache misses and therefore, a decrease in that rate can be directly correlated to the maximum performance that the system can achieve. 


Our primary goal is to answer this question: for a deployment of X servers what is the write ratio at which the ccKVS yields the same throughput as Uniform.
We call this write ratio the \textit{break-even write ratio}. Figure~\ref{figC:break-even} illustrates the break-even write ratio for a ccKVS-SC and ccKVS-Lin deployment of up to 40 servers. For example, a ccKVS-SC deployment with 20 servers will yield the same performance as Uniform at a write ratio of $8\%$. As expected the break-even write ratios of ccKVS-LIN are consistently lower than ccKVS-SC. The reason behind this is that a write in ccKVS-Lin translates into more consistency messages, because LIN requires a two-phase protocol that contains a round of invalidations and acknowledgements before the update.

Additionally we note that, as the number of servers increases the break-even write ratio decreases in both consistency models. The reason this happens is because the consistency traffic increases linearly with the number of servers, since a write to a hot object must be propagated to all servers. With 40 servers the break-even write ratio is almost $4\%$ for ccKVS-SC and $1.7\%$ for ccKVS-Lin. This indicates that in a moderately sized deployment ccKVS outperforms the baseline for moderate write ratios, while maintaining strong consistency guarantees.\vasilis{it may be good to add that this study is independent of the skew}


\begin{comment}

As discussed in Section~\ref{secC:write-perf}, the throughput of ccKVS is proportional to the proportion of data traffic in the network. 
Using this correlation, we build an analytical model that computes the throughput as the proportion of data traffic to the
%decrease in the rate at which cache misses can be serviced, 
consistency traffic changes, for both ccKVS-SC and ccKVS-Lin. 
Our primary goal is to answer this question: for a deployment of X servers what is the write ratio at which the ccKVS yields the same throughput as Uniform.
We call this write ratio the \textit{break-even write ratio}. Figure~\ref{figC:break-even} illustrates the break-even write ratio for a ccKVS-SC and ccKVS-Lin deployment of up to 40 servers. For example, a ccKVS-SC deployment with 20 servers will yield the same performance as Uniform at a write ratio of $8\%$. As expected the break-even write ratios of ccKVS-LIN are consistently lower than ccKVS-SC. The reason behind this is that a write in ccKVS-Lin translates into more consistency messages, because per-key Linearizability requires a two-phase protocol that contains a round of invalidations and acknowledgements before the update.

Additionally we note that, as the number of servers increases the break-even write ratio decreases in both consistency models. The reason this happens is because the consistency traffic increases linearly with the number of servers, since a write to a hot object must be propagated to all servers. With 40 servers the break-even write ratio is almost $4\%$ for ccKVS-SC and $1.7\%$ for ccKVS-Lin. This indicates that in a moderately sized deployment ccKVS outperforms the baseline for moderate write ratios, while maintaining strong consistency guarantees.\vasilis{it may be good to add that this study is independent of the skew}

\end{comment}

%We note that the break-even write ratio per-key SC decreases as the value size increases, because the consistency consists of solely big messages(i.e. broadcasts). In contrast the break-even write ratio increases with per-key Linearizability when the value size increases, because in that case 2/3 of the consistency traffic is small messages (i.e. acknowledgements and invalidations).
\begin{comment}


\\
The parameters are: \\
\textit{N}: Number of Servers\\
\textit{wr}: Write Ratio\\
%f : cache hit ratio\\
Payloads:\\
\textit{Big}: Big message in Bytes (i.e. read reply, or write request)\\
\textit{Sm}: Small message in Bytes (i.e. read request, or write reply)\\
\textit{Avg}: Average of small and big messages in Bytes\\
\textit{HO}: Header only in Bytes (i.e. the credit message has no payload)\\
\textit{CD}: Credit Divider (i.e. how many credits in a credit update message)\\ 
\\
\end{comment}


\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|}  \hline
\multirow{1}{2em}{\textit{N}} & Number of Servers \\  \hline
\multirow{1}{2em}{\textit{Wr}}  & Write Ratio \\  \hline
\multirow{2}{2em}{\textit{Big}} & Big message in Bytes \\ & (read reply, or write request) \\  \hline
\multirow{2}{2em}{\textit{Sm}}  & Small message in Bytes \\  & (read request, or write reply)\\ \hline
\multirow{2}{2em}{\textit{Cub}}  & Credit Update Batch \\  & (credits in a credit update message)\\  \hline
\multirow{1}{2em}{\textit{Avg}}  & Average of Sm and Big \\  \hline
\multirow{1}{2em}{\textit{Ho}}  & Header only in Bytes \\ \hline
\end{tabular}
\caption{Parameters of the break-even write-ratio }
\end{center}
\end{table}



EC break-even write ratio : 
\begin{equation}
\label{eqC:EC_break_even}
 WR = \frac{Avg(1 - \frac{1}{N})} {(N - 1)(Big + (Ho/Cub))}
\end{equation}
\vasilis{TODO: Antonis will double check these, if we end up using them}
\\SC break-even write ratio :
\begin{equation}
\label{eqC:SC_break_even}
 WR = \frac{Avg(1 - \frac{1}{N})}{(N - 1)(Big + 2Sm + 3(Ho/Cub))}
\end{equation}
\begin{comment}

It is worth noting that the cache hit ratio is factored out of this equation. In other words the break-even write ratio is solely a function of the number of servers and the payloads and it is completely independent of the cache hit ratio. 


It is worth highlighting that the break-even write ratio refers to the point where Symmetric Caching breaks even with a baseline with uniform distribution. Therefore, even when the write ratio is at its break-even point, Symmetric Caching will yield better performance than no caching. 

%DEFEND THE SIZE OF THE BLACK BOX
Figure \ref{figC:break-even} shows the break-even write ratio of a black box with Symmetric caching varying the size of the black box from 5 up to 40 servers. There is no hard constraint on the size of the black box, rather each application can choose a different size according to its write ratio \antonis{and skew(?)} . For example, a KVS that fits in 80 servers can be split into 8 10-server black boxes or 4 20-server black boxes, depending on the write ratio. However, the popularity cache only stores data items that belong to the black box and thus, breaking up the KVS into multiple black boxes will have an effect on the hit ratio of the popularity caches. For a complete study on how the skew varies when decreasing the size of the black box we refer the reader to \cite{RNovakovic:2016}.
\end{comment}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/break_even_performance_study.pdf} 
  \caption{Break-even write-rate study. [$\alpha=0.99$]}
  \label{figC:break-even}
\end{figure}

==> Text/5-ccKVS-SC/chapter.tex <==
\markedchapter{Scale-Out ccNUMA}{Scale-out ccNUMA:\nextlinepdf Replication for Load Balance}
\equote{-40}{10}{The whole is greater than the sum of the parts.}{Aristotle}

\label{chap:cckvs}
\parbox{0.8\textwidth}{

\begin{mybox}[title={\large\textcolor{myThemeColor}{Key Ideas}}]
\begin{myitem}
\item First item. hgb 
\item Second item.
\item Third item.
\end{myitem}
\end{mybox}
}


\input{Text/1-ccKVS/1-Introduction}
\input{Text/1-ccKVS/1.5-Contributions}
\input{Text/1-ccKVS/2-Motivation}
\input{Text/1-ccKVS/3-Case}
\input{Text/1-ccKVS/4-Cache}
\input{Text/1-ccKVS/5-Protocols}
\input{Text/1-ccKVS/6-Design}
\input{Text/1-ccKVS/7-Methodology}
\input{Text/1-ccKVS/8-Evaluation}
\input{Text/1-ccKVS/9-Discussion}
\input{Text/1-ccKVS/10-Related}
\input{Text/1-ccKVS/11-Conclusion}

==> Visuals/Include_graphics/fig_design.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{Visuals/Figures/Design.pdf}
	\caption{Throughput and latency comparison of membership-based protocols.} 
	\capline
  \label{fig:design}
\end{figure}

==> Visuals/Tables/eval-table1.tex <==
\begin{table}[h!]
\centering

\begin{adjustbox}{max width=\textwidth}

\begin{tikzpicture}

\node (table) [inner sep=-0pt] {
\begin{tabular}{l|c|c|c|c|c}
\rowcolor[HTML]{9B9B9B} 
\cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Local reads}} & \multicolumn{3}{c}{\cellcolor[HTML]{9B9B9B}\textbf{Writes}} \\ \cline{2-6} 
\rowcolor[HTML]{9B9B9B} 
\multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{System}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Consistency} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency (RTT) & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}Dec.} \\
\textbf{HermesKV} & one per RM & Lin & inter-key & 1 & \cmark \\
\textbf{rCRAQ} & one per RM & Lin & inter-key & O(\textit{n}) & \xmark \\
\textbf{rZAB} & none & SC & serializes all & 2 $\dagger$ & \xmark \\
\textbf{Derecho} & none & SC & serializes all & 1 $\ddagger$ & \cmark
\end{tabular}
};
\draw [rounded corners=.3em] (table.north west) rectangle (table.south east);

\end{tikzpicture}

\end{adjustbox}


\caption{
Comparison of read and write features for the evaluated systems. 
% Write concurrency and local reads lease usage and consistency for evaluated systems.
SC: sequentially consistent; RM: reliable membership; Dec: decentralized; \textit{n}: number of replicas; $\dagger$1 RTT for master's writes; $\ddagger$lock-step commit.}
% \rule[1ex]{14.5cm}{0.5pt}
\capline
% Protocols that provide SC cannot be deployed per-key since SC is not composable.}
\label{tabH:eval}
\vspace{-25pt}
\end{table}

==> Visuals/toc-style.tex <==
\usepackage[T1]{fontenc}
\usepackage{refcount}
\usepackage[colorlinks,linkcolor=black]{hyperref}
\usepackage{tikz}
\usetikzlibrary{calc}

% colors to be used
\definecolor{myred}{RGB}{127,0,0}
\definecolor{myyellow}{RGB}{169,121,69}

% a command to circle the part numbers
\newcommand\Circle[1]{\tikz[overlay,remember picture] 
  \node[draw=myyellow,circle, text width=18pt,line width=1pt,align=center] {#1};}

% redefinition of the name of the ToC
\renewcommand\printtoctitle[1]{\HUGE\sffamily\bfseries\color{myred}#1}

\makeatletter
% redefinitions for part entries
\renewcommand\cftpartfont{\Huge\sffamily\bfseries}
\renewcommand\partnumberline[1]{%
    \hbox to \textwidth{\hss\Circle{\textcolor{myyellow}{#1}}\hss}%
  \vskip3.5ex\color{myred}}

\renewcommand*{\l@part}[2]{%
  \ifnum \c@tocdepth >-2\relax
    \cftpartbreak
    \begingroup
      {\interlinepenalty\@M
       \leavevmode
       \settowidth{\@tempdima}{\cftpartfont\cftpartname}%
       \addtolength{\@tempdima}{\cftpartnumwidth}%
       \let\@cftbsnum \cftpartpresnum
       \let\@cftasnum \cftpartaftersnum
       \let\@cftasnumb \cftpartaftersnumb
       \advance\memRTLleftskip\@tempdima \null\nobreak\hskip -\memRTLleftskip
       \centering{\cftpartfont#1}\par%
       }
      \nobreak
        \global\@nobreaktrue
        \everypar{\global\@nobreakfalse\everypar{}}%
    \endgroup
  \fi}

% redefinitions for chapter entries
\renewcommand\chapternumberline[1]{\mbox{\Large\@chapapp~#1}\par\noindent}
\renewcommand\cftchapterfont{\Large\sffamily}
\cftsetindents{chapter}{0pt}{0pt}
\renewcommand\cftchapterpagefont{\HUGE\sffamily\bfseries\color{myred}}

\newcommand*{\l@mychap}[3]{%
  \def\@chapapp{#3}\vskip1ex%
  \par\noindent\begin{minipage}{\textwidth}%
  \parbox{4.7em}{%
    \hfill{\cftchapterpagefont#2}%
  }\hspace*{1.5em}%
  \parbox{\dimexpr\textwidth-4.7em-15pt\relax}{%
    \cftchapterfont#1%
  }%
  \end{minipage}\par\vspace{2ex}%
}

\renewcommand*{\l@chapter}[2]{%
  \l@mychap{#1}{#2}{\chaptername}%
}

\renewcommand*{\l@appendix}[2]{%
  \l@mychap{#1}{#2}{\appendixname}%
}

% redefinitions for section entries
\renewcommand\cftsectionfont{\sffamily}
\renewcommand\cftsectionpagefont{\sffamily\itshape\color{myred}}
\renewcommand{\cftsectionleader}{\nobreak}
\renewcommand{\cftsectionafterpnum}{\cftparfillskip}
\cftsetindents{section}{7.5em}{3em}
\renewcommand\cftsectionformatpnum[1]{%
  \hskip1em\hbox to 4em{{\cftsectionpagefont #1\hfill}}}

% redefinitions for subsection entries
\renewcommand\cftsubsectionfont{\sffamily}
\renewcommand\cftsubsectionpagefont{\sffamily\itshape\color{myred}}
\renewcommand\cftsubsectionleader{\nobreak}
\renewcommand{\cftsubsectionafterpnum}{\cftparfillskip}
\renewcommand\cftsubsectiondotsep{\cftnodots}
\cftsetindents{subsection}{10.5em}{3em}
\renewcommand\cftsubsectionformatpnum[1]{%
  \hskip1em\hbox to 4em{{\cftsubsectionpagefont #1\hfill}}}
\makeatother

\settocdepth{subsection}
\setsecnumdepth{subsection}

% length to be used when drawing a line from the top of the text area
\newlength\Myhead
\setlength\Myhead{\dimexpr\headheight+\headsep+1in+\voffset+5ex\relax}

% length to be used when drawing a line to the bottom of the text area
\newlength\Myfoot
\setlength\Myfoot{\dimexpr\paperheight-\Myhead-\textheight-\footskip+5ex\relax}

% auxiliary counter to place labels
\newcounter{chapmark}

% Adds a mark and a label at the beginning of each chapter entry in the ToC and draws a line 
% from the start of the chapter to the bottom of the text area if the mark 
% for the chapter ending lies in a different page than the one from the end of the chapter.
% (the value of tjose pages is calculated using the label)
% Must be used right before each \chapter command
\newcommand\StartMark{%
  \addtocontents{toc}{\protect\label{st\thechapmark}%
    \protect\begin{tikzpicture}[overlay,remember picture,baseline]   
    \protect\node [anchor=base] (s\thechapmark) {};%
    \ifnum\getpagerefnumber{st\thechapmark}=\getpagerefnumber{en\thechapmark} \else
    \protect\draw[myyellow,line width=3pt] let \protect\p3= (s\thechapmark),%
      \protect\p4 = (current page.south) in %
      ($ (4em,\protect\y3) + (0,-1ex) $) -- ($ (4em,\protect\y4) + (0,\protect\the\Myfoot)$);\fi
    \protect\end{tikzpicture}\par}%
}

% Adds a mark and a label at the end of each chapter entry in the ToC and draws a line from 
% the top of the text area to the ending of the chapter if the mark 
% for the chapter ending lies in a different page than the one from the start of the chapter
% if both marks are in the same page, simple draws a line connecting the marks
% (the value of tjose pages is calculated using the label)
% Must be used right after the last sectional unit (that will go to the ToC) belonging to 
% a chapter
\newcommand\EndMark{
\addtocontents{toc}{\protect\label{en\thechapmark}%
  \protect\begin{tikzpicture}[overlay,remember picture,baseline]   
  \protect\node [anchor=base] (e\thechapmark) {};
  \ifnum\getpagerefnumber{st\thechapmark}=\getpagerefnumber{en\thechapmark} 
  \protect\draw[myyellow,line width=3pt] let \protect\p1= (s\thechapmark), \protect\p2=(e\thechapmark) in ($ (4em,\protect\y1) + (0,-1ex) $) -- ($ (4em,\protect\y2) + (0,2ex) $);
  \else%
  \protect\draw[myyellow,line width=3pt] let \protect\p1= (e\thechapmark), \protect\p2=(current page.north) in ($(4em,\protect\y2) + (0,-\protect\the\Myhead)$) -- ($ (4em,\protect\y1) + (0,1.5ex) $);
\fi
\protect\end{tikzpicture}\par}\stepcounter{chapmark}%
}

==> Visuals/toc-style2.tex <==
% \documentclass{tufte-book}
\usepackage{lmodern}
\usepackage{tikzpagenodes}
\usetikzlibrary{calc}

\newcounter{chapmark}
\setcounter{tocdepth}{1}

\colorlet{mycolor}{BrickRed}

\titlecontents{chapter}%
  [0em]
  {\vspace{1.5\baselineskip}\begin{fullwidth}\LARGE\rmfamily\itshape}
  {\hspace*{0em}\thecontentslabel}
  {\hspace*{0em}\llap{%
    \parbox[b]{40pt}{%
      \fontsize{25}{30}\sffamily\bfseries\color{mycolor}%
      \hfill\thecontentspage%
      }\hspace{20pt}%
    }%
  }
  {\rmfamily\upshape\qquad}
  [\end{fullwidth}]

\titlecontents{section}
  [0em]
  {\vspace{0\baselineskip}\begin{fullwidth}\Large\rmfamily\itshape}
  {\hspace*{0em}\contentslabel{2em}}
  {\llap{\parbox[b]{40pt}{\hfill\thecontentspage}\hspace{20pt}}\hspace*{0em}}
  {\rmfamily\upshape\qquad}
  [\end{fullwidth}]

\titlecontents{subsection}
  [0em]
  {\vspace{-.15\baselineskip}\begin{fullwidth}\large\rmfamily\itshape}
  {\hspace*{0em}\contentslabel{4em}}
  {\llap{\parbox[b]{40pt}{\hfill\small\thecontentspage}\hspace{20pt}}\hspace*{0em}}
  {\rmfamily\upshape}
  [\end{fullwidth}] 

\newcommand\StartMark{%
\addtocontents{toc}{\protect\label{st\thechapmark}%
\par\protect\begin{tikzpicture}[overlay,remember picture,baseline]   
  \protect\node [anchor=base] (s\thechapmark) {};%
  \ifnum\getpagerefnumber{st\thechapmark}=\getpagerefnumber{en\thechapmark}   
  \else
    \protect\draw[mycolor,line width=3pt] 
      let \protect\p3= (s\thechapmark),%
            \protect\p4 = (current page text area.south) in %
      ( $ (0em,\protect\y3) + (-20pt,-5ex) $ ) -- 
      ( $ (0em,\protect\y4) + (-20pt,-5pt) $ );
  \fi
\protect\end{tikzpicture}\par}%
}

\newcommand\EndMark{%
\addtocontents{toc}{\protect\label{en\thechapmark}%
\par\protect\begin{tikzpicture}[overlay,remember picture,baseline]   
  \protect\node [anchor=base] (e\thechapmark) {};
  \ifnum\getpagerefnumber{st\thechapmark}=\getpagerefnumber{en\thechapmark} 
    \protect\draw[mycolor,line width=3pt] 
    let \protect\p1= (s\thechapmark), 
          \protect\p2=(e\thechapmark) in %
    ( $ (0em,\protect\y1) + (-20pt,-5ex) $ ) -- 
    ( $ (0em,\protect\y2) + (-20pt,2ex) $ );
  \else%
  \protect\draw[mycolor,line width=3pt] 
  let \protect\p1= (e\thechapmark), 
        \protect\p2=(current page text area.north) in 
  ( $ (0em,\protect\y2) + (-20pt,5pt) $ ) -- 
  ( $ (0em,\protect\y1) + (-20pt,2ex) $ );
  \fi
\protect\end{tikzpicture}\par}%
\stepcounter{chapmark}%
}


==> Visuals/toc-style3.tex <==
\usepackage{xcolor}
\usepackage{framed}
\usepackage{tikz}
\usepackage{lmodern}
\usepackage{etoc}
\usepackage[linktoc=all]{hyperref}

%% THE FOLLOWING IS TAKEN (STOLEN) VERBATIM 
%% FROM GONZALO MEDINA'S ANSWER

% definition of some personal colors
\definecolor{myred}{RGB}{127,0,0}
\definecolor{myyellow}{RGB}{169,121,69}

% command for the circle for the number of part entries
\newcommand\Circle[1]{\tikz[overlay,remember picture] 
  \node[draw,circle, text width=18pt,line width=1pt] {#1};}


%% (jfbu) This defines an adjustable length, which gives the position of the
%% section and subsection from the left document margin.
\newlength{\tocmargin}
% Its value is set in the \etocsettocstyle command below, after \sffamily


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% USE OF framed package

% modified (jfbu): it took me a while to settle on that way of using the
% framed package. Initially I had as in Gonzalo Medina's code
% a \parshape, but it applies only to one paragraph (this was from his
% code where the left bar applied only to the chapter entries of the
% toc, not the sections and subsections). Besides, I had some problems
% with disturbing page breaks in certain circumstances, and these
% problems seem to be gone now, I needed to do adjustment to \hsize from
% inside the chapter style. This is all gone now.
\newenvironment{tocleftbar}
  {\def\FrameCommand {\hspace{\dimexpr\tocmargin-4pt\relax}%
           {\color{myyellow}\vrule width 2pt depth 6pt}\hspace{2pt}%
           \hspace{-\tocmargin}}% 
    \MakeFramed {\leftskip\tocmargin\rightskip\tocmargin\FrameRestore}}
 {\endMakeFramed}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% THE PLAGIARISM CONTINUES, WITH SOME MORE MODIFICATIONS, 
%% AND  EMBEDDED INSIDE ETOC COMMANDS

\etocsetstyle{part}
   {\nobreak\etocskipfirstprefix }
   {\pagebreak[3]}% makes a page break before a Part favorable
   {% debugging:
    % \noindent\rule{\tocmargin}{1pt}\par
    %          \rule{\dimexpr2\tocmargin\relax}{1pt}\par
    \addvspace{1.5\baselineskip}%
    {\huge\centering
     \color{myyellow}\Circle{\hfil\etocnumber\hfil}\\*[2ex]%
     \color{myred}\etocname\par}}
   {}

% totalement instable: passer de 2ex à 2.5ex suffit à tout bouleverser!
% toutes choses égales par ailleurs.


\newif\ifintocleftbar

\etocsetstyle{chapter}
% don't break immediately after Part
   {\nobreak\etocskipfirstprefix }
% but allow break after section or subsection
   {\pagebreak[2]}
   {%\addvspace{\baselineskip}%
    % it seems that framed's code too easily allows a page break 
    % if some vertical glue is here, so let's use a \kern
    \kern\baselineskip
    \begin{tocleftbar}
      \intocleftbartrue
      \makebox[0pt][r]{\smash{\parbox{6em}%
                       {\null\hfill\Huge\bfseries\color{myred}\etocpage
                        \hspace*{8pt}}}}%
% use of \parbox, else framed.sty has a tendency to allow page breaks if
% multi-line name
      \parbox[t]{\dimexpr\hsize-2\tocmargin\relax}
      {\Large\textsc{\small \etoclink{Chapter~\etocthenumber}}%
%\\* does not do what I want. \par\nobreak does.
% But as we are now in \parbox, does not matter
      \par\etocname\rule[-\baselineskip]{0pt}{0pt}}%
      \par
      \normalsize\leftskip\dimexpr\leftskip+3em\relax
    }
   {}

% THIS IS A VARIANT ABLE TO COPE WITH CHAPTERS WITHOUT SECTIONS
% it is **complicated** because \etocname etc.. loose their meaning if one
% closes a group in the third ("prefix")  or fourth ("contents")
% arguments to \etocsetstyle. Thus, we have to save them before
% issueing \end{tocleftbar} to close the previous left bar environment.
% Although the code mentions \etocthelink, etc, it works also if
% hyperref is not loaded.
% \etocsetstyle{chapter}
%    {\nobreak\etocskipfirstprefix}% don't break immediately after Part
%    {\pagebreak[2]}% but allow break after section or subsection
%    {\global\let\ETOCthepage\etocthepage
%                    \global\let\ETOCthename\etocthename
%                    \global\let\ETOCthenumber\etocthenumber
%                    \global\let\ETOCthelink\etocthelink
%     \ifintocleftbar\end{tocleftbar}\fi%
%     \kern\baselineskip
%     \begin{tocleftbar}
%       \intocleftbartrue
%       \makebox[0pt][r]{\smash{\parbox{6em}%
%                        {\null\hfill\Huge\bfseries\color{myred}%
%                         \ETOCthelink{\ETOCthepage}%
%                         \hspace*{8pt}}}}%
%       \parbox[t]{\dimexpr\hsize-2\tocmargin\relax}
%       {\Large\textsc{\small \ETOCthelink{Chapter~\ETOCthenumber}}%
% %\\* does not do what I want. \par\nobreak does.
% % But as we are now in \parbox, does not matter
%       \par\ETOCthelink{\ETOCthename}\rule[-\baselineskip]{0pt}{0pt}}%
%       \par
%       \normalsize\leftskip\dimexpr\leftskip+3em\relax
%     }
%    {\ifintocleftbar\end{tocleftbar}\fi}


\etocsetstyle {section}
% avoid break after Chapter
  {\nopagebreak[3]\vspace{1pt}\etocskipfirstprefix}
% allow break after previous subsection or section
  {\vspace {1pt plus .2pt minus .2pt}}
  {\makebox[0pt][r]{\makebox[3em][l]{\etocnumber}}%
   \etocname
   \hspace{0.5em}\nobreak{\itshape\color{myred}\etocpage}\par }
  {\end{tocleftbar}}


% IMPORTANT: this is ALSO executed if the last thing
                   % before the next chapter is a subsection

\etocsetstyle {subsection}
% avoid break immediately after section
  {\nopagebreak[2]\vspace{1pt}\etocskipfirstprefix}
  {\vspace {1pt plus .2pt minus .2pt}}%
  % {\etocskipfirstprefix}
  % {\pagebreak[2]\etocskipfirstprefix}% allow break after previous subsection
  {\makebox[0pt][r]{\makebox[3em][l]{\etocnumber}}\etocname
   \hspace{0.5em}\nobreak{\itshape\color{myred}\etocpage}\par }
  {}


\etocsettocstyle{\sffamily\setlength{\tocmargin}{5.4em}%
          {\Huge\bfseries\color{myred}\contentsname\par}%
          \leftskip 0pt\parindent 0pt }{}

  % for memoir class: (does no harm otherwise) [Nota Bene: this should
  % perhaps be done automatically by etoc when it detects the memoir
  % class, for better compatibility]
\etocsetlevel {appendix}{0}

==> Visuals/toc-style4.tex <==
\usepackage[utf8]{inputenc}
\usepackage{kpfonts}
\usepackage[tmargin=2cm,rmargin=3.8cm,lmargin=3.8cm,bmargin=2cm]{geometry}
\usepackage{tikz}
\definecolor{doc}{RGB}{0,60,110}
\usepackage{titletoc}
\contentsmargin{0cm}
\titlecontents{chapter}[0pc]
{\addvspace{30pt}%
\begin{tikzpicture}[remember picture, overlay]%
\draw[fill=doc!30,draw=doc!30] (-4,-.1) rectangle (-1,.5);%
\pgftext[left,x=-3.7cm,y=0.2cm]{\color{white}\Large\sc\bfseries chapter\ \thecontentslabel};%
\end{tikzpicture}\color{doc!40}\large\sc\bfseries}%
{}
{}
{\;\titlerule\;\large\sc\bfseries Page \thecontentspage
\begin{tikzpicture}[remember picture, overlay]
\draw[fill=doc!25,draw=doc!20] (2pt,0) rectangle (6,0.1pt);
\end{tikzpicture}}%
\titlecontents{section}[2.4pc]
{\addvspace{1pt}}
{\contentslabel[\thecontentslabel]{2.4pc}}
{}
{\hfill\small \thecontentspage}
[]
\titlecontents*{subsection}[4pc]
{\addvspace{-1pt}\small}
{}
{}
{\ --- \small\thecontentspage}
[ \textbullet\ ][]

\makeatletter
\renewcommand{\tableofcontents}{%
\chapter*{%
\vspace*{-20\p@}%
\begin{tikzpicture}[remember picture, overlay]%
\pgftext[right,x=15cm,y=0.2cm]{\color{doc!30}\Huge\sc\bfseries \contentsname};%
\draw[fill=doc!30,draw=doc!30] (13,-.75) rectangle (20,1);%
\clip (13,-.75) rectangle (20,1);
\pgftext[right,x=15cm,y=0.2cm]{\color{white}\Huge\sc\bfseries \contentsname};%
\end{tikzpicture}}%
\@starttoc{toc}}
\makeatother

==> inj_to_inf.tex <==
%%% WARNING this is only so that we have dedication and acks before the abstract
% \begin{comment}
 \input{Text/0-Preface/dedication}
\pagebreak
\input{Text/0-Preface/acknowledgements} %TODO open for final

\input{Text/0-Preface/lay}
% \end{comment}


